A Digitalization Framework for Smart Maintenance of Historic Buildings

Smart maintenance of historic buildings involves integration of digital technologies and data analysis methods to help maintain functionalities of these buildings and preserve their heritage values. However, the maintenance of historic buildings is a long-term process. During the process, the digital transformation requires overcoming various challenges, such as stable and scalable storage and computing resources, a consistent format for organizing and representing building data, and a flexible design to integrate data analytics to deliver applications. This licentiate thesis aims to address these challenges by proposing a digitalization framework that integrates Internet of Things (IoT), cloud computing, ontology, and machine learning. IoT devices enable data collection from historic buildings to reveal their latest status. Using a public cloud platform brings stable and scalable resources for storing data, performing analytics, and deploying applications. Ontologies provide a clear and concise way to organize and represent building data, which makes it easier to understand the relationships between different building components and systems. Combined with IoT devices and ontologies, parametric digital twins can be created to evolve with their physical counterparts. Furthermore, with machine learning, digital twins can identify patterns from data and provide decision-makers with insights to achieve smart maintenance. Overall, this thesis contributes to the field of preservation of historic buildings by proposing a comprehensive digitalization framework that integrates various advanced digital technologies to provide a holistic approach to achieve smart maintenance of historic buildings.

==> abstract.tex <==
%%% Abstract.tex --- 
%% 
%% Filename: Abstract.tex
%% Description: 
%% Author: Ola Leifler
%% Maintainer: 
%% Created: Thu Oct 14 13:34:11 2010 (CEST)
%% Version: $Id$
%% Version: 
%% Last-Updated: Fri Jan 14 08:48:50 2022 (+0100)
%%           By: Ola
%%     Update #: 6
%% URL: 
%% Keywords: 
%% Compatibility: 
%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% 
%%% Commentary: 
%% 
%% 
%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% 
%%% Change log:
%% 
%% 
%% RCS $Log$
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% 
%%% Code:

Smart maintenance of historic buildings involves integration of digital technologies and data analysis methods to help maintain functionalities of these buildings and preserve their heritage values. However, the maintenance of historic buildings is a long-term process. During the process, the digital transformation requires overcoming various challenges, such as stable and scalable storage and computing resources, a consistent format for organizing and representing building data, and a flexible design to integrate data analytics to deliver applications.

This licentiate thesis aims to address these challenges by proposing a digitalization framework that integrates Internet of Things (IoT), cloud computing, ontology, and machine learning. IoT devices enable data collection from historic buildings to reveal their latest status. Using a public cloud platform brings stable and scalable resources for storing data, performing analytics, and deploying applications. Ontologies provide a clear and concise way to organize and represent building data, which makes it easier to understand the relationships between different building components and systems. Combined with IoT devices and ontologies, parametric digital twins can be created to evolve with their physical counterparts. Furthermore, with machine learning, digital twins can identify patterns from data and provide decision-makers with insights to achieve smart maintenance.

Papers I--III have shown that data can be reliably collected, transmitted, and stored in the cloud. Results of Paper IV indicate that a digital twin that depicts the latest status of a historic building can be created and fed with real-time sensor data. The insights discovered from the digital twin provide facts for improving the indoor climate to achieve both heritage conservation and human comfort. Papers V and VI have shown that deep learning methods exhibit strong capabilities in capturing tendency and uncertainty in building energy consumption. Incorporating future information that determines energy consumption is critical for making multi-horizon predictions. Moreover, changes in the operating mode of a building and activities held in a building bring more uncertainty in energy consumption and deteriorate the performance of point forecasts. 

Overall, this thesis contributes to the field of preservation of historic buildings by proposing a comprehensive digitalization framework that integrates various advanced digital technologies to provide a holistic approach to achieve smart maintenance of historic buildings.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Abstract.tex ends here


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "demothesis"
%%% End: 


==> acknowledgments.tex <==
%%% Acknowledgments.tex<2> --- 
%% 
%% Filename: Acknowledgments.tex<2>
%% Description: 
%% Author: Ola Leifler
%% Maintainer: 
%% Created: Wed Nov 10 09:45:11 2010 (CET)
%% Version: $Id$
%% Version: 
%% Last-Updated: Tue Jun 21 13:28:03 2016 (+0200)
%%           By: Ola Leifler
%%     Update #: 6
%% URL: 
%% Keywords: 
%% Compatibility: 
%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% 
%%% Commentary: 
%% 
%% 
%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% 
%%% Change log:
%% 
%% 
%% RCS $Log$
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% 
%%% Code:

\swedishenglish{\chapter*{Författarens tack}}{\chapter*{Acknowledgments}}

First of all, I extend my sincere appreciation to my supervisors, Professor Shaofang Gong and Senior Associate Professor Magnus Karlsson. Shaofang offered me the opportunity to do this interesting research. His guidance, expertise, and support throughout this research journey have been invaluable. Magnus always provides insightful feedback and constructive criticism, continually pushing me to strive for excellence.

I am indebted to my mentor, Dr. Yu Liu, for his valuable input, advice, and encouragement. I would also like to acknowledge the contributions of Gustav Knutsson and other colleagues within the Division of Physics, Electronics, and Mathematics as well as the Department of Science and Technology. Their intellectual discussions, collaborative spirit, and willingness to share their knowledge have greatly enriched my research experience.

Special recognition goes to the collaborators from Uppsala University, Campus Gotland, RISE in Link\"oping, and Norrevo Fastigheter AB in Norrk\"oping within the research project. Their expertise, cooperation, and willingness to share resources and insights have significantly contributed to the success of this study.

Last but not least, I would like to thank my parents, Weibin Ni and Jianhong Luo, as well as my parents-in-law, Guoliang Zhang and Dewen Liu, for their unwavering love and encouragement. To my wife, Chi Zhang, your patience, understanding, and wisdom have been a constant source of inspiration. I want to thank my son Leo for his innocent joy, laughter, and boundless energy.

This research has been financially supported by the Swedish Energy Agency within the research program of \textit{Spara och Bevara}.

\vspace{5mm}

\noindent{Zhongjun Ni}

\noindent{Norrk\"oping, June 2023}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Acknowledgments.tex<2> ends here

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "demothesis"
%%% End: 


==> listofabbreviations.tex <==
\chapter*{List of Abbreviations}

\begingroup

\renewcommand{\arraystretch}{1.5}

\begin{table}[!h]
\begin{tabular}{@{}llll@{}}
3D      &  &  & three dimensional                                      \\
AI      &  &  & artificial intelligence                                \\
ANOVA   &  &  & one-way analysis of variance                           \\
API     &  &  & application programming interface                      \\
BIM     &  &  & building information modeling                          \\
BMS     &  &  & building management system                             \\
CO\textsubscript{2}     &  &  & carbon dioxide                                         \\
CV-RMSE &  &  & coefficient of variation of the root mean square error \\
EDA     &  &  & exploratory data analysis                              \\
GRU     &  &  & gated recurrent unit                                   \\
HVAC    &  &  & heating, ventilation, and air conditioning             \\
ID      &  &  & identity                                               \\
IoT     &  &  & Internet of Things                                     \\
LR      &  &  & linear regression                                      \\
LSTM    &  &  & long short-term memory                                 \\
N-HiTS  &  &  & hierarchical interpolation for time series forecasting \\
NMBE    &  &  & normalized mean bias error                             \\
RH      &  &  & relative humidity                                      \\
SMHI    &  &  & Swedish Meteorological and Hydrological Institute      \\
TCN     &  &  & temporal   convolutional network                       \\
TF      &  &  & transformer                                            \\
TFT     &  &  & temporal fusion transformer                           
\end{tabular}
\end{table}

\endgroup

==> listofpublications.tex <==
\chapter*{List of Publications}

\textbf{Papers included in this thesis:}
{\footnotesize
\begin{enumerate}[{[I]}]
  \item \textbf{Z. Ni}, P. Eriksson, Y. Liu, M. Karlsson, and S. Gong, “Improving Energy Efficiency while Preserving Historic Buildings with Digital Twins and Artificial Intelligence,” \textit{SBE21 Sustainable Built Heritage}, Bolzano-Bozen, Italy, 14--16 Apr. 2021.
  \item \textbf{Z. Ni}, Y. Liu, M. Karlsson, and S. Gong, “Link Historic Buildings to Cloud with Internet of Things and Digital Twins,” \textit{The 4th International Conference on Energy Efficiency in Historic Buildings}, Benediktbeuern, Germany, 4--5 May 2022.
  \item \textbf{Z. Ni}, Y. Liu, M. Karlsson, and S. Gong, “A Sensing System Based on Public Cloud to Monitor Indoor Environment of Historic Buildings,” \textit{Sensors}, vol. 21, no. 16, p. 5266, 2021.
  \item \textbf{Z. Ni}, Y. Liu, M. Karlsson, and S. Gong, “Enabling Preventive Conservation of Historic Buildings Through Cloud-based Digital Twins: A Case Study in the City Theatre, Norrk\"oping,” \textit{IEEE Access}, vol. 10, pp. 90924–90939, 2022.
  \item \textbf{Z. Ni}, C. Zhang, M. Karlsson, and S. Gong, “A Study of Deep Learning-based Multi-horizon Building Energy Forecasting,” Manuscript, 2023.
  \item \textbf{Z. Ni}, C. Zhang, M. Karlsson, and S. Gong, “Leveraging Deep Learning and Digital Twins to Improve Energy Performance of Buildings,” accepted in \textit{The 3rd IEEE International Conference on Industrial Electronics for Sustainable Energy Systems}, 2023.
\end{enumerate}
}

\vspace{5mm}

\noindent\textbf{Papers not included in this thesis:}
{\footnotesize
\begin{enumerate}[{[I]}]\addtocounter{enumi}{6}
  \item Y. Liu, \textbf{Z. Ni}, M. Karlsson, and S. Gong, “Methodology for Digital Transformation with Internet of Things and Cloud Computing: A Practical Guideline for Innovation in Small-and Medium-Sized Enterprises,” \textit{Sensors}, vol. 21, no. 16, p. 5355, 2021.
  \item Y. Liu, S. Mousavi, Z. Pang, \textbf{Z. Ni}, M. Karlsson, and S. Gong, “Plant Factory: A New Playground of Industrial Communication and Computing,” \textit{Sensors}, vol. 22, no. 1, p. 147, 2022.
  \item C. Zhang, AH. Kalantari, Y. Yang, \textbf{Z. Ni}, G. Markkula, N. Merat, C. Berger, “Cross or Wait? Predicting Pedestrian Interaction Outcomes at Unsignalized Crossings,” \textit{2023 IEEE Intelligent Vehicles Symposium (IV)}, Anchorage, Alaska, USA, 4--7 Jun. 2023.
  \item C. Zhang, \textbf{Z. Ni}, C. Berger, “Spatial-Temporal-Spectral LSTM: A Transferable Model for Pedestrian Trajectory Prediction,” accepted in \textit{IEEE Transactions on Intelligent Vehicles}, 2023.
\end{enumerate}
}

==> papers/ni_enabling_2022.tex <==
\begin{abstract}
Historic buildings require good maintenance to sustain their function and preserve embodied heritage values. Previous studies have demonstrated the benefits of digitalization techniques in improving maintenance and managing threats to historic buildings. However, there still lacks a solution that can consistently organize data collected from historic buildings to reveal operating conditions of historic buildings in real-time and to facilitate various data analytics and simulations. This study aims to provide such a solution to help achieve preventive conservation. The proposed solution integrates Internet of Things and ontology to create digital twins of historic buildings. Internet of Things enables revealing the latest status of historic buildings, while ontology provides a consistent data schema for representing historic buildings. This study also gives a reference implementation by using public cloud services and open-source software libraries, which make it easier to be reused in other historic buildings. To verify the feasibility of the solution, we conducted a case study in the City Theatre, Norrk\"oping, Sweden. The obtained results demonstrate the advantages of digital twins in providing maintenance knowledge and identifying potential risks caused by fluctuations of relative humidity.
\end{abstract}

% \begin{keywords}
% digital twin, historic building, indoor environment, Internet of Things
% \end{keywords}


% \begin{category}
%   H.5.3, H.5.4%,M.1, M.4
% \end{category}

% \sloppy{}
\begin{refsection}

\section{Introduction}
\label{sec:enabling_introduction}

Preventive conservation is important for historic buildings because damages to cultural heritage should be avoided rather than be addressed after it has occurred~\cite{marra_digital_2021}. Threats to cultural heritage can be caused by many factors, such as vandalism, natural disasters, and improper environment~\cite{ashrae_handbook_hvac_applications_2011}. For example, in historic buildings used as museums, improper environmental conditions, such as relative humidity (RH) and temperature, might accelerate deterioration in both buildings and housed collections~\cite{balen_preventive_2015}. 
Maintaining a theoretically ideal environment can slow deterioration significantly. However, it also needs to consider public access, e.g., visitors, and financial cost in reality~\cite{ashrae_handbook_hvac_applications_2011}.
For instance, considering both heritage conservation and human comfort, for national museums with diverse collections, the suggested RH is 45--60\%, while the temperature is 19$\pm$1~\textdegree{}C in winter and 24$\pm$1~\textdegree{}C in summer~\cite{thomson_museum_1994}. For historic buildings where the goal is to minimize severe hazards while keeping costs, the RH can be kept at 40--70\%~\cite{thomson_museum_1994}. Therefore, solutions that can manage threats while being cost-effective are significant for preserving historic buildings.

Digital transformation of historic buildings, such as monitoring and modeling, help achieve preventive conservation since they enable the timely maintenance and implementation of necessary interventions~\cite{colace_iot_2021}. For example, environmental monitoring is necessary to prevent fluctuations from causing irreversible and unforeseen damage to materials and discomfort to occupants~\cite{lucchi_review_2018}. Modeling relatively static properties like geometric characteristics helps manage and restore historic buildings~\cite{yang_review_2020}. To reduce operation costs, the indoor environment of historic buildings could be controlled more efficiently~\cite{leijonhufvud_standardizing_2018, ni_improving_2021}, such as adopting an occupancy level-based control strategy~\cite{hammar_realestatecore_2019}.

Several digitalization techniques have been used to monitor and model historic buildings. Considerable research was devoted to 3D geometry modeling of historic buildings~\cite{bruno_historic_2018}. Many techniques, such as 3D computer graphics, photogrammetry, and laser scanning, are used for modeling, managing, and preserving architectural heritage~\cite{yang_review_2020}. However, information stored in such systems is usually static and cannot reflect the real-time operating status of historic buildings. Another bulk of studies deployed wired or wireless sensor networks (WSNs) to monitor the status of historic buildings, such as indoor environment~\cite{zhang_culturebee_2011,ni_sensing_2021} and structural health~\cite{barsocchi_wireless_2021}. Nevertheless, such monitoring studies primarily focused on data collection, transmission, and storage, with little emphasis on data analytics and converting analysis results into applications that benefit the conservation of historic buildings. Also, preserving historic buildings involve many specialists with different backgrounds, and the solutions proposed in these studies do not effectively support knowledge sharing and collaboration. To discover insights and facilitate preservation, some studies~\cite{angjeliu_development_2020, zhang_automatic_2022} have attempted to create digital twins (DTs) of historic buildings. However, the solutions provided in these studies are difficult to transfer to other historic buildings due to the lack of a consistent, reusable, and extendable data format to represent buildings. Lacking a consistent data representation also restricts interoperability between subsystems of a building and limits the implementation of applications~\cite{balaji_brick_2018}.

In this study, we aim to promote the preventive conservation of historic buildings through digitalization techniques, with a focus on mitigating the challenges in creating DTs of historic buildings. The main contributions of this work are as follows:
\begin{itemize}
\item Proposed a solution that can consistently represent the data in historic buildings, reflect the latest operating status of historic buildings, and facilitate further data analytics. The solution combines Internet of Things (IoT) and ontology to create DTs of historic buildings. IoT enables collecting the latest conditions of historic buildings through various sensors and other devices. Ontology provides a consistent schema for representing physical entities in historic buildings, such as spaces and assets. Subsequent analytics can be performed using historical and real-time data streams acquired from historic buildings.
\item Presented a reference implementation using hardware, open-source software libraries, and the public cloud, i.e., Microsoft Azure, to reduce reinvention and make it more easily reproduced and reused in other historic buildings. The use of public cloud services also eases the challenge of dealing with a large volume of collected data since preserving a historic building is a long-term process. Furthermore, the reference implementation can be packaged as software as a service (SaaS), which eases the delivery of applications and be transferred to other historic buildings.
\item Validated the implementation by conducting a practical case study in the City Theatre, Norrk\"oping, Sweden. The City Theatre is a representative of a class of historic buildings with large open interior spaces, and activities held in such buildings bring together many people in the same place over a period of time. The case study demonstrated the functionalities and benefits of the created DT.
\end{itemize}

The remainder of this paper is structured as follows. After a discussion of related work in Section~\ref{sec:enabling_related_work}, the detailed design of the solution is described in Section~\ref{sec:enabling_system_design}. Then, a reference implementation, including used hardware, software, and public cloud services, is given in Section~\ref{sec:enabling_system_impl}. After that, a description of the case study building and the data analysis method is given in Section~\ref{sec:enabling_case_study}. Section~\ref{sec:enabling_results_discussion} presents and discusses the obtained results. The last section concludes the paper.

\section{Related Work}
\label{sec:enabling_related_work}

The reviewed studies in this section focus on the contents of preventive conservation of historic buildings, the background of digital transformation, the concept of DT, the application of DT in different fields, including the built environment, as well as solutions provided by cloud and industrial vendors for creating DTs.

Preventive conservation concentrates on distinct aspects for different types of historic buildings. For historic buildings having interior spaces, e.g., exhibition rooms, keeping an appropriate indoor environment is important~\cite{ashrae_handbook_hvac_applications_2011}. Improper environmental conditions, such as temperature and RH, might harm buildings and collections. For example, high RH levels that are greater than 75\% under 20~\textdegree{}C promote the growth of fungi on surfaces and chemical deterioration in most organic materials~\cite{ashrae_handbook_hvac_applications_2011}. Large fluctuations in temperature or RH could cause physical damage to materials~\cite{en_15757_conservation_2010}. Beyond thermal conditions, good air quality is also necessary for occupants like staff and visitors. Most occupants will be satisfied with a steady-state carbon dioxide (CO\textsubscript{2}) concentration under 1,200 parts per million (ppm)~\cite{ansi_ashrae_621_ventilation_2016}. For historic buildings where optimizing environmental factors is difficult, e.g., monuments, Van Balen~\cite{balen_preventive_2015} claimed that it is more concerned with responding quickly to urgent activities like disasters. In addition to managing threats, Lucchi~\cite{lucchi_review_2018} identified another major area of preventive conservation, i.e., energy modeling of historic buildings. Energy modeling aims to improve the energy efficiency of historic buildings to reduce costs. All these conservation studies could benefit from a deeper understanding of the operating conditions of historic buildings.

Digital transformation aims to integrate information and communication technologies (ICTs) to improve an entity by causing considerable changes to its attributes~\cite{vial_understanding_2019}. IoT and cloud computing are two representative technologies that significantly promote digital transformation~\cite{liu_methodology_2021}. The integration of IoT and cloud computing could benefit from both the data gathering capability of IoT and the data storage and processing capability of cloud computing~\cite{zhu_novel_2014}. A lot of data have been accumulated during the digital transformation and conservation of historic buildings. However, the organization of data is more complex than collecting data~\cite{noor_modeling_2019}. The complexity is due to a large amount of data and the heterogeneity of the sources. The data originates from analytical studies, surveys, diagnostics, and monitoring and must be continuously updated during performance assessment, planning, and execution~\cite{bruno_historic_2018}. The validity of data can also be an issue. Anomaly in data should be detected~\cite{liu_anomaly_2020} and determined to be data source errors, such as sensor failure, or indicative of abnormal status in a building. Therefore, it is challenging to effectively organize the collected data during the digital transformation of historic buildings.

Although the precise concept of DTs varies among scholars, most people believe that a DT represents a physical entity~\cite{grieves_digital_2014,glaessgen_digital_2012}. Furthermore, a DT must evolve to reflect the changes of its physical counterpart~\cite{shahzad_digital_2022}. Thus, creating a DT of a physical object is useful when the physical object changes over time~\cite{wright_tell_2020}. DTs have been applied in various sectors, such as manufacturing~\cite{tao_digital_shop_2017}, aerospace~\cite{glaessgen_digital_2012}, energy~\cite{bp_twin_2018}, and healthcare~\cite{liu_novel_2019}. The built environment research community has various views on the capabilities that a DT must offer. Boje et al.~\cite{boje_towards_2020} believed that a DT's ability to actuate real-world activities, whether proactive or reactive, in response to environmental changes is crucial. Jiang et al.~\cite{jiang_digital_2021} considered that whereas a DT necessitates data transfer from the physical entity to the virtual entity, feedback is not required. Also, the virtual entity can control its physical counterpart, but this is not required. We believe that the ultimate form of a DT in the built environment must include direct interactions from virtual to physical space. However, in practical application, a DT can gradually evolve, e.g., starting from effective monitoring to real-time data analysis, and finally including automatic control.

Within studies on modeling historic buildings, a concept usually confused with DT is historic building information modeling (HBIM). Although both DT and HBIM necessitate using a virtual model to represent a physical entity~\cite{jiang_digital_2021}, there are some differences between them. First, while 3D geometric models, often obtained from 3D point clouds by laser scanning and photogrammetry~\cite{yang_review_2020}, are typically used in HBIM, they are not necessarily required for DTs~\cite{delgado_digital_2021}. Second, the dataset in HBIM is often static. The information update for such a dataset is usually manually carried out by professional operators, resulting in a loss of temporal correlation~\cite{rosati_air_2020}. However, DT is constantly updated~\cite{delgado_digital_2021} which accurately reflects the current state of its physical counterpart~\cite{jiang_digital_2021}. Last, the application of DT is more focused on extracting useful information from data. By analyzing historical and real-time data acquired from the physical entity, a DT enables preventive maintenance, performing what-if analysis, and simulations~\cite{glaessgen_digital_2012}. Therefore, while HBIM is appropriate for modeling, managing, and restoring historic buildings by utilizing reality-based recording data~\cite{yang_review_2020}, DT is suitable for preventive conservation of historic buildings.

Several studies have applied DTs to the built environment. Khajavi et al.~\cite{khajavi_digital_2019} recommended combining three necessary components to construct the DT of a building: data components from existing building information modeling (BIM), WSN, and data integration as well as analytics. Lu et al.~\cite{lu_developing_2020} proposed a hierarchical architecture for creating DTs at the building and city levels and demonstrated the benefits of anomaly detection service in managing the health of building assets. Angjeliu et al.~\cite{angjeliu_development_2020} created a DT model of a historic masonry building by integrating data such as geometry, visual observation, construction process, and material properties. The DT model is calibrated with the dynamic measurements and utilized to investigate the structural reaction of the system or for activities connected to planned preventive maintenance. Zhang et al.~\cite{zhang_automatic_2022} presented an approach based on DT for optimizing relative humidity in underground heritage sites. The own developed web-based DT platform uses IoT technology to control the ventilation system automatically. However, the solutions proposed in these studies to create DTs are difficult to generalize to other historic buildings due to the lack of a consistent, reusable, and extendable data format to represent buildings.

Representing a building aims to conceptualize the whole building or selected parts of a building. The conceptualization contains the objects, concepts, and other entities that are presumptively present in the interesting area, together with the relationships among them~\cite{gruber_toward_1995}. An ontology provides explicit data format of a conceptualization~\cite{acierno_architectural_2017}. Some studies have been reported to address the demand for consistent data format. Balaji et al.~\cite{balaji_brick_2018} proposed a standardized metadata schema called Brick for representing buildings. The schema defines a concrete ontology for sensors, subsystems, and their relationships, enabling the development of applications. Hammar et al.~\cite{hammar_realestatecore_2019} developed an ontology, namely RealEstateCore, to help property owners to describe the data of interaction within the buildings as well as the management, storage, and exchange of these data. Digital Twins Definition Language (DTDL)~\cite{azure_dtdl_2022} is a language for specifying DT models. DTDL is built on a JavaScript Object Notation (JSON) variation known as JSON-LD that is intended to be usable as JSON and in Resource Description Framework (RDF) systems. While DTDL allows users to generate models of any entity from scratch, it is preferable to use DTDL in conjunction with existing domain knowledge.

To reduce reinvention and accelerate the application of DTs, several public cloud and industrial vendors have provided services or software for creating DTs. Some services, e.g., Microsoft Azure Digital Twins~\cite{azure_digital_twins_2022} and Amazon Web Services (AWS) IoT TwinMaker~\cite{aws_iot_twinmaker_2022}, are for general purposes. Others, such as Google Cloud Digital Supply Chain~\cite{google_supply_chain_twin_2022}, Siemens Intosite~\cite{siemens_intosite_2022}, and General Electric (GE) Digital Twin~\cite{ge_dt_software_2022}, are industry-specific. There are also a few open-source DT frameworks like Eclipse Ditto~\cite{eclipse_ditto_2022}. Although these tools do not provide out-of-the-box solutions for creating DTs of historic buildings, some of them could be leveraged to a certain extent to reduce duplication efforts.

Based on those backgrounds, this paper describes our work on applying DT to the preventive conservation of historic buildings. While earlier modeling work documented historic buildings through 3D geometry models, we created parametric DT through ontology. Using ontology also paves the challenge of lacking a consistent data format to represent historic buildings in previous studies. Further, we provided a reference implementation by reusing and extending the RealEstateCore ontology as well as utilizing open-source software libraries and Microsoft Azure services. Although these digital technologies exist, they are not dedicated to preserving historic buildings. The focus of this study is to provide a methodology for using these technologies to facilitate preserving historic buildings. For example, although Microsoft Azure Digital Twins allows users to generate models of any entity from scratch, it does not provide a domain-specific data format for representing historic buildings. We need to combine it with existing domain knowledge to mitigate reinvention. The RealEstateCore ontology provides some domain knowledge to represent building components and subsystems, but we still need to extend it to make it suitable for the application scenario of preserving historic buildings. Furthermore, we do not bind our methodology to Microsoft Azure. Services provided by other cloud vendors may be used to implement this solution. The cloud-based nature also allows our implementation to be packaged as SaaS, making it easy to deliver various applications and scale to accommodate more needs when promoted to more historic buildings. These efforts make our solution more reproducible for other researchers to reuse in their work adaptly.

\section{System Design}
\label{sec:enabling_system_design}

This section presents the overall design of the solution. First, the main modules and their functions are outlined. Then, the detailed architecture is given.

\subsection{Overview}

As shown in Fig.~\ref{fig:enabling_fig1}, the solution involves four main modules, namely physical entities, virtual models, data warehouse, and functional services, as well as connections, i.e., interaction and synchronization, between the modules.

\begin{figure}[!ht]
\includegraphics{figures/enabling/fig1.png}
\centering
\caption{An overview of main modules in the proposed solution.}\label{fig:enabling_fig1}
\end{figure}

\subsubsection{Physical Entities}
Physical entities are real-world objects. An object could be a space or an asset in space. Space ranges from a whole historic building or specific areas inside a building, such as a sub-building, a floor, or a specific room. Assets are those objects located in a historic building but are not a part of the structure. Furniture, housed collections, and infrastructures such as electric power, water, lighting, and heating, ventilation, and air-conditioning (HVAC) systems are examples of assets.

The purpose of the application determines the physical entities that need to be modeled. When it comes to preserving collections in an exhibition room, the physical entities could be the indoor environment of the room. When energy optimization is desired for historic buildings, the physical entities could be energy-consuming equipment and the areas they serve.

\subsubsection{Virtual Models}
Virtual models are digital representations of physical entities. Such representations aim to extract, define, and characterize essential attributes and behaviors of physical entities. Any model that sufficiently accurately depicts the physical entities can be used to create digital twins. This study proposes to build virtual models on a standardized metadata schema that establishes a concrete ontology for spaces, assets, and their relationships.

Besides providing a complete physical and functional description of interested physical entities, virtual models should be able to receive input and evolve with the status changes of modeled physical entities. Virtual models should also provide interfaces for other modules to notify model changes and retrieve model data. In this way, virtual models contain the necessary information for performing specific subsequent tasks to enable the development of portable applications.

\subsubsection{Data Warehouse}
The data warehouse entails defining data structures, operating procedures, and data storage. Operating status, model definitions, and alert rules are examples of data related to physical entities. Operating status refers to past and current situations of physical entities, such as indoor environment and energy consumption. Model definitions include virtual models that depict physical entities and data analysis models that try to extract insights from data. Alert rules describe which preventative conservation actions are taken when certain conditions are met.

Because preserving historic buildings is a long-term process, evolving data related to the physical entities will accumulate. The data warehouse should be capable of handling, processing, and analyzing large monitoring datasets to extract useful information for practical use.

\subsubsection{Functional Services}
Functional services aim to assist users in achieving smart maintenance of historic buildings. This goal is accomplished by integrating and analyzing data from various sources. There are three categories of functional services:
\begin{itemize}
\item Monitoring entails visualizing historical and real-time operating status data to help users keep track of events and behaviors.
\item Analytics uses methods like exploratory data analysis and machine learning to extract valuable insights from data obtained from historic buildings.
\item Decision-making focuses on using the retrieved beneficial insights to guide actions for smart maintenance, such as assessing current situations and diagnosing previous issues. Decision-making also includes notifying the facility managers when maintenance is necessary, or a subsystem fails through pre-defined alert rules.
\end{itemize}

\subsubsection{Interaction and Synchronization}
Interactions and synchronizations are connections between modules that allow data and commands to be shared. Synchronizations focus on data, while interactions focus on commands. Examples of synchronizations are:
\begin{itemize}
\item Physical entities--Data warehouse: the latest status of physical entities is stored in the data warehouse on time.
\item Virtual models--Data warehouse: virtual models obtain the stored latest status from the data warehouse to evolve and reflect the changes of their physical counterparts.
\end{itemize}

Also, examples of interactions are:
\begin{itemize}
\item Physical entities--Virtual models: by operating virtual models, the corresponding commands are issued to control the associated physical counterparts to accomplish in-time adjustment or optimization.
\item Virtual models--Functional services: functional services search the virtual models to obtain information about the digital twins based on their properties, models, and relationships.
\item Data warehouse--Functional services: functional services create queries that locate relevant resources in a building. Then, a functional service adjusts its behavior or applies an anomaly detection algorithm to the collection of retrieved resources.
\end{itemize}

\subsection{Architecture}

Fig.~\ref{fig:enabling_fig2} depicts the architecture. The architecture has two parts: the local part and the cloud part.

\begin{figure*}[!htb]
\includegraphics[width=\textwidth]{figures/enabling/fig2.png}
\centering
\caption{The architecture of the proposed solution.}\label{fig:enabling_fig2}
\end{figure*}

\subsubsection{The Local Part}

The local part consists of the edge platform and devices that retrieve information from historic buildings. The devices are the data sources of the entire system. According to their functions, they are divided into three groups: 
\begin{itemize}
\item Sensors and collectors: sensors measure interested parameters in historic buildings, such as temperature and RH. Collectors obtain measurements from the sensors. 
\item Actuators and controllers: actuators refer to the equipment in the historic building that can be controlled, such as fans and heaters. Controllers send control signals to these equipment and read the operating status from them.
\item Other systems and brokers: other systems refer to existing systems, e.g., the building management system (BMS), in a historic building. Brokers help retrieve information from such systems and forward commands to them.
\end{itemize}

An edge platform has certain storage, computing, and networking resources that serve two purposes. One is to act as a gateway so that the data from local devices can be reported to the cloud platform and receive control commands issued from the cloud platform. The other is to store and process data locally, such as taking over part of the artificial intelligence (AI) and analytics workload offloaded from the cloud platform, which is helpful for sensitive data or critical applications that require high real-time performance. Because the data does not need to be uploaded to the cloud platform, it can be processed locally in time. 

The edge platform can communicate with devices, i.e., collector, controller, and broker, through wired or wireless networks.

\subsubsection{The Cloud Part}

\textbf{Cloud gateway:}
In the cloud part, the cloud gateway is the entry. The cloud gateway manages local edge platforms and enables bi-directional communication between the cloud services and the edge. For example, when receiving a message from an edge, the cloud gateway notifies the downstream components to consume the message, such as updating the status of DT models and storing data.

\textbf{Digital twin models:}
The digital twin models are built on ontology. Ontology provides a consistent data representation to store metadata of physical entities and capture all significant relationships between physical entities. Ontology-based digital twin models provide machine-readable data formats and querying tools, allowing other modules to reason about the semantics of the data.

\textbf{Storage:}
Storage includes databases for storing structured and unstructured data. Other modules can write or read databases through application programming interfaces (APIs) provided by storage. Structured data include telemetries collected by sensors, the status of equipment, or other organized data. Unstructured data include texts and images. Texts may be a maintenance guide for equipment or collections. Images may be photographs of collections taken periodically, such as paintings and sculptures, to see how their surfaces have deteriorated.

\textbf{Insights:}
Based on historical and real-time data, we can do a series of data analytics to discover insights from data. Data analytics usually start with exploratory data analysis (EDA). EDA is a method that uses various techniques (mostly graphical) to maximize insight into a data set~\cite{guthrie_nistsematech}. Based on the understandings obtained from EDA, appropriate machine learning (ML) algorithms can be selected to build predictive models to perform functions such as anomaly detection and energy prediction. After these predictive models are trained and validated, they can be deployed for performing streaming data analysis.

\textbf{Applications:}
The ultimate goal of the system is to provide applications for preventive conservation. Applications can take many forms, including Web Apps, REST APIs, and Streaming APIs. The Web App can be a visualization application of data and models or an interactive simulation application such as energy prediction and occupancy prediction. An API is a contract between our system and information users. For example, the API designed for an indoor environment service could specify that the user supplies a building identity (ID) and a room ID. Our system replies with two indoor environmental conditions, the first being the temperature and the second being the relative humidity.

\section{System Implementation}
\label{sec:enabling_system_impl}

Our developed implementation is an entire IoT system for data collection with multiple sensors, data communication with an edge platform, data storage with the Microsoft Azure cloud, and the creation of DTs of historic buildings with ontology. This implementation emphasizes modeling the indoor environment to provide a deeper understanding of the operating conditions of historic buildings. The implementation does not include detecting other factors, such as pest infestation, natural disasters, theft, and vandalism, that might cause damage to historic buildings and housed collections. We have also reserved interfaces for further expansion, e.g., connecting equipment in historic buildings to exchange operation status and control commands.

\subsection{The Local Part}
\label{sec:enabling_the_local_part_impl}

The used hardware, including sensors, collector, and edge platform, is depicted in Fig.~\ref{fig:enabling_fig3}.

\begin{figure}[!ht]
\includegraphics{figures/enabling/fig3.png}
\centering
\caption{Used hardware and connections between them. The arrows indicate the direction of sensor data flow.}\label{fig:enabling_fig3}
\end{figure}

\subsubsection{Sensors}
\label{sec:enabling_impl_sensors}

Five sensing devices are used for measuring six indoor environmental parameters.
\begin{itemize}
\item DHT22 (Seeed Technology, Shenzhen, CHN) measures temperature and RH.
\item MH-Z16 (Winsen Electronics Technology, Zhengzhou, CHN) measures CO\textsubscript{2} concentration.
\item PPD42NS (Shinyei Corporation, New York, NY, USA) detects pieces (pcs) of particulate matter (PM) with a diameter greater than 1~$\mu$m.
\item MIKOE-1630 (MikroElektronika, Beograd, SRB) detects several gases that affect air quality, such as ammonia (NH\textsubscript{3}), nitrogen oxides (NO\textsubscript{x}), benzene, and CO\textsubscript{2}.
\item The Grove-Piezo sensor (Seeed Technology, Shenzhen, CHN) measures flexibility, vibration, impact, and touch.
\end{itemize}

All sensing devices have been calibrated before being deployed in the case study building. Among the five sensing devices, DHT22 and the Grove-Piezo sensor were calibrated by ourselves. The other three sensing devices, i.e., MH-Z16, PPD42NS, and MIKOE-1630, were calibrated by the manufacturers. In addition, all sensing devices have undergone continuous operational testing that lasts for two weeks in a test room before deployment.
 
\subsubsection{Collector}
An Arduino Uno Rev3 SMD (Arduino, Somerville, MA, USA) together with a Grove Base Shield V2 (Seeed Technology, Shenzhen, CHN) is used as collector. The collector has abundant interfaces, including an SPI connection, a UART connection, six analog input/output (IO) pins, and 14 digital IO pins. These interfaces enable the collector to obtain readings from sensors and communicate with the edge platform. A 16-bit cyclic redundancy check (CRC) is used to detect errors during data transmission between the collector and the edge platform.

\subsubsection{Edge Platform}

The edge platform includes a computing module, i.e., Raspberry Pi CM3+ Dev Kit, and a network module, i.e., ZTE MF833V. The used Raspberry Pi CM3+ Dev Kit (Raspberry Pi Foundation, Cambridge, GBR) has 1~GB RAM and 32~GB flash storage, as well as a processor with a clock speed of 1.2~GHz. The ZTE MF833V (ZTE, Shenzhen, CHN) is a 4G USB modem that allows users to connect to mobile broadband. The download speed for the specific 4G network is up to 150~Mbps, and the upload speed is up to 50~Mbps.

\subsection{The Cloud Part}
The cloud part processes the collected data in real-time, including data visualization and system health monitoring. We have also reserved interfaces to integrate machine learning and streaming analytics to detect anomalies from the six environmental data in real-time.

As shown in Fig.~\ref{fig:enabling_fig4}, several cloud services provided by Microsoft Azure are used to implement the cloud part. The scale tiers, key specifications, and costs of used services can be seen in Table~\ref{tab:enabling_tab1} of Appendix~\ref{apdx:summary}. For each used Azure service, the scale tier was determined by present needs. These services also support scale-up to fulfill future research needs.

\begin{figure}[!ht]
\includegraphics{figures/enabling/fig4.png}
\centering
\caption{Used Azure services to implement the cloud part.}\label{fig:enabling_fig4}
\end{figure}

\subsubsection{IoT Hub}
Azure IoT Hub~\cite{azure_iothub_2021} is a cloud-based managing service that acts as a central messaging hub for enabling communication between an IoT application and its linked IoT devices. IoT Hub serves as the cloud gateway.
 
\subsubsection{Functions}
Azure Functions~\cite{azure_functions_2021} is a cloud service that provides users with event-driven serverless computing. This study uses Azure Functions to transfer messages between different cloud modules, such as updating status of digital twin models and writing data to databases.
 
\subsubsection{Digital Twins}
Azure Digital Twins~\cite{azure_digital_twins_2022} is adopted to deploy DTs. The DT models of historic buildings are defined by using DTDL~\cite{azure_dtdl_2022} and the RealEstateCore ontology~\cite{dtdl_realestatecore_2022}. As shown in Fig.~\ref{fig:enabling_fig5}, the RealEstateCore ontology has three major classes: \textit{Space}, \textit{Asset}, and \textit{Capability}. We reused the definitions of subclasses under the Space category. We extended several subclasses under the Asset and Capability categories to represent used hardware as well as their capabilities.

\begin{figure}[!ht]
\includegraphics{figures/enabling/fig5.png}
\centering
\caption{Main classes and relationships of our extended ontology based on RealEstateCore.}\label{fig:enabling_fig5}
\end{figure}

\subsubsection{SQL Database and Blob Storage}
Azure SQL Database~\cite{azure_sql_database_2021} and Blob Storage~\cite{azure_blob_storage_2021} are utilized to provide storage resources. Azure SQL Database stores structured data, such as all collected sensor data. Blob Storage stores unstructured data, for example, the definitions of DT models.

\subsubsection{Web Apps}
Azure Web App Service~\cite{azure_web_app_2021} is used to host a web App called Minerva (see~\url{https://historicbuildings.azurewebsites.net}). We developed the Minerva by using a low-code open-source framework, i.e., Dash Plotly~\cite{dash_plotly_2021} and a Bootstrap component package, namely Dash Bootstrap Components~\cite{dash_bootstrap_2022}. The Minerva user interface supports visualizing real-time and historically collected data as well as sharing these data.

\section{Case Study}
\label{sec:enabling_case_study}

This section presents a practical application of the implemented system in a historic building. First, a brief description of the historic building is provided. Then, the deployment of local devices is introduced. After that, the data analysis method is given. The results, including created DT and its main functions, the impact of the occupants on the indoor environment, and fluctuation analysis of RH, are given in Section~\ref{sec:enabling_results_discussion}.

\subsection{Description of the City Theatre}

The City Theatre (see Fig.~\ref{fig:enabling_fig6}) is located in the city center of Norrk\"oping, Sweden. The building was erected in 1908 in the Art Nouveau style. Since 1990, the City Theatre has been listed as a protected building under the national historic legislation. Now, the building is used as a platform for performing shows that reflect current society. The building has a salon room (see Fig.~\ref{fig:enabling_fig7}) with a seating capacity of 600 persons. Before the COVID-19 pandemic, in each year of 2018 and 2019, there were more than 50 shows performed, attracting over 13,000 audiences.

\begin{figure}[!ht]
\includegraphics{figures/enabling/fig6.png}
\centering
\caption{Fa\c{c}ade of the City Theatre in Norrk\"oping, Sweden.}\label{fig:enabling_fig6}
\end{figure}

\begin{figure}[!ht]
\includegraphics{figures/enabling/fig7.png}
\centering
\caption{The salon room of the City Theatre. The yellow star marked the position of a deployed sensor box with both sensors and the edge platform. This figure is used with permission from the photographer Markus G{\aa}rder.}\label{fig:enabling_fig7}
\end{figure}

A case study in the City Theatre could be a good inspiration for the digital transformation of similar historic buildings, e.g., theatres and churches, that have large open interior spaces and draw many people to the same place for some time during activities.

\subsection{Deployment of the Local Devices}

To collect environmental conditions that are close to the average values of the seating area in the salon room, a sensor box (see Fig.~\ref{fig:enabling_fig8}) is deployed under the fence of the second floor of the grandstand, which is near the spatial center of the salon (see Fig.~\ref{fig:enabling_fig7}). The sensor box is a plastic box that packages an edge platform, a collector and five sensors as described in Section~\ref{sec:enabling_the_local_part_impl}. The data collection started from March 16, 2021, and will last at least by the end of 2023. All the six environmental parameters, i.e., temperature, RH, CO\textsubscript{2} concentration, dust concentration, harmful gas concentration, and vibration, are collected every 15~s. Undoubtedly, deploying more sensor boxes can provide a better understanding of the spatial distribution of environmental parameters. However, the location where the sensor box is deployed in this paper is representative, and the collected environmental data are supposed to approximate the average values of the seating area. In addition, the methodology to create DT models and the data analysis method (see Section~\ref{sec:enabling_analysis_method}) are also applicable when more sensor boxes are deployed.

\begin{figure}[!ht]
\includegraphics{figures/enabling/fig8.png}
\centering
\caption{The deployed sensor box in the salon room of the City Theatre.}\label{fig:enabling_fig8}
\end{figure}

\subsection{Data Analysis Method}
\label{sec:enabling_analysis_method}

The data analysis in this study serves two purposes. One is to investigate the impact of occupants on the indoor environment when shows are performed in the City Theatre and the relationship between changes in different environmental parameters. Another is to inspect the fluctuations in indoor relative humidity throughout the whole calendar year to see if any risks may harm conservation.

After preliminary observations of collected data, we found that the data were sampled much faster than the expected need, i.e., fast enough to catch any changes in real-time. Therefore, we downsampled the data before further data analysis. After removing invalid data, the original data, collected every 15~s, were downsampled by taking an average value of measurements every five minutes. Due to occasional network or power issues, some readings ($<$~2\%) were lost during transmission. Therefore, after downsampling, missing values are filled in using the nearest previous value. All subsequent times are presented in the 24-hour system and in local time (Greenwich Mean Time (GMT) +1 for summer time and GMT +2 for winter time). All shows performed in the City Theatre (from September 2021 and February 2022) lasted over two hours.

\subsubsection{The Impact of Occupants on Indoor Environment}

The analysis of the impact of occupants on the indoor environment is carried out by combining exploratory data analysis (EDA) and classical statistical analysis. EDA is adopted to observe and compare the changes in the indoor environment before and during shows, as well as analyze what factors cause these changes. The classical statistical analysis focuses on quantitatively studying the impact of different occupancy levels on the indoor environment.

To quantitatively study the impact of different occupancy levels on temperature, as shown in Fig.~\ref{fig:enabling_fig9}, we use the show start time as the boundary to determine two equal periods, namely \textit{before the show} and \textit{during the show}, each has a two-hour duration. Then we use the average value of measurements during these two periods as their representative value, respectively. The difference between these two average values is the change brought by occupants. We denoted average temperature during the period of \textit{before the show} as $T_{before}$ and denoted average temperature during the period of \textit{during the show} as $T_{during}$, then the change of temperature is calculated as $T_{during} - T_{before}$, and is denoted as $\Delta{T}$.

\begin{figure}[!ht]
\includegraphics{figures/enabling/fig9.png}
\centering
\caption{Determination of two periods: \textit{before the show} and \textit{during the show}.}\label{fig:enabling_fig9}
\end{figure}

All days were chosen between September 2021 and February 2022 (during the season with heating) to mitigate the impact of outdoor weather and obtain a relatively consistent indoor temperature. The number of days with shows is three times the number of days without shows. This ratio ensures the equality of group size after splitting days with shows to three groups with different occupancy levels. When selecting days without shows, the distribution is considered by days in each month and the ratio of weekdays versus weekends. Then, among days with shows, occupancy levels are divided into three groups, namely \textit{High}, \textit{Medium}, and \textit{Low}. A control group called \textit{Zero} is determined by picking days without shows at the same time period. For the \textit{Zero} group, the changes represent natural changes that could act as a baseline. In contrast, for the other three groups with occupants, the changes are brought by the combined effect of occupants and the operation of HVAC systems. Hence, we have totally four groups corresponding to four occupancy levels.

In this study, we have one independent categorical variable, i.e., the occupancy level, and one dependent continuous variable, i.e., $\Delta{T}$. To determine whether there are any statistically significant differences between the means of $\Delta{T}$ in the four groups of occupancy levels, we conduct a one-way analysis of variance (ANOVA). This could reveal whether different occupancy levels could result in different temperature changes. For one-way ANOVA, the null hypothesis $H_{0}$ is that there is no difference among group means. i.e., $\mu_{1} = \mu_{2} = \mu_{3} = \mu_{4}$, where $\mu_{k}$ denotes the mean value of $\Delta{T}$ in group $k$. The alternative hypothesis $H_{1}$ is that the means are not all equal. The significance level is set as 0.05.

Four Python libraries, namely SciPy (v1.8.0), Pingouin (v0.5.1), scikit-posthocs (v0.6.7), and statsmodels (v0.13.2), were used for conducting the statistical analysis.

\subsubsection{Fluctuation Analysis of Relative Humidity}

The approach proposed in the European standard EN 15757:2010~\cite{en_15757_conservation_2010} is used to inspect the fluctuation of RH. Three statistics, i.e., yearly average level, seasonal cycle, and fluctuation, characterize indoor RH. The yearly average level is calculated as the arithmetic mean of the RH readings during a whole calendar year. The seasonal cycle is determined by computing the centered moving average (CMA) for each reading, which is the arithmetic mean of all RH readings collected in 30 days consisting of 15 days before and 15 days after the average is computed. A fluctuation is calculated as a current RH reading minus the 30-day CMA determined for that reading.

The $7$th and $93$rd percentiles of the fluctuations recorded during the monitoring period are used to determine the lower and upper bounds of the safe band of RH variations. If the $7$th and $93$rd percentiles are less than 10\%, a 10\% RH deviation from the seasonal RH level can be accepted~\cite{en_15757_conservation_2010}. 

\section{Results and Discussion}
\label{sec:enabling_results_discussion}

This section summarizes obtained results and findings. First, the created DT and its main functions are presented. Then, the impact of occupants on the indoor environment is shown. Finally, the fluctuation of RH in the City Theatre is analyzed.

\subsection{The Created Digital Twin}

A limited parametric DT of the City Theatre is created with the locally deployed sensor box. Fig.~\ref{fig:enabling_fig10} shows the twin graph of the created DT. In the twin graph, the circular nodes represent virtual models of physical objects. The arrows indicate relationships between virtual models. The virtual models and relationships correspond one-to-one with physical objects and relationships in the real world. For example, the top node \textit{The City Theatre} corresponds to the entire building. It is followed by the node \textit{The salon room}. The relationship between the two nodes is called \textit{isPartOf}, i.e., the salon room is part of the City Theatre. The DT is open to extension and modification. When new physical objects need to be modeled, corresponding virtual models and relationships can be added to the twin graph. Existed virtual models can also be modified, e.g., adding more properties to model their physical counterparts more exactly.

\begin{figure}[!ht]
\includegraphics{figures/enabling/fig10.png}
\centering
\caption{The twin graph of the created digital twin (DT) of the City Theatre. (\textbf{a}) Temperature and humidity sensor, (\textbf{b}) CO\textsubscript{2} sensor, (\textbf{c}) dust sensor, (\textbf{d}) air quality sensor, (\textbf{e}) vibration sensor, (\textbf{f}) measuring temperature, (\textbf{g}) measuring relative humidity, (\textbf{h}) measuring CO\textsubscript{2} concentration, (\textbf{i}) measuring dust concentration, (\textbf{j}) measuring harmful gas concentration, and (\textbf{k}) measuring vibration.}\label{fig:enabling_fig10}
\end{figure}

\begin{figure}[!htb]
\includegraphics[width=3.3in]{figures/enabling/fig11.png}
\centering
\caption{The digital twin explorer to explore twin properties of virtual models.}\label{fig:enabling_fig11}
\end{figure}

Such a DT provides three capabilities. The first is that virtual models reflect the latest status of physical objects by fed sensor data collected in nearly real-time. Therefore, through exploring the properties of virtual models, users can obtain the current conditions of physical objects. Fig.~\ref{fig:enabling_fig11} illustrates such a use case: by clicking on the node representing the capability of measuring temperature, users can know the latest indoor temperature of the salon room.

The second is that the DT provides knowledge of a historic building. The twin graph can be searched to learn more about the virtual models and their relationships. These queries are written in a custom SQL-like query language. For instance, suppose several other rooms in the City Theatre have also been deployed the same sensor box as in the salon room. We may ask the DT to find out all rooms currently with CO\textsubscript{2} concentrations below 500 ppm through a query instruction as follows.

\begin{lstlisting}[language=SQL, basicstyle=\ttfamily\footnotesize]
SELECT Room
FROM DIGITALTWINS SensorEquipment
JOIN Sensor RELATED SensorEquipment.hasCapability
JOIN SensorBox RELATED SensorEquipment.isPartOf
JOIN Room RELATED SensorBox.locatedIn
JOIN Building RELATED Room.isPartOf
WHERE Building.$dtId IN ['TheCityTheatre']
AND
IS_OF_MODEL(Sensor,
  'dtmi:digitaltwins:rec_3_3:device:CO2Sensor;1')
AND IS_DEFINED(Sensor.lastValue)
AND Sensor.lastValue < 500
\end{lstlisting}

The third capability lies in collaborating with data analytics to uncover valuable insights from historical and real-time data to help optimize operations and achieve preventive conservation of historic buildings. The dashboard page of Minerva shown in Fig.~\ref{fig:enabling_fig12} presents the collected readings of six environmental parameters in a typical week. Some correlations can be found between changes in readings of different environmental parameters when there were human activities in the salon room. As depicted in Fig.~\ref{fig:enabling_fig12}{a} and Fig.~\ref{fig:enabling_fig12}{c}--{e}, five peaks can be found in each plot of temperature, CO\textsubscript{2}, dust, and harmful gas from October 6 to 10. Such drastic environmental changes are caused by shows performed on that five days. Also, as shown in Fig.~\ref{fig:enabling_fig12}{e}, an extra peak of harmful gas concentration can be found on October 4. We speculate that the existence of other harmful gases except CO\textsubscript{2} causes this peak because the air quality sensor MIKOE-1630 (see Section~\ref{sec:enabling_impl_sensors}) used in this study can detect the presence of various harmful gases, including CO\textsubscript{2}. However, there was no significant increase in CO\textsubscript{2} concentration (measured by the CO\textsubscript{2} sensor MH-Z16) on October 4. Such differences in concentrations of CO\textsubscript{2} and overall harmful gas might be used for developing an anomaly detection service in the DT in further work. It is worth mentioning that the plot of vibration readings (see Fig.~\ref{fig:enabling_fig12}{f}) shows a constant value because we have not yet determined the threshold of collected interruptions for distinguishing if there was a vibration. The threshold will be decided in future work. In the following subsection, the impact of occupants on the indoor environment is analyzed in detail.

\begin{figure}[!ht]
\includegraphics[width=\textwidth]{figures/enabling/fig12.png}
\centering
\caption{Historical indoor environment in the salon room of the City Theatre from October 4 to 10, 2021. For each environmental parameter, 24 data points (one every hour starting at 00:00) are shown per day. (\textbf{a}) Temperature, (\textbf{b}) relative humidity, (\textbf{c}) CO\textsubscript{2} concentration, (\textbf{d}) dust concentration, (\textbf{e}) harmful gas concentration, and (\textbf{f}) detected vibration.}\label{fig:enabling_fig12}
\end{figure}

\subsection{The Impact of Occupants on Indoor Environment}

When shows are performed in the salon room, the presence of audiences can affect the indoor environment. Fig.~\ref{fig:enabling_fig13} provides a typical example of such an impact. The show of the day started at 19:00 and ended around 21:20. As depicted in Fig.~\ref{fig:enabling_fig13}{a}, at around 19:00, as the audience entered the room, the temperature rose and reached the maximum value of 25.6~\textdegree{}C at around 19:30. After that, the temperature fluctuated around a relatively high value. After 20:00, the temperature went through a process of first falling and then rising. This change is attributed to a short break in the show. Some audiences left the salon for rest and then reentered the room. After the show ended, audiences left, and the temperature dropped to below 24~\textdegree{}C. A similar phenomenon can be found in changes of CO\textsubscript{2} concentration (see Fig.~\ref{fig:enabling_fig13}{c}). The change in relative humidity (see Fig.~\ref{fig:enabling_fig13}{b}) is a combination effect of moisture and temperature. Relative humidity fluctuated more during a show than when there is no audience.

\begin{figure}[!ht]
\includegraphics{figures/enabling/fig13.png}
\centering
\caption{Historical indoor environment of the salon room, from 12:00 to 23:59, October 7, 2021. (\textbf{a}) Temperature (T), (\textbf{b}) relative humidity (RH), (\textbf{c}) CO\textsubscript{2} concentration, and (\textbf{d}) dust concentration.}\label{fig:enabling_fig13}
\end{figure}

As seen in Fig.~\ref{fig:enabling_fig13}{d}, there were two time periods when the dust concentration fluctuated at a high level ($\sim$20,000 pcs/L). The first time period was shorter and took place between 17:00 and 18:00, i.e., before the show started, during which we believe that the actors and professionals were doing some pre-show preparation work in the salon room. The second time period was longer and lasted from the start of the show (around 19:00) to one hour after the show ended (around 22:20). High dust concentrations in both of the two periods are mainly due to the operation of the ventilation system, which enhances the mobility of air in the salon room, thereby stirring up small particles. The movement of air makes the environmental conditions relatively uniform, which indicates that data collected by one sensor box (see Fig.~\ref{fig:enabling_fig8}) are good enough to reflect the indoor environment of the salon room.

We can see that CO\textsubscript{2} concentration is more sensitive to indicate the presence of occupants compared with temperature and relative humidity. This is reflected in two aspects. One is the quick response. When comparing Figs.~\ref{fig:enabling_fig13}{a} and ~\ref{fig:enabling_fig13}{c}, we can find that some audiences had already entered the salon room before the show began, resulting in a quick rise in CO\textsubscript{2} concentration. However, there was some hysteresis in the temperature rise.

Another is that the difference in CO\textsubscript{2} concentration can reflect occupancy levels to a certain extent. More audiences lead to higher CO\textsubscript{2} concentrations. Fig.~\ref{fig:enabling_fig14} shows the daily maximum CO\textsubscript{2} concentration during a whole week, from October 4 (Monday) to October 10 (Sunday), 2021. We can find that CO\textsubscript{2} concentrations were below 500 ppm on Monday and Tuesday because no show was performed on that two days. From Wednesday to Sunday, each day had a show performed. The maximum CO\textsubscript{2} concentrations during these five shows all exceeded 900 ppm. On Saturday, the maximum CO\textsubscript{2} concentration even exceeded 1,200 ppm, which might cause discomfort to some audiences. Such difference in CO\textsubscript{2} concentrations between shows reflects differences in the number of audiences attending different shows. It is reasoned that the Saturday show drew the most audiences during that week. In addition, the authors suggest that when the number of audiences is large, the airflow of the ventilation system can be appropriately increased to ensure that the CO\textsubscript{2} concentration is lower than 1,200 ppm and hence guarantee human comfort of audiences.

\begin{figure}[!ht]
\includegraphics{figures/enabling/fig14.png}
\centering
\caption{Historical CO\textsubscript{2} concentration in the salon room of the City Theatre from October 4 (Monday) to 10 (Sunday), 2021.}\label{fig:enabling_fig14}
\end{figure}

Fig.~\ref{fig:enabling_fig15} shows the daily maximum CO\textsubscript{2} concentration in a full calendar year, which indicates the activities in the City Theatre throughout the year. When there was no show, CO\textsubscript{2} concentrations were often lower than 500 ppm. Due to the pandemic of COVID-19, there was no show in the City Theatre until September 2021. Moreover, in October, the City Theatre had more audiences. The occupancy information can be further explored in future work, such as using changes in indoor environmental parameters to estimate occupancy levels in historic buildings in real-time.

\begin{figure}[!ht]
\includegraphics[width=\textwidth]{figures/enabling/fig15.png}
\centering
\caption{Daily maximum CO\textsubscript{2} concentration in the salon room of the City Theatre from April 1, 2021 to March 31, 2022. Seven days of a week, from Monday to Sunday, are abbreviated as M, T, W, T, F, S, and S, respectively.}\label{fig:enabling_fig15}
\end{figure}

\begin{figure}[!ht]
\includegraphics{figures/enabling/fig16.png}
\centering
\caption{76 days between September 1, 2021, and February 28, 2022, are selected to quantitatively study the impact of different occupancy levels on temperature. Among the 76 days, 57 days with shows performed are divided into three groups of occupancy levels, i.e., \textit{High}, \textit{Medium}, and \textit{Low}, according to average CO\textsubscript{2} concentration during shows. The remaining 19 days without shows performed are used as the control group, namely \textit{Zero}.}\label{fig:enabling_fig16}
\end{figure}

The quantitative study of the temperature changes could support that CO\textsubscript{2} concentration reflects occupancy levels. We used the average CO\textsubscript{2} concentration during the period of \textit{during the show} to determine the group of different occupancy levels. Then we investigate if there is a statistically significant difference in $\Delta{T}$ among different occupancy level groups. The days in each group are shown in Fig.~\ref{fig:enabling_fig16}. A lowercase $n$ represents the number of $\Delta{T}$ data points in an occupancy group. Data of $\Delta{T}$ is presented as mean $\pm$ standard deviation. $\Delta{T}$ increased from the \textit{Zero} ($n$ = 19, 0.02 $\pm$ 0.26~\textdegree{}C), to \textit{Low} ($n$ = 19, 0.59 $\pm$ 0.25~\textdegree{}C), to \textit{Medium} ($n$ = 19, 1.00 $\pm$ 0.29~\textdegree{}C) and to \textit{High} ($n$ = 19, 1.72 $\pm$ 0.46~\textdegree{}C) occupancy groups.

To Determine if the data have outliers, the boxplot (see Fig.~\ref{fig:enabling_fig17}) for $\Delta{T}$ for each occupancy level was used. Any data points that are more than 1.5 box lengths from the edge of their box are classified as outliers, illustrated as diamond dots. There was no outlier in the data of $\Delta{T}$ as assessed by inspection of the boxplot.

\begin{figure}[!ht]
\includegraphics{figures/enabling/fig17.png}
\centering
\caption{The boxplot of changes in temperature ($\Delta{T}$) of the four occupancy groups.}\label{fig:enabling_fig17}
\end{figure}

The Shapiro-Wilk test was conducted to test the normality of the data of $\Delta{T}$. Four tests were run, one for the dependent variable $\Delta{T}$ in each group. The data of $\Delta{T}$ were normally distributed for each occupancy level, as assessed by Shapiro-Wilk's test ($p$ $>$ .05). The assumption of homogeneity of variances was violated, as assessed by Levene's test for equality of variances ($p$ $<$ .05). This means that the standard one-way ANOVA is not applicable in this case. A modified version of the ANOVA, i.e., Welch's ANOVA, is used. $\Delta{T}$ was statistically significantly different for different occupancy level groups, Welch's F(3, 39.421) = 77.253, $p$ $<$ .001.

Therefore, the statistically significant difference in $\Delta{T}$ confirms that CO\textsubscript{2} could reflect occupancy levels. Consequently, for historic buildings like the City Theatre, the indoor CO\textsubscript{2} concentration might be used to estimate occupancy levels and thus adaptively make conservation decisions. For example, since a higher occupancy level leads to higher internal heat gain, it is recommended to make a more efficient heating decision like adaptive heating. Through adaptive heating, the heating system of the case study building or similar historic buildings is controlled based on occupancy levels. Hence, one goal of preventive conservation, i.e., saving energy, could be achieved.

\subsection{Fluctuation Analysis of Relative Humidity}

The yearly mean value of RH was 32.1\%. The $7$th diff is -7.0\% while $93$rd diff is 6.9\%. Since the absolute values of both $7$th and $93$rd are lower than 10\%, a 10\% deviation from the 30-day CMA level is adopted as upper and lower bounds of the safe band. The measured values (see Fig.~\ref{fig:enabling_fig18}) show that the RH is higher in summer months and lower in winter months. Also, in summer months, the RH fluctuated more, and more risky data points were measured than in winter months. The authors suggest that this is mainly due to indoor heating. In winter, the temperature and RH are better maintained due to the working of the heating system.

The authors propose that some proactive interventions could be done during the summer months to reduce fluctuations in RH and thus achieve better heritage conservation. It is recommended to cycle on the ventilation system during the summer months, even when the salon room is not occupied, to lower RH and mitigate its fluctuations. It is also suitable to add a dehumidifier for better controlling the RH.

\begin{figure}[!hbt]
\includegraphics{figures/enabling/fig18.png}
\centering
\caption{A full calendar year of historical relative humidity (RH) measured in the salon room of the City Theatre from April 1, 2021 to March 31, 2022. A seasonal RH cycle is obtained by calculating the 30-day centered moving average (CMA) of RH readings. Safe band is determined by 10\% apart from the 30-day CMA.}\label{fig:enabling_fig18}
\end{figure}

\section{Conclusion}
\label{sec:enabling_conclusion}

This study aimed to facilitate the preventive conservation of historic buildings by integrating digitalization techniques to create digital twins. A solution was proposed by combing Internet of Things and ontology to consistently represent the data in historic buildings, reflect the latest operating status of historic buildings, and enable further data analysis. An implementation was provided to verify the proposed solution. The implementation is an entire Internet of Things system developed by ourselves using hardware, open-source software libraries, RealEstateCore ontology, and Microsoft Azure. A practical case study was also conducted in a historic building located in Norrk\"oping, Sweden, to demonstrate the functions of the implemented Internet of Things system. The results indicated that a digital twin that reflects the latest status of a historic building can be created and fed with real-time sensor data. The insights discovered from the digital twin provided facts for improving the indoor environment of the case study building to achieve both heritage conservation and human comfort. For future work, monitored indoor environmental conditions could be used to estimate occupancy levels. More operating status like energy consumption could also be integrated into the digital twin to model energy behaviors of the historic building and to reduce operating costs.

\section{Acknowledgements}
This research was funded by the Swedish Energy Agency (DNR: 2019-023737) within the research program of Spara och bevara. The authors thank Gustav Knutsson at Link\"oping University for his assistance in ordering experimental materials. Johan Bj\"orhn and his colleagues at Norrevo Fastigheter AB in Norrk\"oping are acknowledged for providing access to the City Theatre and support. Anna Donarelli at Uppsala University helps obtain information about activities held in the City Theatre. Photographer Markus G{\aa}rder provides the picture of the salon room in the City Theatre.

\section{Summary of Used Azure Services}
\label{apdx:summary}

\begin{table}[!hbt]
\centering
\caption{A summary of scale tiers, key specifications, and costs of used Azure services in this manuscript. Swedish krona is abbreviated as kr. DTU stands for Database Transaction Unit.\label{tab:enabling_tab1}}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}llll@{}}
\toprule
Azure Service & Scale Tier                                                                       & Key Specifications                                                                           & Costs                                                                                                                                  \\ \midrule
IoT Hub       & Standard S1                                                                      & \begin{tabular}[c]{@{}l@{}}400K messages/day per unit\\ 4 KB message meter size\end{tabular} & 253.3 kr/month                                                                                                                         \\
Functions     & \begin{tabular}[c]{@{}l@{}}Shared Environment\\ (Windows)\end{tabular}           & \begin{tabular}[c]{@{}l@{}}1 GB disk space\\ Shared compute\end{tabular}                     & \begin{tabular}[c]{@{}l@{}}0.000163 kr/(GB$\cdot$s)\\ 2.0 kr/($10^{6}$ executions)\end{tabular}                                               \\
Digital Twins & Not applicable                                                                   & Not applicable                                                                               & \begin{tabular}[c]{@{}l@{}}12.2 kr/($10^{6}$ messages)\\ 30.4 kr/($10^{6}$ operations)\\ 6.1 kr/($10^{6}$ query units)\end{tabular} \\
SQL Database  & Basic                                                                            & \begin{tabular}[c]{@{}l@{}}2 GB storage size\\ 5 DTUs\end{tabular}                           & 49.6 kr/month                                                                                                                          \\
Blob Storage  & Standard/Hot                                                                     & \begin{tabular}[c]{@{}l@{}}Milliseconds latency\\ Low access lost\end{tabular}               & 0.2 kr/GB                                                                                                                              \\
Web App       & \begin{tabular}[c]{@{}l@{}}Basic\\ Dedicated Environment \\ (Linux)\end{tabular} & \begin{tabular}[c]{@{}l@{}}10 GB disk space\\ Dedicated compute\end{tabular}                 & 133.1 kr/month                                                                                                                         \\ \bottomrule
\end{tabular}%
}
\end{table}

Table~\ref{tab:enabling_tab1} summarizes Azure services used in this manuscript. All used services are hosted in the Azure region of North Europe. Costs are in Swedish krona (kr). It is worth noting that the monthly paid services, such as IoT Hub, SQL Database, and Web App, currently support the operations of three sensor boxes. Two other sensor boxes were deployed in other case study buildings in addition to the one mentioned in this research. Moreover, it is estimated that to support the operations of 100 sensor boxes like the one in this study, the monthly cost of Azure services is around 3~000~kr.

\printbibliography[heading=subbibliography]
\end{refsection}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../demothesis"
%%% End: 


==> papers/ni_improving_2021.tex <==
\begin{abstract}
This study proposes a digitalization framework for historic buildings. In this framework, advanced techniques, like Internet of Things (IoT), cloud computing, and artificial intelligence (AI), are utilized to create digital twins for historic buildings. A digital twin is a software representation of a physical object. This study uses digital twins to protect, predict, and optimize through analytics of real-time and historical data of selected features. Heterogeneous data of historic buildings, such as indoor environment, energy consumption metering, and outdoor climate, are collected with proper sensors or retrieved from other data sources. Then, these data are periodically uploaded and stored in the database of the cloud platform. Based on these data, AI models are trained through appropriate machine learning algorithms to monitor historic buildings, predict energy consumption, and control energy-consuming equipment autonomously to reach the balance of energy efficiency, building conservation, and human comfort. The cloud-based characteristic of our digitalization framework makes the digital twins developed in this study easy to be transplanted to many other historic buildings in Sweden and other countries.
\end{abstract}

% \begin{keywords}
% historic buildings preservation, energy efficiency optimization, digital twins, artificial intelligence, Internet of Things
% \end{keywords}

% \begin{category}
%   H.5.3, H.5.4%,M.1, M.4
% \end{category}

% \sloppy{}
\begin{refsection}

\section{Introduction}
In the European Union, 35\% of buildings are over 50 years old, and almost 75\% of buildings are energy inefficient~\cite{buildup_energy_2019}. Therefore, improving energy efficiency of historic buildings contributes to reducing energy consumption and lowering greenhouse gas emissions.

Many factors can affect the energy consumption of a building. Typical factors include weather conditions outside the building, characteristics of the building itself, and occupancy inside the building~\cite{zhao_review_2012}. Figuring out how a building currently consumes energy is a critical step in reducing energy consumption. On the one hand, it helps optimize the scheduling of heating, ventilation, and air conditioning (HVAC) systems. On the other hand, it provides a benchmark for the renovation, which can quantify energy efficiency improvements after the renovation~\cite{miller_more_2019}.

Researchers have proposed two main approaches to predict the energy consumption of a building: the physical modelling approach and the data-driven approach. The physical modelling approach uses physical principles to calculate thermal dynamics and energy behaviour on the whole building level or sub-level components~\cite{zhao_review_2012}. Establishing a comprehensive physical model of a building requires detailed design information of the building and scheduling of HVAC systems~\cite{yik_predicting_2001}. The data-driven approach does not perform such energy analysis or require such detailed data about the target building but learns from available historical data for prediction. Artificial neural network (ANN) is one of the most popular algorithms used for energy consumption prediction~\cite{ahmad_review_2014, amasyali_review_2018}.

Historic buildings require continuous monitoring and maintenance to sustain functionality. Many previous studies have been conducted on deploying various types of sensors to monitor indoor environment~\cite{zhang_web-based_2013}, surface conditions~\cite{walker_thermal_2018}, and structural health~\cite{raffler_mounting_2015} of a building in real-time. Assisted by the evolvement of cloud computing, universal frameworks~\cite{liu_active_2018, liu_data-centric_2019} have been proposed for indoor environmental quality monitoring and management. Public cloud platforms enhance the reliability and scalability of frameworks while lowering the deployment cost.

This study aims to develop a cloud-based digitalization framework for energy efficiency optimization and smart maintenance of historic buildings. Advanced techniques, such as Internet of Things (IoT), artificial intelligence (AI), and cloud computing, are utilized in the framework to create digital twins of buildings. Three historic buildings located in Norrk\"oping, Sweden, as shown in Fig.~\ref{fig:improving_fig1}, are selected for case studies. All these three buildings have a history of more than a hundred years and are still used to host various social and cultural activities. These three buildings are different in their construction age, internal structure, and actual use, which can help verify the adaptability and portability of our framework. Environmental sensors are installed in these three buildings, and corresponding digital twins are created and stored in the cloud. Based on continuously collected sensing data, the digital twins can genuinely reflect real-time operating conditions and predict future states of historic buildings. The framework also facilitates maintenance to realize energy efficiency optimization and sustainable preservation with trained AI models.

\begin{figure}[!ht]
\includegraphics{figures/improving/fig1.png}
\centering
\caption{Three historic buildings in Norrk\"oping are selected for case studies. (\textbf{a}) The City Theatre (\"Ostg\"otateatern), (\textbf{b}) the Auditorium (H\"orsalen), and (\textbf{c}) the City Museum (Stadsmuseum).}\label{fig:improving_fig1}
\end{figure}

\section{Methodology}
In this study, the research objects are historic public buildings used for different social and cultural activities, and the purpose is to realize energy efficiency optimization and smart maintenance with advanced digitalization means.

\subsection{A Cloud-based Digitalization Framework}
To achieve the research goals, we propose a cloud-based digitalization framework for historic buildings. This unified digitalization framework for historic buildings can be developed with state-of-the-art communication and computing technologies. The preservation of historic buildings is a long-term process, and a large amount of data will be accumulated over time. The cloud-based framework can provide enough storage space and computing resources for these data. We also apply machine learning algorithms to learn from these data to develop AI applications to perform specific tasks, such as energy consumption prediction, visitor flow, facade or artwork decay detection, and anomaly detection, considering different cultural and historic buildings in differential indoor and outdoor climate conditions.

Fig.~\ref{fig:improving_fig2} depicts the architecture of the proposed digitalization framework. The framework has two main parts: the local part and the cloud part. The transmission layer is a bridge between the local part and the cloud part for exchanging data. In the local part, sensors and actuators are deployed in the perception layer to collect indoor environment, occupants’ behaviour, and facility operation status about a building. Edge devices are used for packaging these sensor readings and uploading them to the cloud. Besides, edge devices can receive control commands issued from the cloud. In the cloud part, the storage layer is responsible for storing data from heterogeneous sources in relational or non-relational databases. Digital twins are also created and stored in this layer. Once data are ready, evaluation methods and AI models deployed in the analysis layer can utilize them to achieve different goals. The application layer provides interactive functions to users, such as data visualization, smart maintenance, and energy consumption prediction.

\begin{figure}[!ht]
\includegraphics{figures/improving/fig2.png}
\centering
\caption{Layered architecture of the cloud-based digitalization framework for historic buildings.}\label{fig:improving_fig2}
\end{figure}

A brief introduction of the techniques integrated into this framework is illustrated in the following subsubsections.

\subsubsection{IoT and Cloud Computing}
Historic buildings require continuous monitoring and maintenance to keep sustainable functionality. IoT techniques enable a long-term goal to collect data. Cloud computing is a method for enabling ubiquitous, convenient, on-demand network access to a shared pool of configurable computing resources (e.g., networks, servers, storage, applications, and services). Cloud computing has advantages in computing, storage resources, and scalability. Nowadays, the maturity of cloud computing has allowed data storage, processing, and visualization to be done remotely in the cloud. In this study, Microsoft Azure is used as the cloud computing platform. Microsoft Azure provides plenty of components and services, which facilitates the implementation of our framework.

\subsubsection{Digital Twins}
The term Digital Twins was proposed by Grieves~\cite{grieves_digital_2014} and has been widely used in manufacturing~\cite{glaessgen_digital_2012, el_saddik_digital_2018, tao_digital_2019}. A digital twin can be interpreted as a software representation of a physical object. Based on the real-time information obtained from the physical object, a digital twin allows for rapid analysis and real-time decision-making through accurate analytics~\cite{fuller_digital_2020}. Digital twins can be created and stored in the cloud with specific domain knowledge concerning cultural heritage care and preservation.

Some researchers have applied digital twins to buildings. In paper~\cite{khajavi_digital_2019}, a digital twin was created for an office building façade to lower maintenance costs while increasing human comfort. Peng~et~al.~\cite{peng_digital_2020} proposed a digital twin for a hospital to cope with sophisticated facility systems, special medical equipment, strict security requirements, and business systems. In paper~\cite{lu_developing_2020}, the authors presented a system architecture of digital twins that is specifically designed at both building and city levels, which integrates heterogeneous data sources and supports effective data querying and analysis, and decision-making processes.

\subsubsection{AI and AI for Historic Buildings}
AI is to make the behaviour of machines look like intelligent behaviours shown by humans. Early AI applications relied on rules summarized by humans~\cite{goodfellow_deep_2016}. Researchers used human experience to sum up rules based on logic or facts, and then wrote programs to let the computer complete a task. However, for many human intelligent behaviours, such as language understanding and image identification, it is difficult for humans to know the principles and summarize the rules behind these intelligent behaviours. Therefore, researchers began to shift the focus of research to let the computer learn from the data to solve such problems. This kind of process is known as machine learning. The main purpose of machine learning is to design some learning algorithms, so that the computer can automatically analyse and obtain rules from data. The learned rules, also called models, can be used to make predictions on unknown data and solve specific problems.

AI techniques have been used for preserving historic buildings, such as monitoring structural health~\cite{mishra_machine_2021}, identifying superficial damage~\cite{wang_autonomous_2020}, and moisture analysis of walls~\cite{rymarczyk_non-destructive_2018}.

\subsection{Data Collection}
The amount and quality of collected data have a massive impact on model performance. In this part, we define what data to collect and how to collect the data.

The data to be collected mainly include the following categories:
\begin{enumerate}
    \item Indoor environment: temperature, relative humidity, CO\textsubscript{2} concentration, dust concentration, air quality, vibration, noise, and volatile organic compound (VOC).
    \item Operation status of HVAC and lighting systems.
    \item Energy consumption metering: such as electricity, hot water, chilled water, and steam.
    \item Characteristics of a building: total area size, floor count, and floor plan.
    \item Outdoor weather conditions: temperature, cloud coverage, dew temperature, and precipitation.
    \item Others: energy prices, activity schedule in the buildings.
\end{enumerate}

The way to collect data for each category includes:
\begin{enumerate}
    \item Indoor environment: sensors.
    \item Operation status of HVAC and lighting systems: query from building management system (BMS).
    \item Energy consumption metering: query from BMS.
    \item Characteristics of a building: from facility manager.
    \item Outdoor weather conditions: from nearest weather station.
    \item Others: query from corresponding official website.
\end{enumerate}

Collect frequency needs to be determined for each data collection.

\subsection{Data Analysis}
In this study, we mainly use machine learning algorithms to analyse the data to extract valuable models to achieve various predictions. The main four steps of data analysis are shown in Fig.~\ref{fig:improving_fig3}.

\begin{figure}[!ht]
\includegraphics{figures/improving/fig3.png}
\centering
\caption{The main four steps in data analysis.}\label{fig:improving_fig3}
\end{figure}

The main tasks in each step are as follows.
\begin{enumerate}
    \item Data pre-processing: after data are collected, we must process data before use. Usually, we need to detect and correct erroneous data, fill for incomplete data, and randomize data to avoid the order of the data to affect the training. We also need to divide the data into two parts: the training set and the validation set. The training set contains most of the data and is used to train the model. The validation set contains the remaining data and is used to evaluate model performance.
    \item Feature engineering: this step aims to extract useful features from the original data to improve the performance of machine learning algorithms. The extraction of features highly relies on specific domain knowledge. For example, temporal information is an important feature source for predicting the energy consumption of a historic public building because the energy consumption is different on opening hours and non-opening hours.
    \item Model training: this step is to select and use appropriate machine learning algorithms for training models. We need to select machine learning algorithms to learn from data.
    \item Model evaluation: once the training is complete, we need to evaluate the model to determine if it works on data that it has never seen before. If model performance does not meet expectations, we need to go back to the training step to improve it. Sometimes it is necessary to go back to the feature engineering step to redesign the features.
\end{enumerate}

Using the above data analysis process, we can train the corresponding prediction model for the following application scenarios.
\begin{enumerate}
    \item Advanced monitoring and alarm functions to avoid disasters.
    \item Energy optimization based on the number of shows and audience, indoor environment, and outdoor climate will be developed.
\end{enumerate}

\subsection{Framework Performance Metric}
The evaluation for the digitalization framework mainly needs to be carried out from two aspects. One is to evaluate the stability and portability of the framework. The other is to measure the actual effect of each AI model obtained by training, including the prediction performance, whether it is the optimal energy consumption, the amount of labour time saved, and an abnormal alarm calling for emergency action.

\section{Modelling and Evaluation}
To preliminarily test and verify the functionalities of the framework, we created a digital twin of an office room TP6137 at Link\"oping University based on Azure Digital Twins~\cite{azure_digital_twins_2022}. Azure Digital Twins is a platform as a service (PaaS) that enables creating knowledge graphs based on digital models. Digital models are defined according to the actual composition of a physical object. For example, to create a digital twin of a building, a series of digital models, such as Building, Floor, and Room, need to be defined. Each digital model can have several fields to reflect objects in the real world. These fields can be grouped into three categories, namely property, telemetry, and component. Properties are data fields that represent the metadata of an entity. Telemetry fields represent measurements or events. Components are used to represent a group of instances of other models.

Fig.~\ref{fig:improving_fig4} shows the composition of the created digital twin. The room TP6137 is located on the sixth floor of a building called T\"appan, and the relationship “Contains” between models reflects this. Properties of room TP6137 include area and height. Telemetries consist of measurements of environmental conditions, such as temperature and CO\textsubscript{2} concentration. Room TP6137 contains instances of other models, e.g., actuators such as lighting devices and heating equipment.

\begin{figure}[!ht]
\includegraphics{figures/improving/fig4.png}
\centering
\caption{A digital twin of room TP6137 in building T\"appan.}\label{fig:improving_fig4}
\end{figure}

A sensor box integrating IoT techniques, as depicted in Fig.~\ref{fig:improving_fig5}, is deployed in room TP6137 to collect indoor environmental conditions. Sensor readings are periodically uploaded to the cloud platform and ingested to telemetry fields of the digital twin. Based on these sensor readings, the digital twin can reflect the status of the room TP6137 in real-time.

\begin{figure}[!ht]
\includegraphics{figures/improving/fig5.png}
\centering
\caption{A sensor box is deployed in room TP6137 to collect environmental conditions, such as temperature, humidity, CO\textsubscript{2} concentration, dust concentration, air quality, and vibration.}\label{fig:improving_fig5}
\end{figure}

As an illustrative example of indoor environmental status, Fig.~\ref{fig:improving_fig6} shows historical data from a dust sensor dated from December 14 to 18, 2020. The dust concentration was high from 9 am to 3 pm, because the scheduled indoor ventilation in the building during that period enhanced the fluidity of indoor air and drove the movement of small particles.

\begin{figure}[!ht]
\includegraphics[width=3.5in]{figures/improving/fig6.png}
\centering
\caption{Historical data of a dust sensor from December 14 to 18, 2020. The dust concentration was high from 9 am to 3 pm. The scheduled indoor ventilation in the building during that period enhanced the fluidity of indoor air and drove the movement of small particles, which led to the increase of dust concentration in the room.}\label{fig:improving_fig6}
\end{figure}

\section{Future Work}
Our ultimate research goal is a cloud-based solution with both IoT and AI for maintaining unique characters that define values of historic buildings while saving energy. The project has been running for about one year and will totally last for four years. The methodology, together with the developed sensor box presented in this paper, will be utilized in the chosen historic buildings. Moreover, research questions concerning both energy-saving and historic building conservation, summarized as follows, will be studied.
\begin{enumerate}
\item Research questions concerning energy efficiency optimization:
    \begin{enumerate}
    \item What are the characteristics of the current energy consumption of a historic building?
    \item What are the main factors that can affect the energy consumption of a historic building, and how to involve these factors in the digital twin of a building?
    \item How to quantify the energy efficiency of a historic building?
    \item What methods are currently available to optimize building energy efficiency, and what are their advantages and disadvantages?
    \end{enumerate}
\item Research questions concerning smart maintenance:
    \begin{enumerate}
    \item What are the specific scenarios and objects of smart maintenance?
    \item What are the requirements for smart maintenance?
    \item What are the optimum conditions to preserve sensitive parts of the buildings?
    \item What technologies can be utilized for smart maintenance, and what are the advantages and disadvantages?
    \item What parameters of a building need to be included in the corresponding digital twin to realize smart maintenance?
    \end{enumerate}
\end{enumerate}

\section{Conclusion}
This study proposes a cloud-based digitalization framework for creating digital twins and developing AI for historic buildings, which is to be deployed to three historic buildings that are chosen for case studies. The research result so far obtained shows that data can be reliably collected, transmitted, and stored in the cloud, while digital twins that reflect the latest status of a building can be created and fed with real-time sensor data.

In the future, after deploying sensor boxes to the selected historic buildings, we will focus more on extracting useful information from collected data. More specific AI models can be trained to provide plenty of applications, such as anomaly detection, occupancy prediction, and autonomous control for historic buildings to reach energy efficiency optimization and building preservation.

\section{Acknowledgements}
This study has been financially supported by the Swedish Energy Agency within the program of Spara och Bevara. Norrevo Fastigheter AB in Norrk\"oping is acknowledged for their support and providing access to the historic buildings. The authors would like to thank Gustav Knutsson for his assistance in preparing experimental materials.

\printbibliography[heading=subbibliography]
\end{refsection}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../demothesis"
%%% End: 


==> papers/ni_leveraging_2023.tex <==
\begin{abstract}
Digital transformation in buildings accumulates massive operational data, which calls for smart solutions to utilize these data to improve energy performance. This study has proposed a solution, namely Deep Energy Twin, for integrating deep learning and digital twins to better understand building energy use and identify the potential for improving energy efficiency. Ontology was adopted to create parametric digital twins to provide consistency of data format across different systems in a building. Based on created digital twins and collected data, deep learning methods were used for performing data analytics to identify patterns and provide insights for energy optimization. As a demonstration, a case study was conducted in a public historic building in Norrk\"oping, Sweden, to compare the performance of state-of-the-art deep learning architectures in building energy forecasting. 
\end{abstract}

% \begin{keywords}
% deep learning, digital twin, building energy forecasting
% \end{keywords}


% \begin{category}
%   H.5.3, H.5.4%,M.1, M.4
% \end{category}

% \sloppy{}
\begin{refsection}
\section{Introduction}
Digital transformation in buildings has brought considerable opportunities to optimize their energy performance by integrating various advanced information and communication technologies~\cite{liu_methodology_2021}. Among them, digital twin technology is today a powerful tool for building management. With continuously collected data~\cite{ni_link_2022}, a digital twin reflects the latest status of its physical counterpart in nearly real-time~\cite{wang_survey_2022}. In addition, more advanced data analysis applications, such as energy forecasting and predictive controls, can be developed based on the virtual model and data from meters, sensors, actuators, and control systems~\cite{gunay_data_2019}. Deep learning has shown great potential in data analytics~\cite{liu_anomaly_2020,zhang_social_2021}. Based on large amounts of the collected data, deep learning methods can be used to develop models for identifying patterns in operational data, such as making predictions about energy use and revealing the potential for energy optimization~\cite{ni_improving_2021}. 

Previous studies have demonstrated the benefits of digital twins for the built environment, such as indoor or ambient climate monitoring~\cite{khajavi_digital_2019, rosati_air_2020} and anomaly detection for building assets~\cite{lu_digital_2020}. However, these studies lack an emphasis on the consistency of data representation of virtual models. Data collected from buildings are usually produced by various systems and methods~\cite{acierno_architectural_2017}. Even the most advanced building management system generates a bluster of data and information flows that differ among buildings, vendors, and locations~\cite{balaji_brick_2018}. Lacking a consistent data format makes it challenging to extend previous solutions to other buildings and limits the deployment of energy applications. Furthermore, the integration of deep learning and digital twins is still in its early stage. State-of-the-art deep learning architectures, e.g., temporal fusion transformer (TFT)~\cite{lim_temporal_2021}, have not been exploited in the built environment for improving energy performance. 

This study aims to integrate deep learning and digital twins to better understand building energy usage. The main contributions of this work are:
\begin{itemize}
  \item A solution, namely Deep Energy Twin, was proposed for analyzing building energy use and identifying potential for energy optimization. Ontology was adopted to create parametric digital twins to provide consistency of data format across different systems in a building. Deep learning was used for data analytics.
  \item A comprehensive case study was conducted to illustrate the capacity of five deep learning methods, including long short-term memory (LSTM), temporal convolutional network (TCN), Transformer, N-HiTS, and TFT, to predict building energy consumption and measure uncertainties. 
\end{itemize}

\section{Related Work}
This section first introduces the application of digital twins in the built environment. Then, deep learning methods for time series forecasting are reviewed.

\subsection{Digital Twins in the Built Environment}
Several studies have reported developing digital twin applications for the built environment, such as indoor or ambient climate monitoring~\cite{khajavi_digital_2019, rosati_air_2020}, anomaly detection for building assets~\cite{lu_digital_2020}, and heritage preservation~\cite{zhang_automatic_2022, ni_enabling_2022}. However, most of the studies lack an emphasis on the consistency of data representation of virtual models. They typically employ some customized data format, which makes it difficult to extend their solutions to other buildings, limits interoperability between buildings, and limits the deployment of energy applications. Only little work~\cite{ni_enabling_2022} looked into using a consistent metadata structure to represent buildings and subsystems. Nevertheless, integrating energy optimization solutions in buildings requires expertise in multiple domains~\cite{balaji_brick_2018}. For depicting such a complex system, it is preferable to use ontology to ensure accurate alignment across several domains, such as actuators, sensors, management workflows, and web resources~\cite{boje_towards_2020}.    

An ontology is a formal statement of a conceptualization that includes the objects, concepts, and other entities presumed to exist in a given area, together with the relationships between them~\cite{gruber_toward_1995}. Several studies have attempted to tackle the challenge of creating a metadata schema across a broad range of buildings. Balaji et al.~\cite{balaji_brick_2018} proposed Brick, a standardized metadata schema for representing buildings. The schema defines a concrete ontology for sensors, subsystems, and their relationships, enabling the development of portable applications. RealEstateCore~\cite{hammar_realestatecore_2019} is another ontology for the real estate business to speed up building modeling. Both Brick and RealEstateCore allow data output in the Digital Twin Definition Language~\cite{azure_dtdl_2022} format, which facilitates deploying applications in Microsoft Azure Cloud. Using these ontologies to create virtual models is advantageous for gathering and documenting all necessary information for further knowledge management and data analytics.

\subsection{Deep Learning for Time Series Forecasting}
Deep learning methods have emerged in recent years due to their enhanced abilities in addressing massive data, feature extraction, and modeling nonlinear processes~\cite{runge_review_2021}. Three fundamental deep learning methods for time series forecasting are recurrent neural networks (RNNs), convolutional neural networks (CNNs), and attention mechanism-based networks. 

In previous studies, RNN and its variants~\cite{hochreiter_long_1997} have been more frequently applied to building energy forecasting~\cite{kong_short-term_2019, fan_assessment_2019}. A few studies~\cite{lara_temporal_2020,wang_transformer_2022} have also applied TCN~\cite{bai_empirical_2018} and Transformer~\cite{vaswani_attention_2017}. However, recent deep learning methods, such as TFT~\cite{lim_temporal_2021} and N-HiTS~\cite{challu_n-hits_2022}, were rarely used. Therefore, a practical comparison of which method is more effective in building energy forecasting is lacking. In addition, previous studies mostly made point forecasting, and little work was carried out on making probabilistic forecasting.

\section{Methodology}
\label{sec:methodology}
First, the process of creating a parametric digital twin of building energy systems is presented. Then, the method for developing predictive models for a representative building energy application is described.

\subsection{Creation of Parametric Digital Twins}
As depicted in Fig.~\ref{fig:leveraging_fig1}, creating a parametric digital twin of a building lies in two aspects. One is to model essential physical entities and their relationships. The other is to provide the necessary interfaces to continuously update the status of entities from various data sources and supply data access for subsequent tasks, e.g., data analytics. As a reference implementation, the Brick ontology~\cite{balaji_brick_2018} was adopted for creating the parametric digital twin model. The ontology provides a consistent data representation that converts heterogeneous energy system data to a consistent format. In Fig.~\ref{fig:leveraging_fig1}, square boxes represent classes, which abstract physical entities, such as \textit{Location}, \textit{Equipment}, \textit{Resource}, and \textit{Point}. Each round box represents a specific entity, which is an instance of a particular class. A class can have multiple instances of entities.

\begin{figure}[!ht]
\includegraphics{figures/leveraging/fig1.png}
\centering
\caption{An illustration of the parametric digital twin model. A parametric digital twin model contains essential information about physical entities and their relationships. The model also provides necessary read or write application programming interfaces (APIs) for other modules, such as updating model status from data sources and providing data access for data analytics.}\label{fig:leveraging_fig1}
\end{figure}

Locations refer to different spaces in buildings, such as rooms and floors. Resources are physical resources or stuff that are controlled or measured by points. Physical or virtual entities that generate time series data are called points. Typical physical points include sensors, setpoints, and equipment status. Virtual points, on the other hand, are generated by a mechanism that may operate on other time series data, such as an average floor humidity sensor. Each data point can have several relationships that connect it to other classes, such as its location or the equipment it belongs to.

\subsection{Building Energy Forecasting}

As a demonstration of data analytics, this subsection introduces one-step ahead building energy forecasting.

\subsubsection{Problem Formulation}

A specific energy use, i.e., target variable, is denoted as $y$ and $y\in \mathbb{R}_{+}$.
Predictor variables that affect energy use are denoted as $\mathbf{x}$ and $\mathbf{x} \in \mathbb{R}^{k}$.
All target and predictor variables are supposed to be observed at constant intervals over time and grouped chronologically.
At time $t$, the observed value of the target variable is denoted as ${y}_{t}$.
Similarly, observed values of predictor variables are denoted as $\mathbf{x}_{t} =[{x}_{1,t} ,{x}_{2,t} ,...,{x}_{k,t}]$.

Then, a point forecasting model takes the form
\begin{equation}
\hat{y}_{t+1} =f_{\theta}(y_{t-w+1:t} ,\mathbf{x}_{t-w+1:t}), \label{eqn:leveraging_point_forecast}
\end{equation}
where $\hat{y}_{t+1}$ is model forecast, $y_{t-w+1:t} = [y_{t-w+1} ,y_{t-w+2} ,...,y_{t}] $ and $\mathbf{x}_{t-w+1:t}=\{\mathbf{x}_{t-w+1} ,\mathbf{x}_{t-w+2} ,...,\mathbf{x}_{t}\}$ are observations of the target and predictor variables over a loopback window $w$, and $f_{\theta }{(.)}$ is the prediction function learned by the model.

Probabilistic forecasting models are developed to generate interested quantiles directly through quantile regression. Given a set of quantiles $\mathcal{Q} \subset (0,1)$, a quantile forecasting model takes the form
\begin{equation}
\hat{y}_{t+1}^{(p)} =g_{\theta }(y_{t-w+1:t} ,\mathbf{x}_{t-w+1:t}), \label{eqn:leveraging_quantile_forecast}
\end{equation}
where $p \in \mathcal{Q}$, $\hat{y}_{t+1}^{(p)}$ is the model forecast for the $p$th quantile of the target variable, $y_{t-w+1:t}$ and $\mathbf{x}_{t-w+1:t}$ have the same definition as in the point forecasting model, and $g_{\theta}{(.)}$ is the prediction function learned by the model.

\subsubsection{Deep Learning Methods for Comparison}

Five deep learning methods, namely LSTM, TCN, Transformer, N-HiTS, and TFT, were investigated to compare their performance in building energy forecasting.

\subsubsection{Loss Function and Evaluation Metrics}
\label{sec:loss_func_eval_metric}

Point forecasting models were trained to minimize the total squared error. Probabilistic forecasting models were trained to minimize the total quantile loss. The $p$th quantile loss~\cite{lim_temporal_2021} is calculated as 
\begin{equation}
\ell(\hat{y} ,y,p)=(1-p)(\hat{y} -y)_{+} + p(y-\hat{y})_{+}, \label{eqn:leveraging_quantile_loss}
\end{equation}
where $(.)_{+}=max(0,.)$. Then, the training quantile loss $L_{q}(\theta)$ for a set $\mathcal{S} =\{(y_{t-w+1:t} ,\mathbf{x}_{t-w+1:t} ,y_{t+1})\}_{t=w}^{n+w-1}$ is calculated as
\begin{equation}
L_{q}(\theta) =\sum _{t=w}^{n+w-1}\sum _{i=1}^{| \mathcal{Q}| } \ell \left(\hat{y}_{t+1}^{( p_{i})} ,y_{t+1} ,p_{i}\right),
\end{equation}
where $p_{i} \in \mathcal{Q}$.

The prediction accuracy of point forecasting models was evaluated by coefficient of variation of the root mean square error (CV-RMSE) and normalized mean bias error (NMBE). They are calculated by Eq.~\ref{eqn:leveraging_cv-rmse} and~\ref{eqn:leveraging_nmbe}~\cite{ashrae_guideline_14_measurement_2014}.
\begin{equation}
CV\textrm{-}RMSE=\frac{\sqrt{\frac{1}{n}\sum\limits _{t=1}^{n}(\hat{y}_{t} -y_{t})^{2}}}{\overline{y}} \times 100, \label{eqn:leveraging_cv-rmse}
\end{equation}
\begin{equation}
NMBE=\frac{\frac{1}{n}\sum\limits _{t=1}^{n}(\hat{y}_{t} -y_{t})}{\overline{y}} \times 100,  \label{eqn:leveraging_nmbe}
\end{equation}
where $n$ denotes the size of forecast horizon, $y_{t}$ and $\hat{y}_{t}$ have the same definitions in the point forecasting model. $\overline{y}$ is the mean actual value of the target variable over the forecast horizon.

The $\rho$-risk, which normalizes quantile losses, was used for evaluating the performance of probabilistic forecasting models. $\rho$-risk at $p$th quantile is calculated by~\cite{lim_temporal_2021}
\begin{equation}
\rho\textrm{-}risk(p) =\frac{2\times \sum\limits _{t=1}^{n} \ell \left(\hat{y}_{t}^{(p)} ,y_{t} ,p\right)}{\sum\limits _{t=1}^{n} y_{t}}, \label{rho_risk}
\end{equation}
where $n$ denotes the size of forecast horizon, $\hat{y}_{t}^{(p)}$ is the predicted $p$th quantile value of a target variable at time $t$, and $\ell \left(\hat{y}_{t}^{(p)} ,y_{t} ,p\right)$ is the $p$th quantile loss calculated by Eq.~\ref{eqn:leveraging_quantile_loss}. 

\section{Case Study}
\label{sec:case_study}

To verify the performance of different deep learning methods, a case study was conducted to develop predictive models for energy use of one public historic building. This section describes details of the used dataset and experimental setup.

\subsection{Dataset}
\label{sec:dataset}
The dataset includes two parts. One is the historical electricity consumption and heating load from the City Museum (see Fig.~\ref{fig:leveraging_fig2}) in Norrk\"oping, Sweden. The other is the meteorological data from a weather station located $\sim$2~km away from the building. The meteorological data include dry-bulb temperature, relative humidity, dew point temperature, precipitation, air pressure, and wind speed. All data range from 01:00 on January 1, 2016 to 00:00 on January 1, 2020, with a time granularity of one hour. Hours appearing in this paper are expressed in 24-hour format and are in local time.

\begin{figure}[!ht]
\includegraphics{figures/leveraging/fig2.png}
\centering
\caption{The City Museum, Norrk\"oping, Sweden.}\label{fig:leveraging_fig2}
\end{figure}

The normal operation of the City Museum is to maintain an appropriate indoor climate for preservation of collections and human comfort of staff and visitors. In regular time, it is open six days a week, from Tuesday to Sunday. The opening time starts at 11:00. The closing time is 17:00 on Tuesdays, Wednesdays, and Fridays, 20:00 on Thursdays, and 16:00 on Saturdays and Sundays. According to the first three years of energy consumption data (see Fig.~\ref{fig:leveraging_fig3}), both electricity and heating have a yearly seasonality. Moreover, there is no long-term trend in both energy use.

\begin{figure}[!ht]
\includegraphics{figures/leveraging/fig3.png}
\centering
\caption{Historical hourly (\textbf{a}) electricity consumption and (\textbf{b}) heating load of the City Museum from 01:00 on January 1, 2016 to 00:00 on January 1, 2019.}\label{fig:leveraging_fig3}
\end{figure}


\subsection{Data Preprocessing}
\label{sec:data_preprocessing}
Data preprocessing seeks to turn raw data into a format that models can readily handle and understand.

\subsubsection{Data Cleaning and Dataset Splitting}

First, missing values in meteorological data were linearly interpolated. Then, the dataset was partitioned into three subsets: a training set for learning model parameters, a validation set for tuning hyperparameters and avoiding overfitting, and a test set for evaluating model performance. The dataset is divided roughly according to the empirical ratio of 80:10:10, with 38 months of data from January 1, 2016 to February 28, 2019 are utilized as the training set, five months of data from March 1, 2019 to July 31, 2019 are used as the validation set, and the remaining five months of data are used as the test set.

\subsubsection{Feature Preparation}
\label{sec:feature_prep}
Four temporal features are extracted from timestamps: two cyclical and two binary variables. The cyclical variables are \textit{hour} (integer value from 0 to 23) and \textit{weekday} (integer value from 0 to 6, each value represents a day in a week, starting from Monday). The binary variables include one called \textit{is holiday} to indicate if a day is a Sweden public holiday and another called \textit{is weekend} to indicate if a day is a weekend. In addition, one feature called \textit{is open} with a binary value is added to indicate if the City Museum is open for a given hour.

\subsubsection{Data Transformation}
A min-max normalization was used to scale target variables and meteorological features to a range of $[0, 1]$. The training set was utilized to fit all min-max scalers, which were then used to transform the validation and test sets. A sine-cosine transformation was used to convert cyclical features. Binary features were not transformed.

\subsection{Experimental Setup}
\label{sec:experimental_setup}

Models were developed to forecast electricity consumption and heating load of the City Museum in the next hour. A lookback window size of 24 was used. Three baseline models were created for point forecasting. Two of them are based on the seasonal na\"ive (SN) method~\cite{hyndman_forecasting_2018}, namely SN-1 and SN-24, because electricity consumption and heating load are highly seasonal. Each forecast of the SN-1 model is set to be the value observed one hour ago. The SN-24 model seeks to use daily seasonality, and each forecast of a target variable is set to the value observed 24 hours ago. The remaining one is linear regression (LR) model.

Five deep learning models (LSTM, TCN, Transformer, N-HiTS, and TFT) were trained to make both point and probabilistic forecasts. The predefined set of quantiles is $\{0.1,0.5,0.9\}$, and we are interested in evaluating $\rho$-risk on 0.5th and 0.9th quantiles. Models were built using the Python packages PyTorch (v1.12.0), darts (v0.23.1), and scikit-learn (v1.2.1). All experiments were carried out on a computer equipped with an NVIDIA GeForce GTX 1080 graphics card. 

\section{Results and Discussion}
\label{sec:results_and_discussion}

\subsection{Quantitative Analysis}

As shown in Table~\ref{tab:leveraging_tab1}, among all models, the TCN model performed best on predicting both energy use (CV-RMSE 13.90\% on electricity and CV-RMSE 8.16\% on heating). The performance of all models except for the SN-24 model on forecasting electricity has met the criterion suggested by the ASHRAE Guideline 14-2014~\cite{ashrae_guideline_14_measurement_2014} (30\% for CV-RMSE and $\pm$10\% for NMBE). Furthermore, the performance of LR and five deep learning models indicates higher predictability in heating than electricity since all of them achieved a lower CV-RMSE on predictions of heating than electricity. The higher predictability in heating load is because the building utilizes adaptive heating, which is driven by the difference between indoor and outdoor temperatures.

\begin{table}[!ht]
%\footnotesize
\centering
\caption{The prediction accuracy of point forecasts for different models on the test set. For both CV-RMSE and NMBE, a closer value to zero represents better prediction accuracy.}
\label{tab:leveraging_tab1}
\begin{tabular}{@{}lrrcrr@{}}
\toprule
\multirow{2}{*}{Model} & \multicolumn{2}{c}{Electricity} & \phantom{} & \multicolumn{2}{c}{Heating} \\ \cmidrule(lr){2-3} \cmidrule(l){5-6} 
 & \begin{tabular}[c]{@{}r@{}}\textit{CV-RMSE}\\ \textit{(\%)}\end{tabular} & \begin{tabular}[c]{@{}r@{}}\textit{NMBE}\\ \textit{(\%)}\end{tabular} &  & \begin{tabular}[c]{@{}r@{}}\textit{CV-RMSE}\\ \textit{(\%)}\end{tabular} & \begin{tabular}[c]{@{}r@{}}\textit{NMBE}\\ \textit{(\%)}\end{tabular} \\ \midrule
SN-1 & 20.13 & $-$0.04 &  & 20.31 & $-$0.04 \\
SN-24 & 45.12 & $-$0.51 &  & 24.43 & $-$1.08 \\
LR & 14.65 & $-$0.49 &  & 11.55 & 0.45 \\
LSTM & 14.31 & $-$1.12 &  & 8.65 & 2.58 \\
TCN & \textbf{13.90} & 0.69 &  & \textbf{8.16} & 1.44 \\
Transformer & 14.93 & $-$2.59 &  & 10.04 & $-$2.26 \\
N-HiTS & 14.27 & $-$0.65 &  & 8.67 & 2.61 \\
TFT & 14.60 & $-$2.66 &  & 8.18 & 1.45 \\ \bottomrule
\end{tabular}
\end{table}

In contrast to the dominance of the TCN model in point forecast, none of the five deep learning models dominates the probabilistic forecast. For predicting the electricity, the TCN model performed best to capture the central tendency as it achieved the lowest $\rho$-risk at the 0.5th quantile ($\rho$-risk$(0.5)=0.0741$ as in Table~\ref{tab:leveraging_tab2}). The LSTM model, on the other hand, performed best to capture the upper end of the distribution of the electricity ($\rho$-risk$(0.9)=0.0470$) and might be useful for predicting extreme values or identifying outliers. For predicting the heating, the TFT model performed best for both predicting median value ($\rho$-risk$(0.5)=0.0454$) and capturing the upper end of the distribution ($\rho$-risk$(0.9)=0.0231$).

\begin{table}[!ht]
%\footnotesize
\centering
\caption{The $\rho$-risk at 0.5th and 0.9th quantiles of probabilistic forecasts for different models on the test set. For each metric, lower values represent better performance.}
\label{tab:leveraging_tab2}
\begin{tabular}{@{}lrrcrr@{}}
\toprule
\multirow{2}{*}{Model} & \multicolumn{2}{c}{Electricity} & \phantom{} & \multicolumn{2}{c}{Heating} \\ \cmidrule(lr){2-3} \cmidrule(l){5-6} 
 & $\rho$\textit{-risk(0.5)} & $\rho$\textit{-risk(0.9)} &  & $\rho$\textit{-risk(0.5)} & $\rho$\textit{-risk(0.9)} \\ \midrule
LSTM & 0.0784 & \textbf{0.0470} &  & 0.0462 & 0.0234 \\
TCN & \textbf{0.0741} & 0.0480 &  & 0.0468 & 0.0237 \\
Transformer & 0.0903 & 0.0483 &  & 0.0527 & 0.0266 \\
N-HiTS & 0.0833 & 0.0476 &  & 0.0678 & 0.0318 \\
TFT & 0.0812 & 0.0526 &  & \textbf{0.0454} & \textbf{0.0231} \\ \bottomrule
\end{tabular}
\end{table}

The probabilistic forecasts also show that heating is more predictable than electricity. When predicting heating rather than electricity, all models obtained decreased $\rho$-risk at 0.5th quantile. Meanwhile, the uncertainties in electricity consumption are greater than those in heating load since these models achieved a higher $\rho$-risk at 0.9th quantile when predicting electricity than heating. Nevertheless, The uncertainty in predicting electricity also indicates that, on the one hand, it is advantageous to improve confidence by optimizing electricity use while still assuring the regular functionality of a building. On the other hand, for more accurate forecasting, additional operational model-related features that impact electricity consumption should be included.

\subsection{Qualitative Analysis}

Previous quantitative analysis indicates that heating load is more predictable than electricity consumption. The lower predictability was partly due to changes in the operating mode of the City Museum on some days in November and December 2019. Fig.~\ref{fig:leveraging_fig4}{a} shows such a change. During the two days, from November 29 to November 30, the hourly energy consumption in the nighttime was even higher than in the daytime of the previous days.

The changes in operating mode degrade the prediction accuracy of models during these days. On November 29 (the first day when the operating mode started to change), the predicted value has a certain lag (see Fig.~\ref{fig:leveraging_fig4}{a}). As shown in Fig.~\ref{fig:leveraging_fig4}{b}, the 80\% prediction interval (from 0.1th quantile to 0.9th quantile) during the daytime of the two days was relatively higher than during the daytime of the days before the operating mode changed.

\begin{figure}[!ht]
\includegraphics{figures/leveraging/fig4.png}
\centering
\caption{The actual and predicted hourly electricity consumption from November 27 to November 30, 2019. (\textbf{a}) Point forecasts of the best three models and (\textbf{b}) probabilistic forecast of the TCN model. The predicted median is P50, and the 80\% prediction interval (PI) is from 0.1th to 0.9th quantile.}\label{fig:leveraging_fig4}
\end{figure}

The higher predictability of heating load is attributed to strong influencing factors like dry-bulb temperature being involved in making predictions. In addition, the heating load is less affected by the change in operating mode. As shown in Fig.~\ref{fig:leveraging_fig5}{a}, even on November 29 and 30, the two days when the operating mode changed, the best three models still made good predictions.
Similarly, the uncertainty in predictions was greater during the daytime than during the nighttime (see Fig.~\ref{fig:leveraging_fig5}{b}). A possible explanation for the higher uncertainty during daytime is that there is more heat exchange between the indoor and outdoor environments when more people are entering and exiting the building.

\begin{figure}[!ht]
\includegraphics{figures/leveraging/fig5.png}
\centering
\caption{The actual and predicted hourly heating load from November 27 to November 30, 2019. (\textbf{a}) Point forecasts of the best three models and (\textbf{b}) probabilistic forecast of the TFT model.}\label{fig:leveraging_fig5}
\end{figure}

\section{Conclusion}
\label{sec:conclusion}

This study has presented a solution for integrating deep learning with digital twins to provide a more comprehensive understanding of building energy systems. Ontology was adopted for creating parametric digital twins of building energy systems to ensure a consistent data representation across various domains. Deep learning methods were applied to analyze the data collected by digital twins to identify patterns and seek the potential for saving energy. The results obtained from a case study in one public historic building in Norrk\"oping, Sweden, have shown that deep learning methods, such as TCN, LSTM, and TFT, exhibit strong capabilities in capturing tendency and uncertainty in building energy consumption.

The solution provides facility managers with a better insight into building energy use. Thus, facility managers can proactively optimize energy systems to avoid unnecessary energy use. In the long run, this could result in cost savings, increased human comfort, and a more sustainable built environment.

\section{Acknowledgements}
\label{sec:acknowledgements}
The authors thank Johan Bj\"orhn and his colleagues at Norrevo Fastigheter AB in Norrk\"oping for providing access to the City Museum and offering the historical energy consumption data. The Swedish Meteorological and Hydrological Institute is acknowledged for providing the weather data.

\printbibliography[heading=subbibliography]
\end{refsection}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../demothesis"
%%% End: 


==> papers/ni_link_2022.tex <==
\begin{abstract}
Information and communication technologies (ICTs) help preserve historic buildings and optimize energy efficiency. This study proposes a digitalization framework for historic buildings by utilizing ICTs, such as Internet of Things (IoT), digital twins, and cloud computing. A digital twin is a digital representation of physical world assets that genuinely reflects the properties of real-world objects and processes. In this study, historic buildings are modeled with cloud-based digital twins. Indoor environmental data are collected with locally deployed sensors and ingested to a digital twin in real-time. The digital twin enables decision-makers to remotely monitor the indoor environment of a historic building and actively manipulate actuators to perform maintenance. Empowered by data analytics and artificial intelligence (AI), a digital twin can further simulate and predict state changes in a historic building to reach desired autonomous maintenance and energy saving.
\end{abstract}

% \begin{keywords}
%   Internet of Things, digital twins, cloud computing, historic buildings, energy efficiency
% \end{keywords}


% \begin{category}
%   H.5.3, H.5.4%,M.1, M.4
% \end{category}

% \sloppy{}
\begin{refsection}

\section{Introduction}
Preservation of cultural heritage and historic buildings requires preventive approaches to maintain the materials, structure, appearance, and environmental conditions while considering energy efficiency and human comfort~\cite{balen_preventive_2015, martinez_energy_2016}. Several factors, such as ambient climate, building characteristics, and occupants’ behaviour, can affect energy consumption of a building~\cite{dalessandro_real_2018,bacher_identifying_2011,rocha_improving_2015}. To achieve human comfort, it is necessary to reasonably control heating, ventilation, and air conditioning (HVAC) systems~\cite{yu_systematic_2011, boodi_intelligent_2018}. Traditional approaches to improve indoor environmental quality (IEQ) in historic buildings highly rely on artificial manipulation of HVAC systems~\cite{shaikh_intelligent_2016}. 

Assisted by evolving information and communication technologies (ICTs), represented by Internet of Things (IoT), historic building preservation has undergone continuous development. For instance, lots of studies have demonstrated deploying various types of sensors in historic buildings to achieve real-time monitoring of indoor environment~\cite{krzemien_different_2018}, surface conditions~\cite{walker_thermal_2018}, and structural health~\cite{raffler_mounting_2015}. Our previous research~\cite{zhang_remote_2014} has developed a remote monitoring and control system for cultural and historic buildings. Wireless sensor networks based on the Zigbee protocol are deployed to heritage buildings, which enables sensing and manipulating of indoor climate from a centralized server. The results have led to the CultureBee system~\cite{culturebee_2020} that has been adopted by many Swedish churches. Based on the result, further studies~\cite{liu_active_2018, liu_data-centric_2019} proposed a universal framework for IEQ monitoring and management that leverages public cloud platform to enhance the system reliability and scalability while lowing the deployment cost. 

As a continuation, this study aims to develop a cloud-based digitalization framework that integrates IoT and digital twins for energy efficiency optimization and smart maintenance of historic buildings. Three historic buildings located in Norrk\"oping, Sweden, as shown in Fig.~\ref{fig:link_fig1}, are selected as case studies where environmental sensors are installed on site and corresponding digital twins are created and stored in the cloud. Based on continuously collected sensing data, the digital twins can genuinely reflect real-time operating conditions and predict future states of historic buildings. According to learned occupant and operating activities, digital twins also facilitate decision-making of maintenance by exploiting novel artificial intelligence to realize energy saving.

\begin{figure}[!ht]
\includegraphics{figures/link/fig1.png}
\centering
\caption{Three historic buildings are selected for case studies. (\textbf{a}) \"Ostg\"otateatern, (\textbf{b}) Stadsmuseum, and (\textbf{c}) H\"orsalen.}\label{fig:link_fig1}
\end{figure}

\section{System Overview}
Fig.~\ref{fig:link_fig2} depicts the proposed digitalization framework, which comprises five layers, namely perception layer, transmission layer, storage layer, analysis layer and application layer, following a bottom-up order. These layers can be grouped into two main parts: the local part and the cloud part. In the perception layer, sensors and actuators are deployed to collect data of indoor environment, ambient climate, facility operation status and occupants’ behaviour about a building. The transmission layer is a bridge between the local part and the cloud part. Real-time data collected from the local part and control commands issued from the cloud part are exchanged through the transmission layer. In the storage layer, data from heterogeneous sources are pre-processed and stored in relational or non-relational databases. Digital twin instances are also created and stored in this layer. Once data are ready, evaluation methods and AI models deployed in the analysis layer can utilize them to achieve different goals. The application layer provides interactive functions to users, such as data visualization, remote control, and energy consumption prediction.

\begin{figure}[!ht]
\includegraphics{figures/link/fig2.png}
\centering
\caption{Layered architecture of the cloud-based digitalization framework for historic buildings.}\label{fig:link_fig2}
\end{figure}

\section{System Design and Implementation}
The detailed design and implementation are presented in Fig.~\ref{fig:link_fig3}. In the local part, the core module is an edge device composed of a microprocessor and a microcontroller. The edge device aims for data collection, control forwarding, and edge computing. The cloud part integrates a series of services provided by Microsoft Azure. Components of the cloud part are driven by carefully designed data streams and event streams to provide applications ultimately. Detailed implementation of each part is discussed in the subsequent subsections.

\begin{figure}[!ht]
\includegraphics[width=0.9\textwidth]{figures/link/fig3.png}
\centering
\caption{Design and implementation of the cloud-based digitalization framework for historic buildings.}\label{fig:link_fig3}
\end{figure}

\subsection{The Local Part}
The implementation of the local part is presented from aspects of hardware and software.

\subsubsection{Hardware}
In the edge device, a Raspberry Pi Compute Module 3+ (CM3+) is used to provide the function of the microprocessor. The CM3+ contains a 32 GB embedded multimedia card (eMMC) flash memory and an ARMv8 system-on-chip (SoC), which has 1 GB random-access memory (RAM) and runs at 1.2 GHz. The CM3+ works with a board hosting 120 general-purpose input/output (GPIO) pins, a universal serial bus (USB) port, and two camera ports. The microcontroller used in the edge device is an Arduino Uno board, which is based on the ATmega328 chip. Each of the 14 digital pins on the board can be used as an input or output (IO). In addition to rich IOs, the board supports multiple communication buses, such as universal asynchronous receiver-transmitter (UART) and serial peripheral interface (SPI). The microprocessor and the microcontroller communicate via the SPI bus.

The edge device accesses the Internet through a 4G USB adapter. The adapter model is ZTE MF833V. According to testing, the upload and download speeds of the adapter are around 12 Mbit/s and 38 Mbit/s, respectively.

Six types of sensors are used for collecting data from a building. The detailed specifications are summarized in Table~\ref{tab:link_tab1}. The connections between sensors and the edge device are shown in Fig.~\ref{fig:link_fig3}.

\begin{table}[!ht]
\centering
\caption{Detailed specifications of used sensors.}
\label{tab:link_tab1}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}llrrrrc@{}}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Sensor}} & \multicolumn{6}{c}{Specifications} \\ \cmidrule(l){2-7} 
\multicolumn{1}{c}{} & \multicolumn{1}{c}{Measuring object} & \multicolumn{1}{c}{Unit} & \multicolumn{1}{c}{Range} & \multicolumn{1}{c}{Accuracy} & \multicolumn{1}{c}{Resolution} & Model \\ \midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Temperature \& \\humidity sensor\end{tabular}} & Temperature & °C & -40--80 & ±0.5 & 0.1 & \multirow{2}{*}{DHT22} \\
 & Relative humidity & / & 5--99\% & ±2\% & 0.1\% &  \\
CO\textsubscript{2} sensor & CO\textsubscript{2} concentration & ppm & 0--2000 & 200 & 1 & MH-Z16 \\
Dust sensor & \begin{tabular}[c]{@{}l@{}}Small particles ($d>1\mu$m) \\ in the air\end{tabular} & pcs/L & 0--28000 & / & / & PPD42NS \\
\begin{tabular}[c]{@{}l@{}}Air quality\\ sensor\end{tabular} & \begin{tabular}[c]{@{}l@{}}NH3, NOx, and \\ other harmful gases\end{tabular} & ppm & 0--2000 & / & / & MIKROE-1630 \\
\begin{tabular}[c]{@{}l@{}}Vibration\\ sensor\end{tabular} & Whether an object vibrates & / & \{0,1\} & / & / &  LDT0-028 \\
\multirow{2}{*}{Camera} & Picture & \multirow{2}{*}{pixel} & / & / & 3280×2464 & \multirow{2}{*}{RPi NoIR v2.1} \\
 & Video &  & / & / & 1080/720/480p &  \\ \bottomrule
\end{tabular}
}
\end{table}

A sensor box is presented in Fig.~\ref{fig:link_fig4}. A plastic box is used to pack the hardware. We fix the edge device on the bottom and the sensors on the lid. Many holes are drilled on the box surface to ensure enough air circulation.

\begin{figure}[!ht]
\includegraphics{figures/link/fig4.png}
\centering
\caption{Hardware setup and deployment. (\textbf{a}) Placement of the edge device, (\textbf{b}) placement of the sensors, and (\textbf{c}) a sensor box in operation.}\label{fig:link_fig4}
\end{figure}

\subsubsection{Software}
The microcontroller performs two tasks. One is to periodically obtain readings from sensors, and the other is to return the latest sensor readings when receiving a query from the microprocessor. The main modules of the microcontroller program are shown in Fig.~\ref{fig:link_fig5}. The sensor manager uses sensor drivers to obtain latest readings and stores these readings. The SPI slave handles queries from the microprocessor. The watchdog timer (WDT) ensures the long-term stable operation of the program.

\begin{figure}[!ht]
\includegraphics{figures/link/fig5.png}
\centering
\caption{Program architecture of the microcontroller.}\label{fig:link_fig5}
\end{figure}

The core function of the microprocessor is to exchange data with the cloud. On the one hand, it periodically uploads sensor readings and actuator status to the cloud. On the other hand, it takes corresponding actions when receiving instructions issued by the cloud. The main modules of the microprocessor program are shown in Fig.~\ref{fig:link_fig6}. In the application part, the collector proxy periodically queries sensor readings from the microcontroller via SPI Master. The IoT hub proxy interacts with the cloud, i.e., to package sensor readings and actuator status into messages and telemetry to the cloud. When receiving an instruction from the cloud, the method dispatcher parses the instruction and executes the corresponding method, such as taking pictures, downloading files, and uploading files. A series of utilities ensure the long-term operation of the program. For instance, remote access allows researchers to log in to the edge device for management, and the network monitor maximizes the network availability and prevents the device from being offline.

\begin{figure}[!ht]
\includegraphics{figures/link/fig6.png}
\centering
\caption{Program architecture of the microprocessor.}\label{fig:link_fig6}
\end{figure}

\subsection{The Cloud Part}
The implementation of the cloud part is explained from aspects of data routing and digital twins.

\subsubsection{Data Routing}
The IoT hub manages local edge devices and enables bidirectional communication between the cloud platform and the local edge devices. When receiving a message from an edge device, the IoT hub publishes an event. The function apps that subscribe to the event can parse the event and perform operations such as writing data to the database and updating status of digital twins. Based on these events, real-time stream analysis can also be performed. Once data are ready, we can apply different machine learning algorithms, deploy various web services, and finally provide users with applications such as data visualization, remote control, and energy consumption prediction.

\subsubsection{Digital Twins}
A digital twin instance of a building is created based on Azure Digital Twins, a platform as a service (PaaS) that enables creating knowledge graphs based on digital models. A digital model is an abstraction of real-world entities of the same type. To create a digital twin instance of a building, a series of digital models such as Building, Floor, and Room, need to be defined. As an example, Fig.~\ref{fig:link_fig7} shows a digital twin of room TP6137 in a building called T\"appan at Link\"oping University. The relationship between models is designated to reflect their interactions. Each digital model has several fields to reflect objects in the real world, such as Property, Telemetry, and Component. Properties are data fields that represent the state of a building entity such as area and height. Telemetry fields represent measurements or events and are often used to describe sensor readings. Components are used to represent a group of instances of other models, e.g., actuators such as lighting devices and heating equipment.

\begin{figure}[!ht]
\includegraphics{figures/link/fig7.png}
\centering
\caption{Digital twin of Room TP6137, Building T\"appan, Campus Norrk\"oping, Link\"oping University.}\label{fig:link_fig7}
\end{figure}

\section{Results and Discussion}
To preliminarily test and verify the functionalities of the framework, we deployed a sensor box (see Fig.~\ref{fig:link_fig4}c) in a room at Link\"oping University. Environmental parameters were collected, transmitted to the cloud platform, and ingested to the digital twin instance through the aforementioned approach. 

Fig.~\ref{fig:link_fig8} depicts historical data from two sensors. It is seen in Fig.~\ref{fig:link_fig8}a that the dust concentration was high from 9 am to 3 pm in these four days. After investigation, we find that the scheduled indoor ventilation in the building during that period enhanced the fluidity of indoor air and drove the movement of small particles, which led to the increase of dust concentration in the room. Simultaneously, the correlation between CO\textsubscript{2} concentration and room occupancy is seen in Fig.~\ref{fig:link_fig8}b; details are described in Fig.~\ref{fig:link_fig9}.

\begin{figure}[!ht]
\includegraphics{figures/link/fig8.png}
\centering
\caption{Historical data of sensors from November 25 to 28, 2020. (\textbf{a}) Dust sensing, and (\textbf{b}) CO\textsubscript{2} sensing.}\label{fig:link_fig8}
\end{figure}

\begin{figure}[!ht]
\includegraphics{figures/link/fig9.png}
\centering
\caption{Occupant's presence can affect CO\textsubscript{2} concentration. (\textbf{a}) One person in the room, and (\textbf{b}) no one in the room.}\label{fig:link_fig9}
\end{figure}

After comparing the CO\textsubscript{2} concentration changes on November 26 (one person in the room) and November 27 (no one in the room), we find an occupant's presence can significantly affect the CO\textsubscript{2} concentration. The detailed explanation of CO\textsubscript{2} concentration changes near the three marked points in Fig.~\ref{fig:link_fig9}a is as follows. 1) The occupant entered the room and started working, which caused the CO\textsubscript{2} concentration to increase. 2) The occupant went out for lunch and returned after an hour, which caused the CO\textsubscript{2} concentration to decrease first and then increase. 3) The occupant left the room after getting off work, which caused CO\textsubscript{2} concentration to decrease.

Obviously, this correlation can be used to predict the occupancy to realize autonomous control of HVAC systems and lighting. As for the future, with continuously collected sensor data from the three historic buildings, more correlations between sensor readings and occupants' behaviour can be investigated to enrich more applications and finally achieve energy efficiency optimization and intelligent maintenance.

\section{Conclusion}
This study proposes a cloud-based digitalization framework by utilizing IoT and digital twins for historic buildings, which is to be deployed to three heritage buildings that are chosen for case study. The detailed design and implementation in terms of both hardware and software are presented. The experimental deployment results show that data can be collected, transmitted, and stored in the cloud while digital twins that reflect the latest status of a building can be created and fed with real-time sensor data. A sample digital twin instance is given to illustrate the building models.

In the future, after deploying sensor boxes to the selected historic buildings, we will focus more on digging information from collected data. More specific AI models can be trained to provide plenty of applications, such as anomaly detection, energy consumption prediction, and autonomous control for historic buildings to reach energy efficiency optimization.


\section{Acknowledgements}
We thank Gustav Knutsson for his assistance in ordering electronic components and experimental materials. This study has been financially supported by the Swedish Energy Agency within the program of Spara och Bevara. Norrevo Fastigheter AB in Norrk\"oping is acknowledged for their support and providing access to the historic buildings.

\printbibliography[heading=subbibliography]
\end{refsection}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../demothesis"
%%% End: 


==> papers/ni_sensing_2021.tex <==
\begin{abstract}
Monitoring the indoor environment of historic buildings helps to identify potential risks, provide guidelines for improving regular maintenance, and preserve cultural artifacts. However, most of the existing monitoring systems proposed for historic buildings are not for general digitization purposes that provide data for smart services employing, e.g., artificial intelligence with machine learning. In addition, considering that preserving historic buildings is a long-term process that demands preventive maintenance, a monitoring system requires stable and scalable storage and computing resources. In this paper, a digitalization framework is proposed for smart preservation of historic buildings. A sensing system following the architecture of this framework is implemented by integrating various advanced digitalization techniques, such as Internet of Things, Edge computing, and Cloud computing. The sensing system realizes remote data collection, enables viewing real-time and historical data, and provides the capability for performing real-time analysis to achieve preventive maintenance of historic buildings in future research. Field testing results show that the implemented sensing system has a 2\% end-to-end loss rate for collecting data samples and the loss rate can be decreased to 0.3\%. The low loss rate indicates that the proposed sensing system has high stability and meets the requirements for long-term monitoring of historic buildings.
\end{abstract}

% \begin{keywords}
%   Internet of Things, edge computing, cloud computing, historic buildings, indoor environment
% \end{keywords}


% \begin{category}
%   H.5.3, H.5.4%,M.1, M.4
% \end{category}

% \sloppy{}
\begin{refsection}

\section{Introduction}
\label{sec:sensing_intro}
The preservation of historic buildings aims to mitigate the deterioration of fa\c{c}ades, architectural structures and housed valuable artworks as most as possible~\cite{camuffo_microclimate_2019}.
Previous studies on the preservation of museums~\cite{camuffo_indoor_1999,camuffo_environmental_2001,corgnati_methodology_2009,thomson_museum_1994}, galleries~\cite{camuffo_microclimate_2002}, churches~\cite{loupa_indoor_2006}, and cathedrals~\cite{zarzo_long_2011} have indicated that improper maintenance can result in large fluctuations in temperature and relative humidity and, hence, cause irreversible changes in dimensions of artworks.
Furthermore, many historic buildings, such as theaters and museums, are still open to the public for holding activities or visiting. Human comfort also requires a suitable indoor environment, which makes it more difficult for conservation~\cite{camuffo_indoor_1999}. Monitoring the indoor environment can help identify potential risks and provide guidelines for improving the control strategies of heating, ventilation, and air conditioning (HVAC) systems~\cite{camuffo_environmental_2001,camuffo_microclimate_2002,corgnati_methodology_2009} to provide suitable conditions for slowing down the deterioration.
Therefore, concerning preserving artworks and achieving human comfort, implementing a system for monitoring indoor environment of historic buildings is both essential and challenging.

Monitoring the indoor environment usually includes the process of data collection, transmission, storage, analysis, and application. Many previous research studies have focused on one or more of them. For data collection, Diego et~al.~\cite{garcia_design_2015} used open-source hardware and sensors to monitor heritage buildings. Lombardo et~al.~\cite{lombardo_wireless_2017} and Grassini et~al.~\cite{grassini_cloud_2017} proposed monitoring solutions based on small sensing nodes. Low energy consumption is another important property in data collection, which is considered by Huynh et~al.~\cite{huynh_wireless_2010}, Zhang et~al.~\cite{zhang_remote_2010}, and Perles et~al.~\cite{perles_energy_2018}. For data transmission, Burri et~al.~\cite{burri_dozer_2007} proposed a data gathering protocol that enables ultra-low power consumption. Several works used wireless sensor networks in their remote monitoring systems~\cite{huynh_wireless_2010, zhang_remote_2010, lazarescu_design_2013, klein_wireless_2017}.
For data storage, Fernandez et~al.~\cite{fernandez_software_2013} presented the database for storage used for cultural heritage preventive conservation. For data analysis and application, many research studies applied collected data to multiple aspects for the preservation of historic buildings, such as predicting indoor particulate matter~\cite{moon_heterogeneous_2019} and modelling the thermo-hygrometric conditions~\cite{merello_high_2018}.

Previous monitoring systems are usually specific solutions for specific application scenarios. These systems rely on particular technologies and platforms but are not designed for general digitialization and smart service purposes. When data are in focus, advanced technology such as artificial intelligence with machine learning can be utilized. Thus, a general digitalization framework for monitoring indoor environment of historic buildings is needed. Several previous studies have been reported on designing such framework. Guo et~al.~\cite{guo_ima_2012} designed an integrated monitoring system based on web services to facilitate system integration between heterogeneous data sources. Bolchini et~al.~\cite{bolchini_smart_2017} proposed a methodology for monitoring and data analysis of smart buildings based on existing frameworks but lacked the consideration for scenarios of preserving historic buildings. Akrivopoulos et~al.~\cite{akrivopoulos_fog_2018} presented a platform that provides an integrated solution for real-time monitoring and management of educational buildings. Liu et~al.~\cite{liu_data-centric_2019} proposed a data-centric Internet of Things (IoT) framework that is based on a unified device management model and data model with the help of public cloud services, hence, improving the interoperability and compatibility between heterogeneous hardware and communication protocols. However, frameworks proposed in these papers are either hard to be reused by other people because of the usage of private clouds~\cite{guo_ima_2012} and self-developed data visualization modules~\cite{liu_data-centric_2019} or restricted within a small scope of functions, with a limited capability for data analysis~\cite{guo_ima_2012}, and the lack of the interface for viewing real-time and historical data~\cite{akrivopoulos_fog_2018}. Therefore, a novel digitalization framework that is adaptable, i.e., easy to be implemented and reused by other people for monitoring and preserving historic buildings, is studied and presented in this paper.

In addition to being adaptable, the new framework needs to address two challenges. The first challenge is about stable and scalable storage.
Monitoring historic buildings is a long-term process, during which lots of data are collected and the system requires stable and scalable storage resources. For instance, to deploy 32 nodes in a historic building, each node needs to measure five environmental parameters every 15 s and each measured data sample is stored by two bytes, then the storage resource required per day is about two megabyte (MB). If more data are required to collect for preserving historic buildings, stable and scalable storage resources are needed. Some pioneering works used offline data loggers~\cite{zarzo_long_2011,gysels_indoor_2004} or private clouds~\cite{huynh_wireless_2010,zhang_remote_2010,guo_ima_2012,lazarescu_design_2013,corbellini_cloud_2018} to store these data. However, both offline data loggers and private clouds have shortcomings when being used for long-term monitoring of historic buildings. Offline data loggers usually store data on a single storage medium and, once the storage medium fails, all data might be lost. Hence, even with a separate local backup, the data are more vulnerable to potentially catastrophic events such as theft, fire, and events that are similar. Managing private clouds requires considerable cost and accountability. Therefore, it is necessary to find a solution to provide stable and scalable storage.
Recently, the maturity of public cloud services, such as Microsoft Azure~\cite{microsoft_azure_2021}, Amazon Web Services~\cite{amazon_aws_2021}, and Google Cloud~\cite{google_cloud_2021}, fulfills the requirements for stable and scalable storage resources. In this paper, this challenge is tackled by using public cloud storage.

Another challenge is related to the capability of performing real-time analysis to realize preventive maintenance. A significant limitation of early works~\cite{zarzo_long_2011,gysels_indoor_2004} is that data analysis is usually carried out after a period of collection. Although late analysis can still provide some useful information and can improve strategies, it is better to perform real-time analysis for these data to find potential risks in time and realize preventive maintenance~\cite{fernandez_software_2013,liu_anomaly_2020}. Meanwhile, to preserve historic buildings, more and more applications will be developed and deployed and, thus, the computing resources must also be scalable. Public cloud services can provide on-demand computing resources for performing real-time analysis.
Moreover, edge computing is an excellent supplement to cloud computing~\cite{shi_edge_2016} in application scenarios that have sensitive data or require low response time. Moon et~al.~\cite{moon_heterogeneous_2019} proposed a framework to predict indoor particulate matter concentration on an edge device by pre-trained machine learning models. Tse et~al.~\cite{tse_monitoring_2018} used a low-cost sensing system based on edge computing to monitor indoor environment of cultural heritage buildings. Recently, real-time optimization methods~\cite{sands_virtual_2021} and artificial intelligence methods~\cite{sands_development_2020} provide the ability for better control of the system. In this paper, cloud computing and edge computing are integrated to provide the capability for real-time analysis. With the help of public cloud services and edge devices, powerful machine learning methods can be applied to perform real-time analysis and realize automatic control, as presented by Grzonka et~al.~\cite{grzonka_using_2018}, in future work.

This paper focuses on overcoming the aforementioned drawbacks of existing works. An adaptable digitalization framework for preserving historic buildings is presented, which tackles the challenges in stable and scalable storage, as well as the capability of real-time analysis. A sensing system following the architecture of the digitalization framework is implemented to monitor the indoor environment of historic buildings. The implemented sensing system consists of perception devices, an edge platform, and a cloud platform. The perception devices and edge platform are packaged in a locally deployed sensor box.
The sensor box can monitor indoor environmental parameters such as temperature, relative humidity, carbon dioxide (CO\textsubscript{2}) concentration, suspended particulate matter, harmful gases, and vibration. The obtained data are periodically synchronized to the cloud via the cellular network. The cloud part takes advantage of a series of public cloud services. A web-based user interface is developed in this study for facility managers and researchers to view the indoor environment in real-time and to check the historical trend. With the proposed system in this study, data can be analyzed in real-time either on the cloud platform to provide functionalities such as anomaly detection, pushing alerts, and preventive maintenance or on an edge device without uploading them to the cloud.

The contributions of this paper are listed as follows:
\begin{itemize}
\item   An adaptable digitalization framework for smart preservation of historic buildings is proposed. This framework has a flexible architecture that other people can refer to in implementing their systems.
\item A sensing system following the architecture of the proposed digitalization framework is implemented by using public cloud services, open-source software, and hardware. This system supports data collection, transmission, storage, and visualization. This system also supports adding more functionalities in future research.
\item	The implemented sensing system is applied on three historic buildings in Sweden for field testing. The stability for long-term operation of the sensing system is evaluated. A preliminary analysis for the indoor environment is also showcased by following industry standards.
\end{itemize}

The remainder of this paper is structured as follows. In Section~\ref{sec:sensing_system_design}, the layered architecture of the digitalization framework and the main components and functional modules of each layer will be provided. In Section~\ref{sec:sensing_system_implementation}, the detailed implementation of the sensing system, including used hardware, software libraries, and public cloud services, are described. In Section~\ref{sec:sensing_case_studies}, the three historic buildings chosen for conducting field testing and the evaluation methodology are presented. In Section~\ref{sec:sensing_results_discussion}, the field testing results are illustrated and analyzed. The last section concludes the paper and discusses future work.

\section{System Design}
\label{sec:sensing_system_design}
Fig.~\ref{fig:sensing_fig1} depicts the architecture of the digitalization framework. The framework consists of three parts, namely Perception Devices, Edge Platform, and Cloud Platform, following a bottom-up order.

\begin{figure}[!ht]
\includegraphics{figures/sensing/fig1.png}
\centering
\caption{Architecture of the proposed digitalization framework. (\textbf{a}) Perception Devices, (\textbf{b}) Edge Platform, and (\textbf{c}) Cloud Platform.}\label{fig:sensing_fig1}
\end{figure}

The perception devices provide necessary data from historic buildings for the whole system. There are three categories of perception devices: Collector and Sensors, Controller and Actuators, and Broker and Other Systems. The sensors are used to measure the ambient environment. The collector is used to obtain measured environmental data from sensors. The actuators refer to devices, e.g., lighting, that can be controlled. The controller is used to receive control commands issued from upper parts and control actuators by the commands. The broker acts as an intermediary between this system and other systems, such as the building management system (BMS) in a historic building.

Each edge platform can serve multiple sets of perception devices. The communication between the edge platform and perception devices can either be through a wired bus or a wireless channel. The edge platform contains four types of functional modules, namely Aggregator, Local Storage, Local Analytics, and Local Gateway. The aggregator is responsible for communicating with perception devices and has two functions. One is gathering data, e.g., sensing data, actuator status, and the information provided by other systems, and sharing these data with other modules of the edge platform. Another is forwarding control commands to controllers and brokers. The local storage is used to store running logs, configuration files, and privacy data. The local analytics aims to analyze the collected data. The local gateway is used to communicate with the cloud platform and has two functions: One is synchronizing the aggregated data to the cloud platform and another is forwarding instructions and tasks issued by the cloud platform.

The cloud platform also has four types of functional modules, namely Cloud Gateway, Cloud Storage, Cloud Analytics, and Applications. The cloud gateway provides a hub for bidirectional communication with edge devices to synchronize data and commands. The cloud storage provides stable and scalable resources for storing data persistently. The cloud analytics provides the capability for performing data analysis tasks. Based on the collected data and analysis results, users can be provided with a series of applications, such as data visualization, anomaly detection, and preventive maintenance.

Following such a framework, researchers can make full use of resources brought by cloud computing and edge computing to design, deploy, and verify various applications for the smart preservation of historic buildings.

\section{System Implementation}
\label{sec:sensing_system_implementation}
In this section, a sensing system following the proposed digitalization framework is implemented. The detailed components of each part are illustrated.

\subsection{Collector and Sensors}
\label{sec:sensing_collector_sensors}
A collector requires rich peripheral interfaces to facilitate sensors with different output signals. Moreover, in order to aid writing and testing programs, the collector should also provide good software support. In this study, an Arduino microcontroller board (Arduino Uno Rev3 SMD, Arduino, Somerville, MA, USA) equipped with a base shield board (Grove Base Shield V2, Seeed Technology, Shenzhen, CHN) is utilized to act as the collector (see Fig.~\ref{fig:sensing_fig2}) to obtain readings from sensors. The Arduino board is based on the ATmega328 and has 14 digital input/output (IO) pins and six analog input pins. Six of the fourteen digital IO pins can be used as pulse width modulation outputs. The base shield board has sixteen onboard Grove connectors, four for analog inputs, seven for digital IO, one for universal asynchronous receiver-transmitter (UART) communication, and four for inter-integrated circuit communication. These Grove connectors simplify the connections with sensors.

\begin{figure}[!ht]
\includegraphics{figures/sensing/fig2.png}
\centering
\caption{A sketch map for data communication interfaces between the collector and sensors, as well as between the collector and the edge platform.}\label{fig:sensing_fig2}
\end{figure}

Five sensors are used to measure temperature, relative humidity, CO\textsubscript{2}, suspended particulate matter, poisonous gases, and vibration in historic buildings:
\begin{itemize}
\item	A temperature and relative humidity (T\&RH) sensor (DHT22, Seeed Technology, Shenzhen, CHN) is used to measure temperature and relative humidity. The detecting range is $-$40--80~\textdegree{C} for temperature and 5--99\% for relative humidity. The accuracy reaches up to 0.5~\textdegree{C} and 2\% RH. 
\item	A CO\textsubscript{2} sensor (MH-Z16, Winsen Electronics Technology, Zhengzhou, CHN) is adopted to measure CO\textsubscript{2} concentration. This sensor uses non-dispersive infrared to detect CO\textsubscript{2} in the air. The measurement range is 0--2000 parts per million (PPM). The resolution is one PPM, while the accuracy is 200 PPM. The CO\textsubscript{2} sensor can be operated at temperature 0--50 \textdegree{C} and humidity 0--90\% RH.
\item	A dust sensor (PPD42NS, Shinyei Corporation, New York, NY, USA) is utilized to measure suspended particulate matter concentration in the air. This sensor can detect particles with a diameter larger than one $\mu$m. The particulate matter level in the air is measured by counting the low pulse occupancy (LPO) time in a given time unit. LPO time is proportional to the particulate matter concentration. The detecting range is 0--28,000 pieces per liter (pcs/L).
\item  An air quality (AQ) sensor (MIKROE-1630, MikroElektronika, Beograd, SRB), which carries an MQ-135 sensor, is used to detect poisonous gases, e.g., ammonia, nitrogen oxides, and benzene.
\item  A vibration sensor (Grove-Piezo Vibration Sensor, Seeed Technology, Shenzhen, CHN) based on PZT film sensor LDT0-028 is used to measure vibration and impact generated by human activities.
\end{itemize}

The program running on the Arduino board is written, tested, and uploaded with Arduino Integrated Development Environment (version 1.8.13)~\cite{arduino_software_2021}. The native serial communication hardware UART of the Arduino board is reserved for debugging and uploading code. Therefore, the SoftwareSerial Library~\cite{arduino_softwareserial_2021} is used to replicate the serial communication functionality. A watchdog timer is enabled to ensure the long-term stable operation of the program.

\subsection{Edge Platform}
\label{sec:sensing_edge_platform}
In order to cope with the deployment conditions of historic buildings, current and subsequent research demands, the edge platform needs to meet the following requirements:
\begin{itemize}
\item	Compact size and flexible mounting options for easy deployment in historic buildings;
\item   Sufficient computing and storage resources for processing and analyzing collected data or performing partitioned tasks assigned to the edge platform;
\item   Rich peripheral interfaces for connecting with perception devices.
\end{itemize}

In this study, three components (see Fig.~\ref{fig:sensing_fig3}) are integrated to implement an edge platform to fulfill the requirements as mentioned above.

\begin{figure}[!ht]
\includegraphics{figures/sensing/fig3.png}
\centering
\caption{Components of the edge platform.}\label{fig:sensing_fig3}
\end{figure}

A Raspberry Pi Compute Module 3+ Development Kit (RPi CM3+ Dev Kit) (Raspberry Pi Foundation, Cambridge, GBR) is adopted as the core edge device of the edge platform. The development kit contains a Raspberry Pi Computing Module 3+ (RPi CM3+) and a Raspberry Pi Compute Module IO Board V3. The RPi CM3+ is based on Broadcom BCM2837B0, which is a Cortex-A53 (ARMv8) 64-bit system-on-chip that runs at 1.2 GHz. The RPi CM3+ has one gigabyte (GB) synchronous dynamic random-access memory (SDRAM) and up to 32 GB embedded multimedia card (eMMC) flash memory. The IO board hosts 120 general-purpose input/output (GPIO) pins, a high-definition multimedia interface (HDMI) port, a universal serial bus (USB) port, two camera ports, and two display~ports.

In order to obtain more USB ports to meet future needs, the RPi CM3+ Dev Kit is equipped with a USB hub (DUB-H4 rev E, D-Link Corporation, Taipei City, Taipei, TWN). One highlight of this USB hub is that it supports controlling USB power per port. This feature is handy for the RPi CM3+ Dev Kit to power off and restart the connected USB~devices.

A 4G USB adapter (ZTE MF833V, ZTE, Shenzhen, CHN), together with a mobile broadband subscription, is used to gain access to the Internet. The supported maximum link rate is 150 Mbit/s for download and 50 Mbit/s for upload under the specific 4G~network.

The Raspberry Pi Imager~\cite{raspberry_os_2021} is used to install Raspberry Pi OS for the edge device. A terminal tool called MobaXterm~\cite{mobaxterm_2021} is used to operate the RPi CM3+ via serial or secure shell session. Other terminal tools, e.g., PuTTY, can also be used as alternatives to MobaXterm. The communication between the RPi CM3+ and the microcontroller is based on the serial peripheral interface (SPI) bus. The python Linux SPI library spidev 3.5~\cite{spidev_2021} is used to implement communication functionality between the edge device and a collector. The SPI clock frequency is 122,000 Hz. The python Azure IoT Device software development kit (SDK) azure-iot-device 2.3.0~\cite{azure-iot-device_2021} is used for communicating with the Azure IoT Hub. In order to facilitate remote management and maintenance, a connection service~\cite{remoteit_2021} is adopted to gain access to the edge platform. A series of utilities ensure the long-term operation of the program. For instance, remote access allows researchers to log in to the edge device for management and the network monitor maximizes the network availability and prevents the device from being offline.

A plastic box (TPC 201610T/TAM 201610, Fibox AB, Bromma, Stockholm, SWE) with a dimension 163~$\times$~201~$\times$~98 mm is used for packaging the edge platform and the first set of a collector and five sensors. An assembled sensor box is shown in Fig.~\ref{fig:sensing_fig4}{a}. In order to obtain good heat dissipation performance, a sufficient number of holes are drilled on the surface of the box to allow air circulation. To mitigate the effect of internal heat dissipation, the T\&RH sensor is mounted at the farthest place from the heat source (the processor of RPi CM3+ and the AQ sensor) and is completely exposed to the external environment through a rectangular hole (see Fig.~\ref{fig:sensing_fig4}{b}).

\begin{figure}[!ht]
\includegraphics{figures/sensing/fig4.png}
\centering
\caption{The assembled sensor box. (\textbf{a}) Front view and (\textbf{b}) right side view.}\label{fig:sensing_fig4}
\end{figure}

\subsection{Cloud Platform}
\label{sec:sensing_cloud_platform}
Microsoft Azure is one of representatives of public cloud and is used to provide services for the sensing system in this study. In addition to Microsoft Azure, other public cloud services can also be used to implement the cloud part of such a sensing system.

According to the focused tasks, the cloud platform (see Fig.~\ref{fig:sensing_fig5}) is divided into two parts, namely the back-end and the front-end. The back-end focuses on domain logic, that is, data acquisition, analysis, and storage. The front-end focuses on providing user-friendly interfaces for users to utilize applications.

\begin{figure}[!ht]
\includegraphics{figures/sensing/fig5.png}
\centering
\caption{The service components used on the cloud platform and the data flow between the service components.}\label{fig:sensing_fig5}
\end{figure}

The Azure services that are used to build the back-end are as follows:
\begin{itemize}
\item	``IoT Hub''~\cite{azure_iothub_2021} acts as a central message hub for reliable and secure bi-directional communication between the edge and cloud platforms. The IoT Hub supports multiple messaging patterns such as device-to-cloud telemetry, cloud-to-device messages, and invoking direct methods on devices from the cloud. In this study, the device-to-cloud telemetry is used to deliver collected environmental data from the edge platform to the cloud platform.
\item	``Event Hubs''~\cite{azure_eventhubs_2021} is used to build a pipeline for ingesting data in real-time. When the IoT Hub receives device-to-cloud telemetries from the edge platform, Event Hubs notifies subscribed consumers to consume the messages.
\item	``Functions''~\cite{azure_functions_2021} is an event-driven serverless compute platform. A serverless function is implemented by utilizing Functions to consume events from Event Hubs, parse sensing data from device-to-cloud telemetry, and insert sensing data into the database.
\item	``SQL Database''~\cite{azure_sql_database_2021} provides scalable storage resources and is used for storing structured data in this study. Metadata of historic buildings, metadata of edge devices, and sensing data are stored in separated tables.
\item	``Blob Storage''~\cite{azure_blob_storage_2021} helps to store and access unstructured data at scale. Images or documents produced in this study are stored in Blob Storage.
\item	``Web Apps''~\cite{azure_web_app_2021} facilitates deployment of web applications. The sensing system provides data visualization for collected data by using a web application deployed by Web Apps service.
\end{itemize}

For each used Azure service, the scale tier is selected by current needs (see Table~\ref{tab:sensing_tab3} in Appendix). These services also support scale-up to meet future research needs.

In order to help facility managers and researchers view real-time and historical data, a web application is developed based on dash plotly~\cite{dash_plotly_2021}. The application mainly uses module Scattergl to visualize sensing data points as line charts. Compared to module Scatter, Scattergl has advantages such as faster speed and improved interactivity.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Case Studies}
\label{sec:sensing_case_studies}
This section focuses on the practical application of the implemented sensing system in historic buildings. First, a brief description of three historic buildings chosen as case studies is provided. Then, a metric to evaluate the stability of the operating status of the sensing system is illustrated. Finally, the procedure of performing relative humidity fluctuation analysis according to a European standard is introduced.

\subsection{Description of Three Historic Buildings}
\label{sec:sensing_desc_of_buildings}
In this study, three historic buildings (see Fig.~\ref{fig:sensing_fig6}) with different kinds of use and characteristics in Norrk\"oping, Sweden, are chosen as case studies to test the functionalities and stability of the sensing system. These three historic buildings have been listed as protected buildings and are still open to the public for visiting and holding activities.

\begin{figure}[!ht]
\includegraphics{figures/sensing/fig6.png}
\centering
\caption{Three historic buildings in Norrk\"oping, Sweden, are chosen as case studies: (\textbf{a}) the City Museum, (\textbf{b}) the City Theatre, and (\textbf{c}) the Auditorium.}\label{fig:sensing_fig6}
\end{figure}

The City Museum (Fig.~\ref{fig:sensing_fig6}{a}) is housed in old factory premises beside the Motala river, in the middle of Norrk\"oping's old industrial landscape. Those factory premises were erected in the 19{th} and 20{th} centuries and have been listed as protected buildings according to the national heritage legislation since 1990. The City Museum's collection of objects includes almost 40,000 individual objects. The collections include, for example, handicraft tools of all kinds, weaving and spinning machines, billboards, printed fabrics, and sheets. These are all kinds of objects that, in different ways, illustrate Norrk\"oping's history, mainly the 19{th} and 20{th} century crafts and industrial history.

The City Theatre (Fig.~\ref{fig:sensing_fig6}{b}) is located in the city centre of Norrk\"oping. The building was completed in 1908 and is a representative of the Art Noveau style. The building is used as a platform for performing arts and is owned by region \"Osterg\"otland and Norrk\"oping Municipality. The building has been listed as a protected building according to the national heritage legislation since 1990.

The Auditorium (Fig.~\ref{fig:sensing_fig6}{c}) was originally constructed as a church in 1827. From 1913 the building had been used as the city concert hall until 1994. Today, the Auditorium hosts local concerts and is used as a lecture hall by the local culture school. Norrk\"oping Municipality is the owner of the building. The Auditorium was listed as a protected building according to the national heritage legislation in 1978.

Since 16 March 2021, the first batch of three sensor boxes (see Figure~\ref{fig:sensing_fig7}) has been deployed, one for each building. There are two key focus points for deploying the first batch of sensor boxes: One is to examine the stability of the sensing system in the actual operating environment; the other is to obtain a preliminary understanding of the variations in the indoor environment of the three historic buildings. 

\begin{figure}[!ht]
\includegraphics{figures/sensing/fig7.png}
\centering
\caption{The deployments in: (\textbf{a}) the City Museum, (\textbf{b}) the City Theatre, and (\textbf{c}) the Auditorium.}\label{fig:sensing_fig7}
\end{figure}

In the City Museum, the sensor box (Figure~\ref{fig:sensing_fig7}{a}) is deployed in an exhibition room housing ancient collections on the third floor to improve the preservation of these collections. In the City Theatre, the sensor box (Figure~\ref{fig:sensing_fig7}{b}) is deployed under the fence of the second floor of the grandstand, which is nearly the spatial center of the hall, to obtain environmental conditions that are close to the average values of the entire hall. In the Auditorium, the sensor box (Figure~\ref{fig:sensing_fig7}{c}) is deployed under the stage to measure the indoor environment while detecting human activities.

\subsection{Metric to Evaluate the Stability}
\label{sec:sensing_metric_stability}
The loss rate of data samples is taken as the metric to evaluate the stability of data acquisition. The transmission of data is an end-to-end process and it involves cooperation between various modules. Therefore, the loss rate can be a good measurement of the operating stability of the entire system. The loss rate (\textit{lr}) in a time interval is given by:

\begin{equation}
lr=\frac{expected-actual}{expected} \times 100\%
\end{equation}

where \textit{expected} denotes the number of data samples expected to be collected and \textit{actual} denotes the actual number of collected data samples.

In this paper, the time interval chosen for calculating the loss rate of data samples is 56 days, from 5 April 2021 12:00 a.m. to 31 May 2021 12:00 a.m.; the timezone is Central European Time (CET). The expected number of data samples that each sensor box collects is $56\times24\times60\times60\div15$~=~322,560.

\subsection{Fluctuation Analysis of Relative Humidity}
\label{sec:sensing_fluctuation_analysis}
To preliminarily analyze fluctuation of relative humidity, the method in European standard EN 15757:2010~\cite{en_15757_conservation_2010} is used. This European standard serves as a guide for establishing temperature and relative humidity conditions in historic buildings to prevent climate-induced physical damage to hygroscopic and organic materials.

In this paper, a preliminary fluctuation analysis is performed for relative humidity in the City Museum because it has rich collections. First, to eliminate occasional spike noises of the relative humidity readings, a resampling was performed by taking the median of the readings every five minutes. Then, based on resampled readings, the following values are calculated according to this European standard.
\begin{itemize}
\item	Average level over a selected period: This level is calculated as the arithmetic mean of the relative humidity readings as follows:

\begin{equation}
\label{eq:sensing_avg}
\bar{x} = \frac{1}{n}\sum_{i=1}^{n}{x}_{i}
\end{equation}
where $\bar{x}$ denotes the average level, \textit{x\textsubscript{i}} denotes single resampled reading, and \textit{n} denotes the total number of resampled readings over the selected period. In this paper, the selected period is from 5 April 2021 12:00 a.m. (CET) to 31 May 2021 12:00 a.m. (CET).
\item   Monthly cycles: This cycle is determined by computing the central moving average (MA) for each reading, which is the arithmetic mean (see Equation~\ref{eq:sensing_avg} for calculation) of all the relative humidity readings recorded over a 30-day period that includes 15 days before and 15 days after the average is computed. In this paper, relative humidity readings measured from 21 March 2021 12:00 a.m. (CET) to 15 June 2021 12:00 a.m. (CET) are used to calculate monthly cycles between 5 April 2021 12:00 a.m. (CET) and 31 May 2021 12:00 a.m. (CET).
\item	Short-term fluctuations: A short-term fluctuation is defined as the difference between a current reading and the 30-day MA calculated for that reading as mentioned above. As a result, the short-term fluctuations consider both natural seasonal variability and the stress relaxation time constant of the materials.
\end{itemize}

After calculating the average level, monthly cycles, and short-term fluctuations, the target range of relative humidity can be determined by the procedure: 
\begin{itemize}
\item    If the relative humidity is steady, there is no need to adjust the relative humidity or temperature.
\item    If the relative humidity is unsteady, the 7{th} and 93{rd} percentiles of the fluctuations recorded during the monitoring period are used to determine the lower and upper boundaries of the target range of relative humidity, respectively.
\item    The 7{th} and 93{rd} percentiles are obtained by ordering the fluctuations from the lowest negative value to the greatest positive value and picking the values below which 7{th} or 93{rd} percent of observations are found, respectively.
\end{itemize}

In this manner, 14\% of the greatest and most risky fluctuations are excluded. If the above procedure determines that the target range of relative humidity fluctuations deviates by less than 10\% from the 30-day MA relative humidity level, the calculated limit is deemed unnecessary severe and the permissible short-term fluctuations can be adjusted to 10\%.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Results and Discussion}
\label{sec:sensing_results_discussion}
This section summarizes obtained results and findings. First, the portal of the developed web application is presented. Then, the performance of system stability is shown. Finally, the fluctuation of relative humidity in the City Museum is analyzed.

\subsection{Data Visualization and Sharing}
\label{sec:sensing_data_visualization}
Fig.~\ref{fig:sensing_fig8} shows the dashboard page of the developed web application~\cite{minerva_2021} for visualizing collected sensing data. The dashboard supports viewing real-time and historical data by selecting target building (see Fig.~\ref{fig:sensing_fig8}{a}) and date range (see Fig.~\ref{fig:sensing_fig8}{b}).

\begin{figure}[!ht]
\includegraphics{figures/sensing/fig8.png}
\centering
\caption{The dashboard provides data visualization for real-time and historical data by selecting the following: (\textbf{a}) the target building, (\textbf{b}) the target date range, and (\textbf{c}) whether to resample.}\label{fig:sensing_fig8}
\end{figure}

A resampling option (see Fig.~\ref{fig:sensing_fig8}{c}) is provided to improve user experience by reducing the number of data points to be rendered in a graph. Since the data are collected every 15 s, the number of data points for each environmental parameter per day is $24\times60\times60\div15$~=~5760. Therefore, when the selected date range (see Fig.~\ref{fig:sensing_fig8}{b}) is too extensive, the total number of data points to be rendered will be huge, resulting in a long page response time and, hence, affecting the user experience. When users only need to observe the overall trend of the data, the resolution of the data can be appropriately reduced. In this case, selecting a resampling option helps to display large quantities of data faster. The adopted resampling method is that, regardless of the selected date range, 720~data points are resampled uniformly according to the time distribution. For example, if one-day historical data are selected to show, then the data points will be resampled every two minutes.

Once the target building, date range, and the decision on whether to resample are selected , the dashboard page will show the historical sensing data in separated graphs (see Figure~\ref{fig:sensing_fig9}).

\begin{figure}[!ht]
\includegraphics{figures/sensing/fig9.png}
\centering
\caption{Historical sensing data collected in the City Museum from 16 March to 23 June 2021. (\textbf{a})~Temperature, (\textbf{b}) relative humidity, (\textbf{c}) CO\textsubscript{2} concentration, (\textbf{d}) harmful gas concentration, (\textbf{e}) dust concentration, and (\textbf{f}) vibration.}\label{fig:sensing_fig9}
\end{figure}

Each graph on the dashboard page is interactive. The menu bar (see Fig.~\ref{fig:sensing_fig10}{a}) consists of common interactive options, such as Download plot, Zoom in/out, and Reset axes. Interaction can also be performed by directly clicking, dragging, and dropping the plot area. For instance, when moving the mouse cursor over the data point (see Fig.~\ref{fig:sensing_fig10}{b}), the graph supports the revelation of more information about a data point by showing a hover label near the mouse cursor.

\begin{figure}[!ht]
\includegraphics{figures/sensing/fig10.png}
\centering
\caption{The graph supports various interactive options by the following operations: (\textbf{a}) clicking the options in the menu bar and (\textbf{b}) hovering over points on the curve.}\label{fig:sensing_fig10}
\end{figure}

This study is part of a multidisciplinary cooperation project with partners from Link\"oping University-Campus Norrk\"oping, Uppsala University-Campus Gotland, and the Research Institute of Sweden (RISE) in Link\"oping and Norrevo in Norrk\"oping. To facilitate data sharing, a Download page (see Fig.~\ref{fig:sensing_fig11}) is provided for sharing collected raw data between partners.

\begin{figure}[!ht]
\includegraphics{figures/sensing/fig11.png}
\centering
\caption{The download page supports sharing collected raw data between partners.}\label{fig:sensing_fig11}
\end{figure}

All sensed data since deployment can be downloaded from this page. The data are organized in three comma-separated values (CSV) files. The descriptions for the columns of each file are as follows:
\begin{itemize}
    \item   buildings.csv
    \begin{itemize}
        \item   Id: Primary key for buildings. Each building has a unique value;
        \item   BuildingName: Name of a building.
    \end{itemize}
    \item   devices.csv
    \begin{itemize}
        \item   Id: Primary key for edge devices. Each edge device has a unique value;
        \item   DeviceName: Name of an edge device;
        \item   BuildingId: Foreign key. References the primary key of buildings.csv.
    \end{itemize}
    \item   sensing.csv
    \begin{itemize}
        \item   Id: Primary key for sensing data. Each record has a unique value;
        \item   UtcTimestampMs: Milliseconds from 1 January 1970 at Coordinated Universal Time (UTC), for indicating when the measurement was taken;
        \item   PartitionKey: Days from 1 January 1970 at UTC, for helping partition table;
        \item   DeviceId: Foreign key, references the primary key of devices.csv;
        \item   CollectorId: Unique identification for collectors under an edge device;
        \item   Humidity: Relative humidity. The real value is dividing the raw value by 100;
        \item   Temperature: Degree Celsius. The real value is dividing the raw value by 100;
        \item   CO2: CO\textsubscript{2} concentration in PPM. The raw value is the real value;
        \item   Dust: Dust concentration in pcs/L. The raw value is the real value;
        \item   AirQuality: An integer value (0--1023) mapped from output voltage (0--5 V) of the AQ sensor;
        \item   Vibration: Rising edge count in a period of 15 s.
    \end{itemize}
\end{itemize}

\subsection{System Stability}
\label{sec:sensing_system_stability}
Table~\ref{tab:sensing_tab1} shows that all the loss rate per sensor box between 5 April 2021 12:00 a.m. (CET) and 31 May 2021 12:00 a.m. (CET) was about 2\%. Therefore, there is no significant difference in the loss rate of each sensor box. The total number of data samples expected to be collected from the three sensor boxes was 967,680, the total number of lost data samples was 19,330, and the average loss rate was 2\%.

\begin{table}[!ht]
\footnotesize
\centering
\caption{The loss rate of data samples per sensor box and the average loss rate of data samples for three sensor boxes.}
\label{tab:sensing_tab1}
\begin{tabular}{@{}clrrrr@{}}
\toprule
\multicolumn{2}{c}{Sensor Box Deployed In} & Expected & Actual & Lost & Loss Rate \\ \midrule
 & The City Museum & 322,560 & 316,251 & 6309 & 1.96\% \\
 & The City Theatre & 322,560 & 316,121 & 6439 & 2.00\% \\
 & The Auditorium & 322,560 & 315,978 & 6582 & 2.04\% \\
\multicolumn{2}{l}{Total} & 967,680 & 948,350 & 19,330 & 2.00\% \\ \bottomrule
\end{tabular}
\end{table}

Metrics embedded in Azure IoT Hub and Functions are used to investigate when and where the loss happened. Fig.~\ref{fig:sensing_fig12} shows that IoT Hub received $\sim$964,540 messages, which means the number of the lost data samples between sensor boxes and IoT Hub was about 967,680 $-$ 964,540 = 3140. It is speculated that the loss between sensor boxes and IoT Hub is because access to the Internet is occasionally unstable.

\begin{figure}[!ht]
\includegraphics{figures/sensing/fig12.png}
\centering
\caption{Hourly aggregated metrics for messages sent from edge to IoT Hub between 5 April and 31 May. The total number of sent messages was $\sim$964,540. Among them, (\textbf{a}) $\sim$482,250 messages were sent between 5 April and 3 May and (\textbf{b}) $\sim$482,290 messages were sent between 3 May and 31 May.}\label{fig:sensing_fig12}
\end{figure}

Fig.~\ref{fig:sensing_fig13} shows that the function was executed $\sim$947,940 times. The count of executed times is slightly less than the actual number of collected data samples (948,350). It is speculated that this difference is caused by the counting error of metrics and the count of executed times is corrected to 948,350, which means that the number of lost data samples between IoT Hub and Functions was about 964,540 $-$ 948,350 = 16,190.

\begin{figure}[!ht]
\includegraphics{figures/sensing/fig13.png}
\centering
\caption{Hourly aggregated metrics for executed function count between 5 April and 31 May. The total executed function count was $\sim$947,940. Among them, (\textbf{a}) $\sim$474,430 function counts were executed between 5 April and 3 May and (\textbf{b}) $\sim$473,510 function counts were executed between 3 May and 31 May.}\label{fig:sensing_fig13}
\end{figure}

Therefore, $\sim$84\% of data loss occurs between the IoT Hub and Functions (see Table~\ref{tab:sensing_table2}). This is due to a shared service plan that was used to host the Function App and Azure does not provide service level agreement (SLA) for shared service plan~\cite{azure_subscription_2021}. The data loss can be easily mitigated by upgrading to service plans with SLA.

\begin{table}[!ht]
\footnotesize
\centering
\caption{A summary of location, amount, and proportion of lost data samples.}
\label{tab:sensing_table2}
\begin{tabular}{@{}lrr@{}}
\toprule
Location & Amount & Proportion \\ \midrule
Edge to IoT Hub & $\sim$3140 & $\sim$16\% \\
IoT Hub to Functions & $\sim$16,190 & $\sim$84\% \\ \bottomrule
\end{tabular}
\end{table}

Overall, the sensing system can run stably for long-term monitoring of the indoor environment of historic buildings. A uniformly distributed loss rate of $\sim$2\% is acceptable for sampling environmental data. Of course, if a lower loss rate is needed in the future, the service plan can be easily upgraded to obtain a 99.95\% SLA, which can decrease the total loss rate to $\sim$0.3\%.

\subsection{Fluctuation Analysis of Relative Humidity in the City Museum}
\label{sec:sensing_result_fluctuations}
The measured relative humidity, calculated in a monthly cycle, and average values are shown in Fig.~\ref{fig:sensing_fig14}. The average relative humidity between 5 April and 31 May was 25.7\%. From 5 April to 10 May, most relative humidity values were lower than the average. After 10 May, the relative humidity increased and most values were above the average.

\begin{figure}[!ht]
\includegraphics{figures/sensing/fig14.png}
\centering
\caption{Relative humidity readings measured during eight weeks and a monthly relative humidity cycle obtained by calculating the 30-day central moving average (MA) of the readings.}\label{fig:sensing_fig14}
\end{figure}

According to the obtained monthly cycle, the fluctuation of each sampling point for the monthly cycle was calculated. After sorting these fluctuations in ascending order, the obtained 7{th} percentile value was $-$4.0\% while the 93{rd} percentile value was 4.2\% (see Fig.~\ref{fig:sensing_fig15}). The absolute values of the 7{th} and the 93{rd} percentiles are both less than 10\%. Therefore, according to the standard, the allowable fluctuation range can be relaxed to 10\%.

\begin{figure}[!ht]
\includegraphics{figures/sensing/fig15.png}
\centering
\caption{Target range of relative humidity fluctuations. Lower and upper limits of the range are calculated as the 7{th} and the 93{rd} percentiles of the fluctuation magnitudes, respectively.}\label{fig:sensing_fig15}
\end{figure}

Fig.~\ref{fig:sensing_fig16} shows the obtained safe band and the relationship between the original measured value and the safe band. Most of the values were within the safe band. This indicates that the fluctuation of relative humidity in the City Museum is within the acceptable limit. A few points outside the safe band (around 11 May) can be regarded as abnormal points so that when detecting abnormal points, the HVAC systems can be improved to reduce fluctuations in relative humidity.

\begin{figure}[!ht]
\includegraphics{figures/sensing/fig16.png}
\centering
\caption{The safe band of relative humidity values for the City Museum.}\label{fig:sensing_fig16}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Conclusions}
\label{sec:sensing_conclusions}
This paper presents a digitalization framework for smart preservation of historic buildings implemented with a sensing system for long-term monitoring of the indoor environment. By utilizing open-source software and services provided by the Azure cloud, the developed sensing system has good scalability, portability, and stability. The field testing results of the deployment of the implemented sensor boxes so far in three historic buildings in Norrk\"oping, Sweden, have verified these advantages. The field testing results show that the implemented sensing system has a 2\% end-to-end loss rate for collecting data samples and the loss rate can be decreased to 0.3\%. The low loss rate indicates that the sensing system has high stability and meets the requirements for long-term monitoring of historic buildings. Due to COVID-19, these three buildings have been in a state of restricted opening to the outside world so that environmental data that are less affected by human activities have been collected. After gradual opening, further measurements and analysis, e.g., studying the impact of human activities on the indoor environment of historic buildings, will be performed. The research study will continue at least to the end of 2023. Therefore, further data analysis will be conducted and the analysis results will be used to provide facility managers and users with more applications and preventive maintenance can finally be realized.

\section{Acknowledgements}
The authors would like to thank Gustav Knutsson for his assistance in ordering electronic components and experimental materials. Norrevo Fastigheter AB in Norrk\"oping is acknowledged for their support and providing access to the historic buildings.

\section{Appendix}
This appendix contains a table of Azure services and their scale tiers used in this manuscript.

\begin{table}[!ht]
\footnotesize
\centering
\caption{A summary of scale tiers and key specifications of used Azure services in this manuscript.}
\label{tab:sensing_tab3}
\begin{tabular}{@{}lll@{}}
\toprule
Azure Service & Scale Tier & Key Specifications \\ \midrule
IoT Hub & Standard S1 & \begin{tabular}[c]{@{}l@{}}400 K messages/day per unit\\ 4 KB message meter size\end{tabular} \\
Functions & Shared Environment (Windows) & \begin{tabular}[c]{@{}l@{}}1 GB disk space\\ Shared compute\end{tabular} \\
SQL Database & Basic & \begin{tabular}[c]{@{}l@{}}2 GB storage size\\ 5 DTUs\end{tabular} \\
Blob Storage & Standard/Hot & \begin{tabular}[c]{@{}l@{}}Milliseconds latency\\ Low access lost\end{tabular} \\
Web App & Basic Dedicated Environment (Linux) & \begin{tabular}[c]{@{}l@{}}10 GB disk space\\ Dedicated compute\end{tabular} \\ \bottomrule
\end{tabular}
\end{table}

\printbibliography[heading=subbibliography]
\end{refsection}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../demothesis"
%%% End: 


==> papers/ni_study_2023.tex <==
\begin{abstract}
Building energy forecasting facilitates optimizing daily operation scheduling and long-term energy planning. Many studies have demonstrated the potential of data-driven approaches in producing point forecasts of energy use. Despite this, little work has been undertaken to understand uncertainty in energy forecasts. However, many decision-making scenarios require information from a full conditional distribution of forecasts. This study has adapted and applied state-of-the-art deep learning architectures to address the problem of multi-horizon building energy forecasting. Eight different methods, including seven deep learning-based ones, were investigated to develop models to perform point and probabilistic forecasts. A comprehensive case study was conducted in two public historic buildings with different operating modes, namely the City Museum and the City Theatre, in Norrk\"oping, Sweden. The performance of the developed models was evaluated, and the predictability of different scenarios of energy consumption was studied. The results show that incorporating future information on exogenous factors that determine energy use is critical for making accurate multi-horizon predictions. Furthermore, changes in the operating mode and activities held in a building bring more uncertainty in energy use and deteriorate the prediction accuracy of models. The temporal fusion transformer (TFT) model exhibited strong competitiveness in performing both point and probabilistic forecasts. As assessed by the coefficient of variance of the root mean square error (CV-RMSE), the TFT model outperformed other models in making point forecasts of both types of energy use of the City Museum (CV-RMSE 29.7\% for electricity consumption and CV-RMSE 8.7\% for heating load). When making probabilistic predictions, the TFT model performed best to capture the central tendency and upper distribution of heating load of the City Museum as well as both types of energy use of the City Theatre.
\end{abstract}

% \begin{keywords}
% building energy forecasting, probabilistic forecast, deep learning, quantile regression, prediction interval
% \end{keywords}

% \begin{category}
%   H.5.3, H.5.4%,M.1, M.4
% \end{category}

% \sloppy{}
\begin{refsection}

\section{Introduction}
\label{sec:study_introduction}

Building energy forecasting is essential for energy efficiency, lowering energy use and greenhouse gas emissions. For example, short-term energy forecasting (for the next several hours or a few days) gives valuable references to facility managers. Maintainers can thus optimize daily operation scheduling~\cite{runge_review_2021} and design cost-effective energy-saving methods~\cite{fan_assessment_2019} while still ensuring the functions of a building. Medium- and long-term forecasting are useful for renovating buildings, e.g., examining a design during an early phase~\cite{olu_building_2022}, as well as government policy-making for energy planning~\cite{zhang_review_2021}. In addition to the demand side, building energy forecasting is also critical to the supply side. For instance, because of the rising energy demand (in 2021, 30\% of the world's total energy use was attributed to the operation of buildings~\cite{delmastro_buildings_2022}), energy companies must manage energy production more efficiently~\cite{lara_temporal_2020}. Accurate demand forecasting enables these companies to obtain sustainable production plans. However, accurate and reliable building energy forecasting also has challenging issues. On the one hand, energy systems of a building or a cluster of buildings can be complex and dynamic due to trend, seasonality and irregularity~\cite{zhang_review_2021}. On the other hand, various exogenous factors, such as outdoor climate, thermal characteristics of a building envelope, and occupants' energy use habits, can affect the energy consumption of a building~\cite{amasyali_review_2018, somu_deep_2021}. For example, thermal characteristics of a building envelope, e.g., insulation levels, determine the amount of heat gained or lost through the envelope, which affects the energy required to maintain a comfortable indoor temperature.

Methods for building energy forecasting can be broadly classified into three categories: physical, data-driven, and hybrid approaches that integrate physical and data-driven approaches. Physical approaches adopt thermodynamic rules for precise energy modeling and analysis. They often rely on building energy simulation software, e.g., EnergyPlus~\cite{crawley_energyplus_2001}, to calculate the energy consumption of a building based on characteristics of the building structure, design specifications of heating, ventilation, and air-conditioning (HVAC) systems and lighting systems, operation schedules, as well as indoor or outdoor climate~\cite{amasyali_review_2018}. Physical approaches have benefits in interpreting results and are excellent at simulating energy consumption during the design phase~\cite{qiao_towards_2021}. However, the dependency on building characteristics limits the application scenario of physical approaches since many historic buildings lack such data, and it is labor-intensive to obtain these data or even not allowed to obtain them due to regulations concerning preservation. In contrast to physical approaches, detailed physical characteristics of building structures are not necessary for data-driven approaches~\cite{khalil_machine_2022}. Data-driven approaches leverage historical energy consumption and other data to develop predictive models. These data are becoming more readily available with the digital transformation in buildings, for example, deploying monitoring systems~\cite{ni_sensing_2021} through integration of Internet of Things devices and cloud computing~\cite{liu_methodology_2021, ni_link_2022}. Therefore, it is necessary to fully utilize the accumulated data to create advanced data-driven energy forecasting models for optimizing building operations.

Deep learning methods have emerged among data-driven approaches in recent years due to their enhanced ability to address massive volumes of data, extract features, and model nonlinear processes~\cite{runge_review_2021}. Open-source frameworks like PyTorch~\cite{paszke_pytorch_2019} have also dramatically simplified network implementation and model training. There have been many studies using deep learning techniques, such as recurrent neural network (RNN) and its variants~\cite{fan_assessment_2019, kong_short-term_2019, zhang_hybrid_2020, kim_sequence_2021}, temporal convolutional network (TCN)~\cite{lara_temporal_2020}, and attention mechanism-based network~\cite{wang_transformer_2022, dong_short_2023}, for one-step-ahead or multi-horizon building energy forecasting. Nevertheless, most studies focused on point forecast, that is, forecasting the conditional mean or median of future values of the target energy consumption. Only limited cases~\cite{o_development_2016} studied probabilistic forecast.

Recently, probabilistic forecasting has grown in popularity because it can extract deeper information from historical data and better capture future uncertainty~\cite{chen_probabilistic_2020}. Many decision-making scenarios require more information from a probabilistic forecasting model that returns the full conditional distribution rather than a point forecasting model that merely forecasts the conditional mean~\cite{wen_multi-horizon_2017}. In addition, limited work~\cite{kim_sequence_2021} adopted the operational data, such as opening hours and occupancy, of buildings as features for making multi-horizon predictions. On the one hand, this may be related to the building type of the case study. On the other hand, data collection is also tricky. Nevertheless, scheduling, such as opening hours and activity arrangements, is critical for public buildings because it determines public access and energy consumption.
Moreover, in terms of predicted energy use, most deep learning-based studies only predict total energy consumption or one particular type. Further comparisons of the predictability of various types of energy use are needed. Furthermore, previous research mainly selected three types of buildings for case studies: residential, office, and educational. Limited work chose public historic buildings as case studies. However, energy forecasting is equally important for these buildings to optimize daily operations while maintaining functionality and preserving heritage values~\cite{ni_improving_2021}.

This study aims to use state-of-the-art deep learning architectures to address the problem of multi-horizon building energy forecasting. In addition to performing point forecasts, we involve probabilistic forecasts to measure and interpret the uncertainties in forecasts. Moreover, we propose to incorporate future information on exogenous factors, especially the operational data of a building, to improve the accuracy of multi-horizon forecasting. The main contributions of the paper are:
\begin{itemize}
  \item In addition to linear regression, we adapted and applied seven deep learning architectures, including hierarchical interpolation for time series forecasting (N-HiTS), TCN, Transformer (TF), NLinear, long short-term memory (LSTM), gated recurrent unit (GRU), and temporal fusion transformer (TFT), to the field of multi-horizon building energy forecasting. Among them, N-HiTS and NLinear were improved to support performing probabilistic forecasts based on quantile regression.
  \item A comprehensive case study was conducted in two public historic buildings with different operating modes to evaluate the performance of developed models. The obtained results provide insights for subsequent studies of public historic buildings with similar operating modes. The findings indicate that involving strong influencing factors makes energy consumption more predictable. Moreover, incorporating future information on exogenous factors that determine energy use is critical for enhancing multi-horizon building energy forecasting. The TFT model shows competitiveness in both point and probabilistic forecasts. Furthermore, involving building operational data, such as opening hours, can improve the prediction accuracy of models.
\end{itemize}

The remainder of this paper is organized as follows. After discussing related work in Section~\ref{sec:study_related_work}, the detailed methodology for conducting this study is described in Section~\ref{sec:study_methodology}. Then, a case study, including a detailed description of the dataset and experimental setup, is given in Section~\ref{sec:study_case_study}. After that, Section~\ref{sec:study_results_and_discussion} presents and discusses the obtained results. The last section concludes the paper.

\section{Related Work}
\label{sec:study_related_work}

Energy consumption of a building is a form of time series, a sequence of values recorded over time (typically at constant intervals) and organized chronologically~\cite{torres_deep_2021}. Therefore, this section starts with foundational deep learning methods and recent architectures for time series forecasting. Then, studies on deep learning-based building energy forecasting are presented.

\subsection{Foundational Deep Learning Methods for Time Series Forecasting}

Fully connected networks have limitations in extracting temporal dependencies of a time series. As a result, more specialized deep learning architectures, such as RNNs, convolutional neural networks (CNNs), and attention mechanism-based networks, began gaining prominence in time series forecasting. Vanilla RNN has a hidden state that serves as a concise summary of previous inputs in a sequence. The hidden state is recursively updated at each time step after processing new inputs. However, the vanishing and expanding gradient problems limit the learning ability of vanilla RNNs. Two variants of RNNs, namely LSTM~\cite{hochreiter_long_1997} and GRU~\cite{cho_properties_2014}, address the gradient problems. LSTM employs three gates to retain long-standing essential information while discarding nonessential information. GRU simplifies LSTM and is computationally faster than LSTM since it only has two gates.

Recent research suggests that specific CNNs can achieve state-of-the-art accuracy in various application domains of sequence modeling, such as audio synthesis and autonomous driving~\cite{zhang_social_2021, zhang_learning_2022}. CNNs are built with convolution, pooling, and fully connected layers~\cite{lecun_comparison_1995}. The convolution layers learn features from input data by filters with a predefined size. Then, pooling layers process the convolution results by average or maximum pooling. Finally, the flattened features produced by the convolutional and pooling layers provide the input for fully connected layers to perform the forecasting. Parallelism is an essential advantage of CNNs, as convolutions can be performed in parallel because the same filter is used in each layer.

There is a growing interest in understanding how and why a model makes a particular prediction. Based on a better understanding of temporal dynamics and the rationale behind a forecast, decision-makers can improve their actions further. Attention mechanism~\cite{bahdanau_neural_2014} has become an intrinsic part of sequence modeling in various tasks. The attention mechanism is a key-value lookup technique depending on a provided query. For time series modeling, the output of the attention layer can be interpreted as a weighted average across temporal features. An analysis of attention weights can thus determine the relative importance of features at each time step~\cite{lim_time_series_2021}. 

\subsection{Recent Deep Learning Architectures for Time Series Forecasting}

Recent competitive deep learning architectures for time series forecasting are mainly built on previous advances. RNN (and its variants)-based architectures include MQ-RNN~\cite{wen_multi-horizon_2017} and DeepAR~\cite{salinas_deepar_2020}. Both MQ-RNN and DeepAR aim to handle the challenge of large-scale time series forecasting. Rather than predicting each time series individually, they learn a global model from historical data for all time series in a dataset. Meanwhile, they both employ an LSTM for encoding all historical information into hidden states. Unlike DeepAR uses an LSTM as the recursive decoder when generating forecasts, MQ-RNN adopts two multilayer perceptron branches. In addition, while DeepAR is trained using maximum likelihood and teacher forcing (feeding ground truth recursively in training)~\cite{salinas_deepar_2020}, MQ-RNN uses a more efficient training technique and generates quantile forecasts directly~\cite{wen_multi-horizon_2017}.

Convolution-based architectures include MQ-CNN~\cite{wen_multi-horizon_2017}, TCN~\cite{bai_empirical_2018}, and DeepTCN~\cite{chen_probabilistic_2020}. MQ-CNN has a similar architecture with MQ-RNN by just replacing the encoder with a stack of dilated causal 1D convolution layers~\cite{oord_wavenet_2016}. Bai et al.~\cite{bai_empirical_2018} built TCN by condensing dilated and causal convolution. In addition, TCN employs a generic residual module~\cite{he_deep_2016} for stabilization. Based on TCN, Chen et al.~\cite{chen_probabilistic_2020} proposed DeepTCN as a non-autoregressive probabilistic forecasting framework for large-scale related time series. Like MQ-CNN, DeepTCN follows an encoder-decoder design.

A representative of attention-based architectures is Transformer~\cite{vaswani_attention_2017}. While the attention mechanisms are used together with RNN in many cases, Vaswani et al.~\cite{vaswani_attention_2017} proposed the Transformer, which relies entirely on attention mechanisms to draw global dependencies between input and output. Self-attention enables linking different positions in the sequence, while multi-head attention enables the model to attend to information from distinct representation subspaces at different points~\cite{vaswani_attention_2017}. Based on Transformer, FEDformer~\cite{zhou_fedformer_2022} further incorporates classical time series analysis techniques like frequency processing through Fourier transformation. Lim et al.~\cite{lim_temporal_2021} created TFT using canonical components, such as gated residual network, LSTM, and multi-head attention. Gating mechanisms enable TFT to skip over any unused components of the architecture, providing adaptive depth and network complexity to accommodate a wide range of datasets and scenarios. Some studies questioned the validity of Transformer-based solutions for long-term time series forecasting tasks. For example, Zeng et al.~\cite{zeng_transformers_2022} proposed a simple direct multi-step model through a linear temporal layer named LTSF-Linear. In many cases, it outperforms FEDformer~\cite{zhou_fedformer_2022} on multi-horizon forecasting of multivariate time series.

Some architectures are based on a deep stack of fully connected layers, such as N-BEATS~\cite{oreshkin_n-beats_2019} and its improved version N-HiTS~\cite{challu_n-hits_2022}. Oreshkin et al.~\cite{oreshkin_n-beats_2019} proposed N-BEATS, an architecture built on backward and forward residual links and a very deep stack of fully connected layers. Challu et al.~\cite{challu_n-hits_2022} enhanced the N-BEATS architecture by improving its input decomposition through multi-rate data sampling and its output synthesizer through multi-scale interpolation. N-HiTS adds sub-sampling layers before fully-connected blocks in N-BEATS. This modification dramatically decreased the required computation and memory usage while retaining the capacity to capture long-term dependencies. 

\subsection{Deep Learning-based Building Energy Forecasting}
 
Many studies have employed deep learning to predict the energy consumption of buildings. The architectures used include RNN and its variants~\cite{fan_assessment_2019, kong_short-term_2019, zhang_hybrid_2020, kim_sequence_2021}, TCN~\cite{lara_temporal_2020}, attention-based~\cite{wang_transformer_2022, dong_short_2023}, and hybrid models~\cite{somu_deep_2021, wang_short-term_2021, gao_interpretable_2021} that combine multiple architectures. Both one-step ahead~\cite{kong_short-term_2019, zhang_hybrid_2020, wang_short-term_2021, gao_interpretable_2021, zhang_accurate_2020} and multi-horizon forecasting~\cite{fan_assessment_2019, lara_temporal_2020, somu_deep_2021, kim_sequence_2021, wang_transformer_2022, dong_short_2023, lei_building_2021} were investigated. However, most studies only performed point forecasts. Furthermore, there is a need for studies that apply cutting-edge competitive architectures, such as TFT and N-HiTS, to building energy forecasting and a thorough comparison of these most recent and older architectures.

Most studies used energy data from residential~\cite{olu_building_2022, kong_short-term_2019, dong_short_2023}, educational~\cite{fan_assessment_2019, somu_deep_2021, wang_transformer_2022}, and office buildings~\cite{kim_sequence_2021, gao_interpretable_2021}. Models were mainly developed using time granularity of hourly and sub-hourly data, and only a few~\cite{gao_interpretable_2021, lei_building_2021} used daily data. The time span of data in most datasets was less than three years, and only a few studies employed datasets longer than three years~\cite{lara_temporal_2020, wang_transformer_2022, gao_interpretable_2021}. For the type of predicted energy use, most studies only predicted one kind or total energy consumption. Few studies used public historic buildings for case studies. However, energy forecasting is also critical for these buildings to optimize daily operations while maintaining their functionalities and preserving heritage values.

Outdoor weather and historical energy consumption were the most commonly used features for predicting energy consumption, regardless of building type. In contrast, data about occupants' behavior~\cite{kim_sequence_2021} was rarely utilized. This preference for features is primarily due to more readily available outdoor weather data. Outdoor weather, for example, can be gathered from many public databases. However, privacy policies make obtaining features such as occupants' behavior challenging~\cite{qiao_towards_2021}. Other used features include indoor environmental parameters, such as room temperature and relative humidity, as well as temporal features, e.g., the type of day (weekday, weekend, or holiday) and the type of hour (daytime or nighttime)~\cite{amasyali_review_2018}. Building operational data like opening hours and scheduling of HVAC systems were rarely used. Nevertheless, involving available operational data can potentially increase the prediction accuracy of models, especially for public buildings where energy consumption is highly correlated with held activities.

\subsection{Innovation of This Study}

This study adapted and applied state-of-the-art deep learning architectures to multi-horizon building energy forecasting. A comprehensive case study was conducted in two public historic buildings to compare the performance of various models. While previous studies mainly focused on point forecasts, we also investigated probabilistic forecasts. Quantile regression was adopted to achieve a complete understanding of the distribution of energy consumption. Regarding features, we proposed incorporating future information on factors that determine energy use, especially data related to building operations, to improve prediction accuracy. Furthermore, the predictability of different types of energy consumption inside the same building and between buildings with different operating modes was studied. These efforts could bring inspiration to predicting energy use and optimizing energy efficiency of public buildings, especially historic buildings.

\section{Methodology}
\label{sec:study_methodology}

This section begins by formulating the problem of multi-horizon building energy forecasting. Then, the encoder-decoder architecture is described. After that, seven deep learning architectures for comparison are given. Finally, the loss function for model training and metrics for evaluating model performance are introduced.

\subsection{Problem Formulation}

This study considers the problem of multi-horizon forecasting for energy consumption of buildings.
We denote a specific type of energy use, i.e., the target variable, as a non-negative real variable $y\in \mathbb{R}_{+}$.
Predictor variables that might affect the energy use are divided into two parts: observable in the past (i.e., before (including) a forecast origin, see Fig.~\ref{fig:study_fig1}) and observable in the future (i.e., after the forecast origin).
The former is denoted as a real row vector $\mathbf{x_{b}} \in \mathbb{R}^{k}$ while the latter is denoted as a real row vector $\mathbf{x_{f}} \in \mathbb{R}^{m}$.
All target and predictor variables are assumed to be observed across time at constant intervals and organized chronologically.
At time $t$, the observed value of the target variable is denoted as ${y}_{t}$.
Similarly, observed values of predictor variables are denoted as $\mathbf{x_{b}}_{t} =[{x_{b}}_{1,t} ,{x_{b}}_{2,t} ,...,{x_{b}}_{k,t}]$ and $\mathbf{x_{f}}_{t} =[{x_{f}}_{1,t} ,{x_{f}}_{2,t} ,...,{x_{f}}_{m,t}]$, respectively.

\begin{figure}[!ht]
\includegraphics{figures/study/fig1.png}
\centering
\caption{An illustration of multi-horizon building energy forecasting. In this example, black dots are observed values of a specific type of energy consumption over a lookback window ($size=10$) in the past. Blue triangles are predicted values (conditional mean or median) of the energy consumption over a forecast horizon ($size=6$) in the future. The shadow area represents a particular prediction interval.}\label{fig:study_fig1}
\end{figure}

Then, a point energy forecasting model takes the form
\begin{equation}
\hat{y}_{t+1:t+h} =f_{\theta }(y_{t-w+1:t} ,\mathbf{x_{b}{}}_{t-w+1:t} ,\mathbf{x_{f}{}}_{t+1:t+h}), \label{eqn:study_point_forecast}
\end{equation}
where $\hat{y}_{t+1:t+h} = \left[\hat{y}_{t+1},\hat{y}_{t+2},...,\hat{y}_{t+h}\right] \in \mathbb{R}_{+}^{h}$ are model forecasts for mean values of the target variable over a forecast horizon $h$, $y_{t-w+1:t} = [y_{t-w+1} ,y_{t-w+2} ,...,y_{t}] \in \mathbb{R}_{+}^{w}$ as well as $\mathbf{x_{b}}_{t-w+1:t} = \{\mathbf{x_{b}}_{t-w+1} ,\mathbf{x_{b}}_{t-w+2} ,...,\mathbf{x_{b}}_{t}\}$ are observations of the target and predictor variables over a loopback window $w$, $\mathbf{x_{f}}_{t+1:t+h} =\{\mathbf{x_{f}}_{t+1} ,\mathbf{x_{f}}_{t+2} ,...,\mathbf{x_{f}}_{t+h}\}$ are observations of predictor variables over the forecast horizon $h$, and $f_{\theta}{(.)}$ is the prediction function learnt by the model.

For developing probabilistic forecasting models, we do not assume that energy consumption follows some distributions but develop models that generate interested quantiles directly. Quantile forecasts are performed through quantile regression~\cite{koenker_regression_1978}. The $p$th quantile denotes the value where the cumulative distribution function crosses $p$~\cite{hao_quantile_2007}. Thus, quantiles can specify any position of a distribution.

Given a predetermined set of quantiles $\mathcal{Q} \subset (0,1)$, a quantile energy forecasting model takes the form
\begin{equation}
\hat{y}_{t+1:t+h}^{(p)} =g_{\theta}(y_{t-w+1:t} ,\mathbf{x_{b}{}}_{t-w+1:t} ,\mathbf{x_{f}{}}_{t+1:t+h}), \label{eqn:study_quantile_forecast}
\end{equation}
where $p$ is an element of the set $\mathcal{Q}$, $\hat{y}_{t+1:t+h}^{(p)} = \left[\hat{y}_{t+1}^{(p)} ,\hat{y}_{t+2}^{(p)} ,...,\hat{y}_{t+h}^{(p)}\right] \in \mathbb{R}_{+}^{h}$ are the model forecasts for the $p$th quantile of the target variable over a predicting horizon $h$, $y_{t-w+1:t}$, $\mathbf{x_{b}}_{t-w+1:t}$ and $\mathbf{x_{f}}_{t+1:t+h}$ have the same definition as in the point forecasting model, and $g_{\theta}{(.)}$ is the prediction function learnt by the model.

\subsection{The Encoder-Decoder Architecture}

Most competitive sequential transduction models employ an encoder-decoder architecture~\cite{vaswani_attention_2017}. This design decouples handling inputs and generating outputs into two separate stages and works much better. The encoder converts an input sequence to a sequence of representations called hidden states. Given hidden states, the decoder generates an output sequence of target variables. Specific to the problem of building energy forecasting, Fig.~\ref{fig:study_fig2} illustrates a design that supports incorporating past and future information for predicting multi-horizon energy consumption. The encoder takes observations of the target and predictor variables over the loopback window as input. The target and predictor variables are concatenated as input at each time step in the look-back window. Then, the encoder outputs a summary of past information. The decoder takes the summary and observations of predictor variables over the forecast horizon as input and outputs the quantile forecasts. At each time step during the forecast horizon, the decoder outputs a set of predetermined quantile forecasts. Point forecast adopts the same architecture, except it outputs only one predicted value (conditional mean) at each time step during the forecast horizon.

\begin{figure}[!ht]
\includegraphics{figures/study/fig2.png}
\centering
\caption{A high-level illustration of the encoder-decoder architecture. The encoder takes observations of a target variable $y$ and predictor variables $\mathbf{x_{b}}$ over the loopback window as input. At each time step in the lookback window, the observations of target and predictor variables are concatenated. The encoder outputs a representation of the information in $\mathbf{z}_\mathit{encoded}$. The decoder takes the representation as well as observations of predictor variables $\mathbf{x_{f}}$ over the forecast horizon as input and outputs the quantile forecasts. At each time step during the forecast horizon, the decoder outputs a set of predetermined quantile forecasts.}\label{fig:study_fig2}
\end{figure}

\subsection{Deep Learning Architectures for Comparison}

In addition to linear regression (LR), seven deep learning architectures, namely N-HiTS~\cite{challu_n-hits_2022}, TCN~\cite{bai_empirical_2018}, Transformer (TF)~\cite{vaswani_attention_2017}, NLinear~\cite{zeng_transformers_2022}, LSTM~\cite{hochreiter_long_1997}, GRU~\cite{cho_properties_2014}, and TFT~\cite{lim_temporal_2021}, were investigated to develop predictive models and compare their performance in multi-horizon building energy forecasting. For simplicity, this paper does not give the detailed design of these architectures. The LR model makes predictions based on a linear relationship between the target variable and past and future values of some predictor variables. Among the seven deep learning architectures, N-HiTS, TCN, and TF only support incorporating past values of target and predictor variables for making predictions. Other four architectures, NLinear, LSTM, GRU, and TFT, support incorporating past values of target variables and past and future values of predictor variables. Moreover, architectures, such as N-HiTS and NLinear, were improved to support producing probabilistic forecasts based on quantile regression. 

Ensemble methods are not used in this study since any deep learning algorithm can profit from model averaging at the expense of extra computation and memory~\cite{goodfellow_deep_2016}.

\subsection{Loss Function and Evaluation Metrics}
\label{sec:study_loss_func_eval_metric}

Point forecasting models were trained on a training set to minimize the total  squared error, which leads to forecasts of the mean~\cite{hyndman_forecasting_2018}. The training squared error for a set $\mathcal{S} =\{(y_{t-w+1:t} ,\mathbf{x_{b}{}}_{t-w+1:t} ,\mathbf{x_{f}{}}_{t+1:t+h} ,y_{t+1:t+h})\}_{t=w}^{n+w-1}$ is denoted by $L_{s}(\mathbf{\theta})$, and
\begin{equation}
L_{s}(\theta) = \sum _{t=w}^{n+w-1}\sum _{i=1}^{h} \left(\hat{y}_{t+i} -y_{t+i}\right)^{2}, \label{eqn:study_square_loss}
\end{equation}
where $n$ denotes the number of training samples and definitions of other variables are as in Eq.~\ref{eqn:study_point_forecast}.

Probabilistic forecasting models, i.e., quantile forecasting models in this study, were trained to minimize the total quantile loss. As in studies~\cite{wen_multi-horizon_2017, lim_temporal_2021}, the $p$th quantile loss for one prediction at one time step is calculated as 
\begin{equation}
\ell(\hat{y} ,y,p)=(1-p)(\hat{y} -y)_{+} + p(y-\hat{y})_{+}, \label{eqn:study_quantile_loss}
\end{equation}
where $(.)_{+}=max(0,.)$. Then, the training quantile loss for a set $\mathcal{S} =\{(y_{t-w+1:t} ,\mathbf{x_{b}{}}_{t-w+1:t} ,\mathbf{x_{f}{}}_{t+1:t+h} ,y_{t+1:t+h})\}_{t=w}^{n+w-1}$ is denoted by $L_{q}(\theta)$, and
\begin{equation}
L_{q}(\theta) =\sum _{t=w}^{n+w-1}\sum _{j=1}^{| \mathcal{Q}| }\sum _{i=1}^{h} \ell \left(\hat{y}_{t+i}^{( p_{j})} ,y_{t+i} ,p_{j}\right),
\end{equation}
where $\mathcal{Q}$ denotes a predetermined set of quantiles and $p_{j}$ is an element of $\mathcal{Q}$.

The performance of developed models was compared through two aspects: prediction accuracy and computational cost. The computational cost was expressed as the training time of each model in seconds. As suggested by the ASHRAE Guideline 14-2014~\cite{ashrae_guideline_14_measurement_2014}, the prediction accuracy of point forecasting models was evaluated by two scale-independent metrics, namely coefficient of variation of the root mean square error (CV-RMSE) and normalized mean bias error (NMBE), over the entire test set. They are calculated by Eq.~\ref{eqn:study_cv-rmse} and~\ref{eqn:study_nmbe}.
\begin{equation}
RMSE=\sqrt{\frac{1}{n}\sum\limits _{t=1}^{n}(\hat{y}_{t} -y_{t})^{2}}, \label{eqn:study_rmse}
\end{equation}
\begin{equation}
CV\textrm{-}RMSE=\frac{RMSE}{\overline{y}} \times 100, \label{eqn:study_cv-rmse}
\end{equation}
\begin{equation}
MBE=\frac{1}{n}\sum\limits _{t=1}^{n}(\hat{y}_{t} -y_{t}), \label{eqn:study_mbe}
\end{equation}
\begin{equation}
NMBE=\frac{MBE}{\overline{y}} \times 100,  \label{eqn:study_nmbe}
\end{equation}
where $n$ denotes the size of forecast horizon, $y_{t}$ is the actual value of a target variable at time $t$, $\hat{y}_{t}$ is the predicted value of the target variable at time $t$, and $\overline{y}$ is the mean actual value of the target variable over the forecast horizon.

The CV-RMSE measures the variation between the actual values and the predictions of a model~\cite{ashrae_guideline_14_measurement_2014}. NMBE normalizes the mean bias error and gives the global difference between the actual and predicted values~\cite{ramos_validation_2017}. A positive NMBE value means that the model over-predicts actual energy consumption, and a negative one means under-prediction. For both CV-RMSE and NMBE, a closer value to zero represents better prediction accuracy. When making comparisons, we mainly focused on the CV-RMSE if the NMBE of a model is within the required range. As suggested by the ASHRAE Guideline 14-2014~\cite{ashrae_guideline_14_measurement_2014}, an applicable predictive model for energy use of whole building should have a CV-RMSE $\leq$~30\% and an NMBE within $\pm$10\% when using hourly data for training models. 

As in studies~\cite{salinas_deepar_2020,lim_temporal_2021}, the $\rho$-risk, which normalizes quantile losses across the entire forecast horizon, was used for evaluating the performance of probabilistic forecasting models. $\rho$-risk at $p$th quantile is calculated by
\begin{equation}
\rho\textrm{-}risk(p) =\frac{2\times \sum\limits _{t=1}^{n} \ell \left(\hat{y}_{t}^{(p)} ,y_{t} ,p\right)}{\sum\limits _{t=1}^{n} y_{t}}, \label{eqn:study_rho_risk}
\end{equation}
where $n$ denotes the size of forecast horizon, $y_{t}$ is the actual value of a target variable at time $t$, $\hat{y}_{t}^{(p)}$ denotes the predicted $p$th quantile value at time $t$, and $\ell \left(\hat{y}_{t}^{(p)} ,y_{t} ,p\right)$ is the $p$th quantile loss calculated by Eq.~\ref{eqn:study_quantile_loss}. 

\section{Case Study}
\label{sec:study_case_study}

To verify the performance of different deep learning architectures, a case study was conducted to develop predictive models for the energy consumption of two public historic buildings. This section describes details of the used dataset and experimental setup. The obtained results and discussion will be presented in Section~\ref{sec:study_results_and_discussion}.

\subsection{Dataset}
\label{sec:study_dataset}
The dataset consists of two parts. One is the historical energy consumption data from two public historic buildings: the City Museum (Fig.~\ref{fig:study_fig3}{a}) and the City Theatre (Fig.~\ref{fig:study_fig3}{b}) in Norrk\"oping, Sweden. The other is the meteorological data of Norrk\"oping. The energy consumption data (see Fig.~\ref{fig:study_fig4}) are electricity use and heating load provided by the building maintainer. Heating energy comes from the district heating system. Both types of energy use data are of the entire building. The meteorological data include dry-bulb temperature, relative humidity, dew point temperature, precipitation, air pressure, wind speed, and global irradiance. The meteorological data are obtained through open application programming interfaces (APIs) provided by the Swedish Meteorological and Hydrological Institute. The global irradiance is collected according to the latitude and longitude of the buildings, while other meteorological data are from a weather station located $\sim$2~km away from the two buildings. All energy consumption and meteorological data range from 01:00 on January 1, 2016 to 00:00 on January 1, 2020, with a time granularity of one hour. Hours appearing in this paper are expressed in 24-hour format and are all in local time (Greenwich Mean Time (GMT) +1 for summer time and GMT +2 for winter time). The time span of the collected data is before the pandemic of COVID-19, which means that it excludes the impact of COVID-19 on public activities held in these two buildings.

\begin{figure}[!ht]
\includegraphics{figures/study/fig3.png}
\centering
\caption{A case study was conducted in two public historic buildings: (\textbf{a}) the City Museum and (\textbf{b}) the City Theatre in N\"orrkping, Sweden.}\label{fig:study_fig3}
\end{figure}

\begin{figure}[!ht]
\includegraphics[width=\textwidth]{figures/study/fig4.png}
\centering
\caption{Historical hourly (\textbf{a}) electricity consumption and (\textbf{b}) heating load of the City Museum, as well as (\textbf{c}) electricity consumption and (\textbf{d}) heating load of the City Theatre in Norrk\"oping, Sweden from 01:00 on January 1, 2016 to 00:00 on January 1, 2020. Hours appearing in this paper are expressed in 24-hour format and are all in local time.}\label{fig:study_fig4}
\end{figure}

These two public historic buildings have different operating modes. The normal operation of the City Museum is to maintain an appropriate indoor climate for preservation of collections and human comfort of staff and visitors. As shown in Table~\ref{tab:study_tab1}, the City Museum has regular opening hours. For the City Theatre, the operation mainly serves the delivery of live shows to audiences. For example, sound and light equipment and the ventilation system should work during a show or rehearsal. The performed shows have some seasonality. Several shows of the same production are typically performed in adjacent 2--4 weeks. For example, 16 shows of the production \textit{Farmor och V\aa{r} Herre} were performed during the period of February 24 to March 18, 2018. If a show is performed on one day, the start time is usually 19:00 on working days, 18:00 on Saturdays, and 16:00 on Sundays. Long shows last around three hours. In addition, shows are generally not performed on Mondays. 

\begin{table}[!ht]
\centering
%\footnotesize
\caption{Opening hours of the City Museum. Normally, it is open for six days, from Tuesday to Sunday every week. The opening hours will change in some holidays. On the day before Christmas Eve (December 23) and Epiphany (January 6), it opens from 11:00 to 16:00. On Christmas Eve (December 24), Christmas Day (December 25), and New Year's Day (January 1), it is closed.}
\label{tab:study_tab1}
\begin{tabular}{@{}lrlr@{}}
\toprule
 & \multicolumn{1}{c}{June--August} & \phantom{} & \multicolumn{1}{c}{In other months} \\ \midrule
Monday & Closed &  & Closed \\
Tuesday & 12:00--16:00 &  & 11:00--17:00 \\
Wednesday & 12:00--16:00 &  & 11:00--17:00 \\
Thursday & 12:00--20:00 &  & 11:00--20:00 \\
Friday & 12:00--16:00 &  & 11:00--17:00 \\
Saturday & 12:00--16:00 &  & 11:00--16:00 \\
Sunday & 12:00--16:00 &  & 11:00--16:00 \\ \bottomrule
\end{tabular}
\end{table}

The different operating modes of the two buildings could verify the adaptability of different predictive models to some extent. The distinctions in operating modes can be reflected in the electricity consumption of the two buildings. Due to regular opening hours, the pattern in electricity consumption of the City Museum (see Fig.~\ref{fig:study_fig4}{a}) is more evident and stable. However, the irregularity of show arrangements makes electricity consumption of the City Theatre (see Fig.~\ref{fig:study_fig4}{c}) vary from year to year. Compared to the considerable dissimilarity in the pattern of electricity consumption, the pattern in heating load of the two buildings (see Fig.~\ref{fig:study_fig4}{b} and~\ref{fig:study_fig4}{d}) has a high similarity. This similarity is mainly because both buildings employ adaptive district heating, which is driven by the difference between indoor and outdoor temperatures. Generally, there is no notable trend in electricity consumption and heating load for both buildings. No long-term increase or decrease can be inspected from both type of energy consumption. Nevertheless, a yearly seasonality exists. Both electricity consumption and heating load are lower in summer and higher in winter.

\subsection{Data Preprocessing}
\label{sec:study_data_preprocessing}
Data preprocessing aims to convert the raw data into a format that can be easily handled and understood by models. In this study, data preprocessing includes data cleaning, dataset splitting, feature preparation, and data transformation.  

\subsubsection{Data Cleaning and Dataset Splitting}
\label{sec:study_data_cleaning}
First, missing values in meteorological data were interpolated linearly. Then, the dataset was divided into three subsets: a training set for learning the parameters of models, a validation set for tuning hyperparameters and preventing overfitting, and a test set for evaluating the performance of models. The dataset splitting roughly follows the empirical ratio of 80:10:10, where 38 months of data from January 1, 2016 to February 28, 2019 are used as the training set, five months of data from March 1, 2019 to July 31, 2019 are used as the validation set, and five months of data from August 1, 2019 to December 31, 2019 are used as the test set. The three subsets do not overlap in time, avoiding information leakage from the future. We did not identify and address outliers in meteorological data since the provider has ensured their validity. For the energy data, only the training set was inspected to avoid information leakage from the test set. As shown in Fig.~\ref{fig:study_fig5}, many outliers in electricity consumption of both buildings and one outlier in heating load of the City Theatre are identified. After inspecting the occurrence of these outliers, they are kept in the training set as these outliers are high energy consumption due to activities held in the buildings and are not anomalies.


\begin{figure}[!ht]
\includegraphics{figures/study/fig5.png}
\centering
\caption{The boxplot of hourly electricity consumption and heating load of the City Museum and the City Theatre from January 1, 2016 to February 28, 2019. Data points that are more than 1.5 box lengths from the edge of their box are classified as outliers, illustrated as diamond dots.}\label{fig:study_fig5}
\end{figure}

\subsubsection{Feature Preparation}
\label{sec:study_feature_prep}
Feature preparation includes extracting temporal features from timestamps, generating features from operating modes of buildings, and reducing redundant features. Four temporal features are extracted: two binary and two cyclical variables. The binary variables include one called \textit{is holiday} to indicate if a day is a Sweden public holiday and another called \textit{is weekend} to indicate if a day is a weekend. The cyclical variables are \textit{hour} (integer value from 0 to 23) and \textit{weekday} (integer value from 0 to 6, each value represents a day in a week, starting from Monday). In addition to the temporal features, one feature called \textit{is open} with a binary value is added to reflect the occupancy of a building for a given hour. For the City Museum, \textit{is open} indicates that if it is open to visitors. For the City Theatre, \textit{is open} indicates that if there is a show performed.

These features could help predict energy use. For example, there is usually a daily seasonality for operating a building. Fig.~\ref{fig:study_fig6} shows the distribution of electricity consumption per hour of the two buildings during four weeks of the training set. The electricity consumption of the City Museum (see Fig.~\ref{fig:study_fig6}{a}) was stable, and the distribution was narrow before 8:00 and after 20:00. Between 8:00 and 17:00, hourly electricity consumption rose significantly due to the work of staff and the opening to the public, and the data was distributed wider. Between 18:00 and 20:00, although the median electricity consumption decreased, many outliers appeared because the City Museum remained open until 20:00 on Thursdays. A similar phenomenon can be observed in the electricity consumption of the City Theatre. As depicted in Fig.~\ref{fig:study_fig6}{b}, the highest median electricity consumption is at 19:00 because shows performed on working days started at that time. During the show time, the distribution of electricity consumption also became wider. The heating load of the two buildings also has a similar correlation with the hour of a day (see Fig.~\ref{fig:study_fig7}), although it is not as strong as for the electricity consumption. Therefore, extracting temporal features such as hour and weekday from timestamps helps predict energy consumption. Furthermore, opening hours can also provide information for making predictions. 

\begin{figure}[!ht]
\includegraphics{figures/study/fig6.png}
\centering
\caption{The boxplot of electricity consumption per hour of (\textbf{a}) the City Museum and (\textbf{b}) the City Theatre from 00:00 on February 19 to 23:00 on March 18, 2018.}\label{fig:study_fig6}
\end{figure}

\begin{figure}[!ht]
\includegraphics{figures/study/fig7.png}
\centering
\caption{The boxplot of heating load per hour of (\textbf{a}) the City Museum and (\textbf{b}) the City Theatre from 00:00 on February 19 to 23:00 on March 18, 2018.}\label{fig:study_fig7}
\end{figure}

A filter method based on finding the correlation between variables was employed to select critical features and reduce redundant features. The Pearson correlation coefficient ($r$) was used for measuring the linear relationship between two variables. As general rules of thumb, a threshold of $|r|\geq 0.3$ was employed to filter out critical features with at least moderate correlation with a target variable. To reduce redundant features, when two features are highly correlated ($|r|\geq 0.7$), the one holding larger $|r|$ with the target variable was kept to avoid duplicate information.

As coefficients shown in Table~\ref{tab:study_tab2}, to predict electricity consumption of the City Museum, \textit{dew point temperature}, \textit{is open}, and extracted temporal features \textit{hour} and \textit{weekday} were used. To predict heating load of the City Museum, \textit{dry-bulb temperature}, \textit{relative humidity}, \textit{global irradiance}, \textit{hour}, and \textit{weekday} were used. Similarly, according to coefficients shown in Table~\ref{tab:study_tab3}, to predict electricity consumption of the City Theatre, \textit{is open}, \textit{hour}, and \textit{weekday} were used. To predict heating load of the City Theatre, \textit{dry-bulb temperature}, \textit{relative humidity}, \textit{global irradiance}, \textit{hour}, and \textit{weekday} were used.

\begin{table}[!ht]
\centering
%\footnotesize
\caption{Pearson correlation coefficient ($r$) between variables for the City Museum in the training set. Electricity and Heating are target variables, while others are features. Temperature is abbreviated as temp.. Except for the dry-bulb temperature, the coefficients between other features are not shown in the table because their $|r|<0.7$.}
\label{tab:study_tab2}
\begin{tabular}{@{}lrrr@{}}
\toprule
\multicolumn{1}{c}{} & Electricity & Heating & \begin{tabular}[c]{@{}r@{}}Dry-bulb temp.\end{tabular} \\ \midrule
Dry-bulb temp. & $-$0.466 & \textbf{$-$0.887} & 1.000 \\
Relative humidity & 0.088 & \textbf{0.384} & $-$0.562 \\
Dew point temp. & \textbf{$-$0.517} & $-$0.843 & \textbf{0.861} \\
Precipitation & $-$0.005 & $-$0.017 & 0.001 \\
Air pressure & 0.019 & 0.000 & $-$0.020 \\
Wind speed & 0.152 & 0.081 & 0.055 \\
Global irradiance & 0.127 & \textbf{$-$0.332} & 0.547 \\
Is holiday & $-$0.090 & 0.035 & $-$0.038 \\
Is weekend & $-$0.216 & $-$0.025 & $-$0.004 \\
Is open & \textbf{0.435} & 0.102 & 0.101 \\ \bottomrule
\end{tabular}%
\end{table}

\begin{table}[!ht]
\centering
%\footnotesize
\caption{Pearson correlation coefficient ($r$) between variables for the City Theatre in the training set. Electricity and Heating are target variables, while others are features. Except for the dry-bulb temperature, the coefficients between other features are not shown in the table because their $|r|<0.7$.}
\label{tab:study_tab3}
\begin{tabular}{@{}lrrr@{}}
\toprule
\multicolumn{1}{c}{} & Electricity & Heating & \begin{tabular}[c]{@{}r@{}}Dry-bulb temp.\end{tabular} \\ \midrule
Dry-bulb temp. & $-$0.102 & \textbf{$-$0.850} & 1.000 \\
Relative humidity & $-$0.057 & \textbf{0.336} & $-$0.562 \\
Dew point temp. & $-$0.152 & $-$0.826 & \textbf{0.861} \\
Precipitation & $-$0.011 & $-$0.022 & 0.001 \\
Air pressure & 0.046 & 0.011 & $-$0.020 \\
Wind speed & 0.155 & 0.087 & 0.055 \\
Global irradiance & 0.053 & \textbf{$-$0.309} & 0.547 \\
Is holiday & $-$0.090 & 0.041 & $-$0.038 \\
Is weekend & $-$0.152 & $-$0.037 & $-$0.004 \\
Is open & \textbf{0.734} & 0.153 & $-$0.066 \\ \bottomrule
\end{tabular}
\end{table}

The features that are used to predict the electricity use and heating load of the two buildings are summarized in Table~\ref{tab:study_tab4}. For predicting each target variable, past observations of itself, as well as past and future observations of predictor variables, are used. Given a forecast origin, temporal features in a forecast horizon such as \textit{hour} and \textit{weekday} are naturally known in advance. Operational features like \textit{is open} in the forecast horizon can be retrieved from APIs provided by the maintainer of a building. Values of meteorological features in the forecast horizon are also considered available, as short-term weather forecasts, i.e., for the next 24 hours, are highly accurate nowadays. Many organizations provide APIs to access them. However, it is worth noting that this study used actual meteorological data to train and evaluate the model. Therefore, the prediction performance of models might have some degradation when these models are deployed in real applications due to the use of forecasted meteorological data.

\begin{table}[!ht]
\centering
%\footnotesize
\caption{A summary of used features for predicting each target variable.}
\label{tab:study_tab4}
\begin{tabular}{@{}cll@{}}
\toprule
Target variable & \multicolumn{1}{c}{Features} & \multicolumn{1}{c}{Observable in} \\ \midrule
\multicolumn{1}{l}{\textit{The City Museum}} &  &  \\
\multirow{2}{*}{Electricity} & electricity & past \\ \cmidrule(l){3-3} 
 & \begin{tabular}[c]{@{}l@{}}dew point temp.\\ is open\\ hour\\ weekday\end{tabular} & past and future \\ \cmidrule(l){2-3} 
\multirow{2}{*}{Heating} & heating & past \\ \cmidrule(l){3-3} 
 & \begin{tabular}[c]{@{}l@{}}dry-bulb temp.\\ relative humidity\\ global irradiance\\ hour\\ weekday\end{tabular} & past and future \\ \cmidrule(l){2-3} 
\multicolumn{1}{l}{\textit{The City Theatre}} &  & \textit{} \\
\multirow{2}{*}{Electricity} & electricity & past \\ \cmidrule(l){3-3} 
 & \begin{tabular}[c]{@{}l@{}}is open\\ hour\\ weekday\end{tabular} & past and future \\ \cmidrule(l){2-3} 
\multirow{2}{*}{Heating} & heating & past \\ \cmidrule(l){3-3} 
 & \begin{tabular}[c]{@{}l@{}}dry-bulb temp.\\ relative humidity\\ global irradiance\\ hour\\ weekday\end{tabular} & past and future \\ \bottomrule
\end{tabular}
\end{table}

\subsubsection{Data Transformation}
Data transformation aims to change raw features into a more suitable representation for model learning. For target variables electricity and heating, as well as meteorological features such as dry-bulb temperature, relative humidity, global irradiance, and dew point temperature, a min-max normalization was performed to scale each of them to a range of $[0, 1]$. All min-max scalers were fitted on the training set, then used for transforming validation and test sets. Cyclical features \textit{hour} and \textit{weekday} were transformed into two dimensions using a sine-cosine transformation. Binary features like \textit{is open} were not transformed.

\subsection{Experimental Setup}
\label{sec:study_experimental_setup}

Models are developed for predicting hourly electricity consumption and heating load of the City Museum and the City Theatre 24 steps ahead. In other words, given a forecast origin, models should predict electricity consumption and heating load of the two buildings for each hour of the following 24 hours. The maximum lookback window size was determined by the partial autocorrelation function. Both electricity consumption and heating load of the two buildings on the training set are non-stationary as assessed by the Kwiatkowski–Phillips–Schmidt–Shin test ($p<.01$). Consequently, we took a difference of lag 24 followed by a first difference for each target variable. The result suggested a maximum lookback window size of 168 hours, i.e., seven days, for all target variables.

Based on the seasonal na\"ive (SN) method~\cite{hyndman_forecasting_2018}, two models, namely SN-24 and SN-168, were prepared as baselines because electricity consumption and heating load are highly seasonal. SN-24 model aims to utilize daily seasonality, and each forecast of a target variable was set to be its value observed 24 hours ago. Similarly, for the SN-168 model, each forecast was set to be the value observed 168 hours ago to use weekly seasonality.

All models except for the two baseline models were trained according to the following four cases:
\begin{itemize}
  \item Case 1, point forecast: train the eight models (LR, N-HiTS, TCN, TF, NLinear, LSTM, GRU, and TFT) by only using past values (in the lookback window) of target and predictor variables (see Table~\ref{tab:study_tab4}).
  \item Case 2, point forecast: train the five models (LR, NLinear, LSTM, GRU, and TFT) by incorporating past values (in the lookback window) of target and predictor variables, as well as future values of predictor variables (in the forecast horizon).
  \item Case 3, probabilistic forecast: train the six models that achieved highest prediction accuracy in Cases 1 and 2 with all information they support using. The predefined set of quantiles is $\{0.1,0.5,0.9\}$.
  \item Case 4, point forecast: train the eight models with all information they support using except for the feature related to operating buildings.
\end{itemize}

Case 1 compares the performance of models in making multi-horizon predictions when only using past information. Case 2 looks into the impact of incorporating future information on model prediction accuracy. Case 3 is to investigate the performance of models in probabilistic forecast, and we are interested in evaluating $\rho$-risk on 0.5th and 0.9th quantiles. Case 4 is a sensitivity analysis to examine how operating mode-related features affect model prediction accuracy.

Models were trained by minimizing an appropriate loss function (as defined in Section~\ref{sec:study_loss_func_eval_metric}) on the training set. A sliding window with a step size of one hour was used to generate training samples. All deep learning models were trained by a maximum of 100 epochs. An early-stopping training technique was employed to avoid overfitting. This technique stops the training process when the resulting accuracy in the validation set stops rising after a specified number of iterations. The performance of models was then compared by evaluating the loss function using the validation set, and the models having the lowest loss for the validation set were selected. Finally, the selected models were evaluated and compared by predefined metrics (see Section~\ref{sec:study_loss_func_eval_metric}) on the test set. A sliding window with a step size of 24 hours was used to generate all forecasts on the test set. Since the heating energy of both buildings is from the district heating system, the criterion recommended by the ASHRAE Guideline 14-2014 was applied separately to electricity use and heating load.

All experiments were conducted on a computer with Ubuntu 20.04 operating system. The computer has an Intel Xeon W-2145 CPU, a total of 16~GB memory, and a graphics card NVIDIA GeForce GTX 1080. Models were implemented by Python (v3.8.16) programming language based on libraries PyTorch~\cite{paszke_pytorch_2019} (v1.12.0), darts~\cite{herzen_darts_2022} (v0.23.1), and scikit-learn~\cite{pedregosa_scikit_2011} (v1.2.1).

\section{Results and Discussion}
\label{sec:study_results_and_discussion}
The presentation and discussion of results include three parts. First is the quantitative analysis of the results based on predefined metrics. Then, the results are qualitatively analyzed through the exploratory data analysis approach. Finally, a discussion about integrating the predictive models developed in this study into applying a digital twin model was given.

\subsection{Quantitative Analysis}

The quantitative analysis is to analyze the predictability of various energy use and the performance of models under the four cases.

\subsubsection{Comparison of Predictability of Electricity and Heating}

Both electricity consumption and heating load of the two buildings exhibit a stronger daily seasonality than weekly seasonality as the SN-24 model performed better than the SN-168 model on all metrics (see Table~\ref{tab:study_tab5}). Meanwhile, heating load has stronger daily seasonality than electricity consumption for both buildings since the SN-24 model obtained a lower CV-RMSE on predictions of heating load than that of electricity consumption. Furthermore, prediction accuracy of the SN-24 model suggests that electricity consumption is less predictable than heating load for both buildings. Interestingly, the SN-24 model provides a strong baseline, especially for heating load of both buildings, as its performance on predicting heating loads has met the criterion (30\% for CV-RMSE and $\pm$10\% for NMBE) of the ASHRAE Guideline 14-2014~\cite{ashrae_guideline_14_measurement_2014}.

\begin{table}[!ht]
\centering
%\footnotesize
\caption{The prediction accuracy of point forecasts for different models on the test set when not incorporating future information (Case 1). For both CV-RMSE and NMBE, a closer value to zero represents better prediction accuracy. Electricity is abbreviated as Electr.. }
\label{tab:study_tab5}
\begin{tabular}{@{}llrrcrr@{}}
\toprule
\multicolumn{2}{c}{\multirow{2}{*}{}} & \multicolumn{2}{c}{The City Museum} & \phantom{} & \multicolumn{2}{c}{The City Theatre} \\ \cmidrule(lr){3-4} \cmidrule(l){6-7} 
\multicolumn{2}{c}{} & Electr. & Heating & \multicolumn{1}{l}{} & Electr. & Heating \\ \midrule
\multicolumn{2}{l}{\textit{CV-RMSE (\%)}} \\
 & SN-24 & 45.1 & 24.4 &  & 30.1 & 27.0 \\
 & SN-168 & 55.3 & 41.2 &  & 31.2 & 46.2 \\
 & N-HiTS & \textbf{32.2} & 22.0 &  & 27.7 & 23.5 \\
 & TCN & 37.6 & 22.0 &  & 25.5 & 25.0 \\
 & TF & 40.3 & 23.0 &  & 32.2 & 29.6 \\
 & LR & 36.6 & 20.7 &  & \textbf{23.6} & 24.2 \\
 & NLinear & 33.8 & 29.1 &  & 30.6 & 22.9 \\
 & LSTM & 36.1 & 18.5 &  & 29.4 & 22.4 \\
 & GRU & 37.7 & 20.9 &  & 31.5 & 23.3 \\
 & TFT & 32.6 & \textbf{17.4} &  & 24.7 & \textbf{21.9} \\
\multicolumn{2}{l}{\textit{NMBE (\%)}}\\
 & SN-24 & $-$0.5 & $-$1.1 &  & $-$0.1 & $-$1.2 \\
 & SN-168 & $-$4.9 & $-$8.1 &  & 0.1 & $-$8.9 \\
 & N-HiTS & $-$2.2 & $-$0.4 &  & $-$2.4 & $-$5.9 \\
 & TCN & $-$4.7 & $-$0.6 &  & $-$6.0 & $-$0.3 \\
 & TF & $-$10.0 & 0.1 &  & $-$2.3 & $-$3.3 \\
 & LR & $-$2.8 & $-$0.3 &  & $-$0.9 & $-$0.8 \\
 & NLinear & 7.5 & 18.3 &  & 5.9 & 0.8 \\
 & LSTM & $-$6.4 & $-$0.2 &  & $-$6.0 & 0.8 \\
 & GRU & $-$5.3 & $-$7.3 &  & $-$2.0 & 0.6 \\
 & TFT & $-$1.3 & 2.1 &  & $-$3.5 & 0.3 \\ \bottomrule
\end{tabular}
\end{table}

In addition to baseline models, the performance of the other eight models also indicates higher predictability in heating load. As shown in Table~\ref{tab:study_tab5}, except for the performance of the LR model on the City Theatre, the other seven models achieved a lower CV-RMSE on predictions of heating load than electricity consumption. Moreover, all eight models have met the criterion of the ASHRAE Guideline 14-2014 in predicting heating load of the City Museum, while seven of the eight models (except for the NLinear model, which has an NMBE of 18.3\%) have met the criterion in predicting heating load of the City Theatre. However, no model achieved a CV-RMSE $\leq$~30\% when predicting electricity consumption of the City Museum. This result indicates that it is difficult to make an accurate prediction of the hourly electricity consumption of the City Museum for the next 24 hours by relying only on past information. The situation becomes better when predicting electricity consumption of the City Theatre, where five of the eight models obtained a CV-RMSE $\leq$~30\%. The higher predictability in heating load is attributed to the fact that the two buildings employ adaptive heating, which is driven by the difference between indoor and outdoor temperatures. 

For the same type of energy consumption in different buildings, electricity consumption of the City Museum is less predictable than that of the City Theatre, while heating load is more predictable for the City Museum than the City Theatre. As shown in Table~\ref{tab:study_tab5}, all eight models achieved higher values of CV-RMSE on predictions of electricity consumption of the City Museum than the City Theatre. At the same time, seven of the eight models (except for the NLinear model) achieved lower values of CV-RMSE on heating load of the City Museum than the City Theatre. This phenomenon is attributed to the arrangement of shows in the City Theatre as adjacent days typically performed shows of the same production. For example, 11 shows of the production \textit{Faust II} were performed during the period of September 28 to October 12, 2019. Such an arrangement leads to a high similarity in the operating mode of the City Theatre in neighboring days. However, gathering many audiences in a place for a long time also caused more considerable fluctuations in heating load as more audiences lead to higher internal heat gain~\cite{ni_enabling_2022}.

However, most of the eight models did not obtain a remarkably improved prediction accuracy, e.g., a decrease of 10\% in CV-RMSE, over the baseline SN-24 model when not incorporating future information. For predicting electricity consumption, the N-HiTS model performed best for the City Museum (CV-RMSE 32.2\%), and the LR model performed best for the City Theatre (CV-RMSE 23.6\%). The TFT model obtained the best performance on both buildings for predicting heating load (CV-RMSE 17.4\% for the City Museum and CV-RMSE 21.9\% for the City Theatre). Nevertheless, some models, such as the NLinear model for predicting the heating load of the City Museum and the TF model for predicting the electricity consumption of the City Theatre, cannot even outperform the SN-24 model.

\subsubsection{The Impact of Incorporating Future Information}

Including future values of predictor variables in the forecast horizon increases the prediction accuracy of models by providing information on factors that determine energy consumption. As shown in Table~\ref{tab:study_tab6}, all five models achieved improved performance on the CV-RMSE metric for predicting both types of energy consumption of the two buildings. Also, the improvements of most models (except for NLinear and GRU models on the City Theatre) in predicting heating load are more evident than in predicting electricity consumption. The TFT model performed best on both types of energy consumption of the City Museum (CV-RMSE 29.7\% on electricity consumption and CV-RMSE 8.7\% on heating load). For the City Theatre, the LR model performed best on electricity consumption (CV-RMSE 17.9\%), while the LSTM model performed best on heating load (CV-RMSE 12.5\%). 

\begin{table}[!ht]
\centering
%\footnotesize
\caption{The prediction accuracy of point forecasts for different models on the test set after incorporating future information (Case 2). The values in brackets represent the change in corresponding performance compared to Table~\ref{tab:study_tab5}, and negative values represent improvements.}
\label{tab:study_tab6}
\begin{tabular}{@{}llrrcrr@{}}
\toprule
\multicolumn{2}{c}{\multirow{2}{*}{}} & \multicolumn{2}{c}{The City Museum} & \phantom{} & \multicolumn{2}{c}{The City Theatre} \\ \cmidrule(lr){3-4} \cmidrule(l){6-7} 
\multicolumn{2}{c}{} & Electr. & Heating & \multicolumn{1}{l}{} & Electr. & Heating \\ \midrule
\multicolumn{2}{l}{\textit{CV-RMSE (\%)}} \\
 & \multirow{2}{*}{LR} & 34.5 & 12.4 &  & \textbf{17.9} & 15.8 \\
 &  & ($-$2.1) & ($-$8.3) &  & ($-$5.7) & ($-$8.4) \\
 & \multirow{2}{*}{NLinear} & 32.8 & 23.8 &  & 24.4 & 20.6 \\
 &  & ($-$1.1) & ($-$5.3) &  & ($-$6.3) & ($-$2.3) \\
 & \multirow{2}{*}{LSTM} & 35.7 & 10.9 &  & 22.2 & \textbf{12.5} \\
 &  & ($-$0.3) & ($-$7.6) &  & ($-$7.2) & ($-$9.9) \\
 & \multirow{2}{*}{GRU} & 32.6 & 9.8 &  & 21.4 & 13.5 \\
 &  & ($-$5.1) & ($-$11.1) &  & ($-$10.1) & ($-$9.8) \\
 & \multirow{2}{*}{TFT} & \textbf{29.7} & \textbf{8.7} &  & 20.3 & 12.9 \\
 &  & ($-$2.9) & ($-$8.7) &  & ($-$4.4) & ($-$9.0) \\
\multicolumn{2}{l}{\textit{NMBE (\%)}} \\
 & \multirow{2}{*}{LR} & $-$3.4 & 1.6 &  & $-$0.2 & $-$0.5 \\
 &  & ($+$0.6) & ($+$1.3) &  & ($-$0.8) & ($-$0.3) \\
 & \multirow{2}{*}{NLinear} & $-$3.0 & 11.5 &  & 4.7 & 2.7 \\
 &  & ($-$4.4) & ($-$6.8) &  & ($-$1.2) & ($+$1.9) \\
 & \multirow{2}{*}{LSTM} & $-$6.7 & $-$2.4 &  & 0.8 & $-$1.2 \\
 &  & ($+$0.2) & ($+$2.2) &  & ($-$5.2) & ($+$0.4) \\
 & \multirow{2}{*}{GRU} & $-$6.6 & $-$2.5 &  & 0.0 & $-$3.8 \\
 &  & ($+$1.3) & ($-$4.8) &  & ($-$2.0) & ($+$3.2) \\
 & \multirow{2}{*}{TFT} & $-$6.2 & $-$0.1 &  & $-$0.2 & $-$1.8 \\
 &  & ($+$4.9) & ($-$2.0) &  & ($-$3.3) & ($+$1.5) \\ \bottomrule
\end{tabular}
\end{table}

The highest prediction accuracy achieved with the LR model for predicting electricity consumption of the City Theatre brings some inspiration. If there exist strong linear correlations between some predictor variables and a specific type of energy consumption, a basic linear model might provide a strong baseline for energy forecasting. As illustrated in Table~\ref{tab:study_tab3} of Section~\ref{sec:study_feature_prep}, a strong linear correlation (Pearson's $r=0.734$) exists between the operating mode-related feature \textit{is open} and electricity consumption of the City Theatre. The LR model managed to extract this correlation and generate accurate predictions.

\subsubsection{The Performance of Probabilistic Forecast}

Based on the results in Cases 1 and 2, the best six models for performing point forecasts are N-HiTS, LR, NLinear, LSTM, GRU, and TFT. Among the six models, the TFT model dominates the probabilistic forecast. It performed best to capture the central tendency and upper distribution of heating load of the City Museum as well as both energy consumption of the City Theatre as it achieved the lowest $\rho$-risk at the 0.5th and 0.9th quantiles as in Table~\ref{tab:study_tab7}. For predicting electricity consumption of the City Museum, the GRU model performed best to capture the central tendency of the electricity consumption as it achieved the lowest $\rho$-risk at the 0.5th quantile ($\rho$-risk$(0.5)=0.182$). The N-HiTS model, on the other hand, performed best to capture the upper distribution of electricity consumption of the City Museum ($\rho$-risk$(0.9)=0.142$) and might be useful for predicting extreme values or identifying outliers. Among all models, the LR model performed worst when producing probabilistic forecast. The authors speculated that it is because the LR model assumed that the residuals are normally distributed, which may not hold true when estimating quantiles, as the distribution of the residuals can be skewed.

\begin{table}[!ht]
\centering
%\footnotesize
\caption{The $\rho$-risk at 0.5th and 0.9th quantiles of probabilistic forecasts for different models on the test set (Case 3). For each metric, lower values represent better performance.}
\label{tab:study_tab7}
\begin{tabular}{@{}llrrcrr@{}}
\toprule
 &  & \multicolumn{2}{c}{The City Museum} & \phantom{} & \multicolumn{2}{c}{The City Theatre} \\ \cmidrule(lr){3-4} \cmidrule(l){6-7} 
 &  & Electr. & Heating && Electr. & Heating \\ \midrule
\multicolumn{2}{l}{$\rho$\textit{-risk (0.5)}}\\
 & N-HiTS & 0.199 & 0.133 && 0.199 & 0.164 \\
 & LR & 0.520 & 0.662 && 0.410 & 0.683 \\
 & NLinear & 0.241 & 0.177 && 0.187 & 0.197 \\
 & LSTM & 0.186 & 0.055 && 0.140 & 0.086 \\
 & GRU & \textbf{0.182} & 0.059 && 0.143 & 0.091 \\
 & TFT & 0.192 & \textbf{0.054} && \textbf{0.136} & \textbf{0.081} \\
\multicolumn{2}{l}{$\rho$\textit{-risk (0.9)}}\\
 & N-HiTS & \textbf{0.142} & 0.074 && 0.120 & 0.116 \\
 & LR & 0.266 & 0.296 && 0.210 & 0.268 \\
 & NLinear & 0.159 & 0.136 && 0.099 & 0.122 \\
 & LSTM & 0.143 & 0.029 && 0.072 & 0.058 \\
 & GRU & 0.148 & 0.027 && 0.074 & 0.067 \\
 & TFT & 0.165 & \textbf{0.027} && \textbf{0.070} & \textbf{0.056} \\ \bottomrule
\end{tabular}
\end{table}

The probabilistic forecasts also reflect that heating load has higher predictability than electricity consumption. Except for the NLinear model on heating load of the City Theatre and the LR model, other models achieved lower $\rho$-risk at 0.5th quantile when predicting heating load than electricity consumption for both buildings. Meanwhile, the uncertainties in electricity consumption are larger than heating load since these models also achieved higher $\rho$-risk at 0.9th quantile when predicting electricity consumption than heating load for the two buildings. Nevertheless, The uncertainty in predicting electricity consumption also implies that, on the one hand, it is favorable to enhance certainty by optimizing electricity usage while still ensuring the regular functionality of a building. On the other hand, additional operating model-related features that determine electricity use should be involved for a better forecast.

\subsubsection{Computational Cost}

More complex models typically require more training time to extract patterns in data. As shown in Table~\ref{tab:study_tab8}, the basic LR model consumed far less training time than other deep learning models. Among deep learning models, the TCN and the NLinear models consumed less training time since they processed the entire data sequence in parallel. Recurrent models LSTM and GRU process temporal data sequentially, leading to a slower training process. The computational cost of the N-HiTS model is better than recurrent models. Models employing the self-attention mechanisms, such as TF and TFT, require quadratic time complexity concerning the length of the input sequence, making them less efficient than recurrent models for processing long sequences.

\begin{table}[!ht]
\centering
%\footnotesize
\caption{The computational cost of training different models in seconds. For point forecasting models, TCN, TF, and N-HiTS are from Case 1, while the other six models are from Case 2. Probabilistic forecasting models are all from Case 3.}
\label{tab:study_tab8}
\begin{tabular}{@{}llrrcrr@{}}
\toprule
\multicolumn{2}{c}{} & \multicolumn{5}{c}{Training time (s)} \\ \cmidrule(l){3-7}
\multicolumn{2}{c}{} & \multicolumn{2}{c}{The City Museum} & \phantom{} & \multicolumn{2}{c}{The City Theatre} \\ \cmidrule(lr){3-4} \cmidrule(l){6-7} 
\multicolumn{2}{c}{} & Electr. & Heating &  & Electr. & Heating \\ \midrule
\multicolumn{2}{l}{\textit{Point}} \\
\multicolumn{1}{c}{} & TCN & 664 & 620 &  & 575 & 590 \\
 & TF & 4646 & 4889 &  & 4714 & 4712 \\
 & N-HiTS & 1318 & 1222 &  & 1121 & 1170 \\
 & LR & \textbf{3} & \textbf{3} &  & \textbf{1} & \textbf{2} \\
 & NLinear & 688 & 603 &  & 676 & 451 \\
 & LSTM & 1353 & 2044 &  & 1617 & 1531 \\
 & GRU & 1314 & 1391 &  & 2355 & 1468 \\
 & TFT & 5757 & 6348 &  & 3274 & 3852 \\
\multicolumn{2}{l}{\textit{Probabilistic}} \\
 & N-HiTS & 1389 & 1335 &  & 1150 & 1334 \\
 & LR & \textbf{144} & \textbf{180} &  & \textbf{119} & \textbf{175} \\
 & NLinear & 707 & 753 &  & 258 & 782 \\
 & LSTM & 1958 & 2901 &  & 2018 & 3668 \\
 & GRU & 2405 & 2440 &  & 1595 & 2709 \\
 & TFT & 5529 & 7220 &  & 3653 & 4602 \\ \bottomrule
\end{tabular}
\end{table}

It is worth the training time to develop recurrent models like LSTM and GRU, as well as the TFT model, which integrates LSTM and attention mechanisms. The three models exhibited better performance based on the findings of point and probabilistic forecasts. According to the prediction accuracy of point forecasts (Table~\ref{tab:study_tab6}), the TFT model outperformed other models in predicting both types of energy use of the City Museum (CV-RMSE 29.7\% for electricity consumption and CV-RMSE 8.7\% for heating load) and the LSTM model performed best in predicting heating load of the City Theatre (CV-RMSE 12.5\%). For performing probabilistic forecasts (Table~\ref{tab:study_tab7}), LSTM, GRU, and TFT models obtained lower $\rho$-risks than other models.

\subsubsection{Sensitivity Analysis}

Removing the operating mode-related feature, i.e., \textit{is open}, has a greater impact on predicting electricity consumption of the City Theatre than the City Museum. As shown in Table~\ref{tab:study_tab9}, all five models that support incorporating future information obtained a deteriorated CV-RMSE on forecasts of electricity consumption of the City Theatre. The performance of the TFT (CV-RMSE 31.4\%) and LSTM (CV-RMSE 30.4\%) models failed to outperform the baseline SN-24 model (CV-RMSE 30.4\%). For the City Museum, the performance change of the models varied. Some increased and some decreased, but the overall change was smaller than that of the City Theatre. This is mainly because the linear correlation between the City Theatre and opening hours (Pearson's $r=0.734$ as in Table~\ref{tab:study_tab3}) is greater than that between the City Museum and opening hours (Pearson's $r=0.435$ as in Table~\ref{tab:study_tab2}).

\begin{table}[!ht]
\centering
%\footnotesize
\caption{The change of prediction accuracy of point forecasts when not incorporating opening hours (Case 4). Values in brackets after each metric reflects the performance change (negative values represent improvements, and positive values represent deterioration) versus the model using opening hours. The N-HiTS, TCN, and TF models are compared with Table~\ref{tab:study_tab5} while the other models are compared with Table~\ref{tab:study_tab6}.}
\label{tab:study_tab9}
\begin{tabular}{@{}llrcr@{}}
\toprule
\multicolumn{2}{c}{\multirow{2}{*}{}} & \multicolumn{1}{c}{The City Museum} & \phantom{} & \multicolumn{1}{c}{The City Theatre} \\ \cmidrule(lr){3-3} \cmidrule(l){5-5} 
\multicolumn{2}{c}{} & Electricity &  & Electricity \\ \midrule
\multicolumn{2}{l}{\textit{CV-RMSE (\%)}} \\
 & N-HiTS & 33.8 ($+$1.7) &  & 26.1 ($-$1.6) \\
 & TCN & 38.2 ($+$0.6) &  & 25.0 ($-$0.5) \\
 & TF & 38.0 ($-$2.3) &  & 31.9 ($-$0.3) \\
 & LR & 36.0 ($+$1.6) &  & \textbf{23.4} ($+$5.5) \\
 & NLinear & 35.3 ($+$2.5) &  & 29.8 ($+$5.4) \\
 & LSTM & 33.8 ($-$2.0) &  & 30.4 ($+$8.2) \\
 & GRU & 33.2 ($+$0.6) &  & 28.1 ($+$6.7) \\
 & TFT & \textbf{32.5} ($+$2.7) &  & 31.4 ($+$11.1) \\
\multicolumn{2}{l}{\textit{NMBE (\%)}} \\
 & N-HiTS & $-$9.0 ($+$6.8) &  & $-$5.9 ($+$3.4) \\
 & TCN & $-$6.6 ($+$1.9) &  & $-$4.6 ($-$1.5) \\
 & TF & $-$4.3 ($-$5.8) &  & $-$2.0 ($-$0.2) \\
 & LR & $-$3.3 ($-$0.1) &  & $-$0.9 ($+$0.8) \\
 & NLinear & 4.6 ($+$1.6) &  & $-$5.2 ($+$0.5) \\
 & LSTM & $-$1.1 ($-$5.6) &  & $-$4.2 ($+$3.4) \\
 & GRU & $-$2.8 ($-$3.8) &  & $-$1.4 ($+$1.4) \\
 & TFT & $-$7.5 ($+$1.3) &  & $-$0.7 ($+$0.5) \\ \bottomrule
\end{tabular}
\end{table}

No model met the criterion (30\% for CV-RMSE) of the ASHRAE Guideline 14-2014 for predicting electricity consumption of the City Museum when not incorporating operational features. This suggests that more factors that determine electricity consumption, such as the scheduling of ventilation and lighting systems, should be involved to improve prediction accuracy.

\subsection{Qualitative Analysis}

The qualitative analysis interprets the impact of operating modes and activities on energy use.

\subsubsection{Changes in Operating Mode of the City Museum}
Previous quantitative analysis suggested that electricity consumption of the City Museum is less predictable than that of the City Theatre. The lower predictability was partly due to changes in the operating mode of the City Museum on some days in November and December 2019. Fig.~\ref{fig:study_fig8}{a} shows such a change. During the five days, from November 29 to December 3, the hourly energy consumption in the nighttime was even higher than in the daytime of the previous days. Meanwhile, the operating mode in these five days was also different. Among them, the hourly electricity consumption in the daytime was relatively high on November 29, December 2, and December 3, while it was relatively low on November 30 and December 1. From December 4, the operating mode changed to the pattern before November 29.

\begin{figure}[!ht]
\includegraphics[width=\textwidth]{figures/study/fig8.png}
\centering
\caption{The actual and predicted hourly electricity consumption of the City Museum from November 26 to December 6, 2019. (\textbf{a}) Point forecasts of the best three models and (\textbf{b}) probabilistic forecast of the GRU model. The predicted median is P50, and the 80\% prediction interval (PI) is from 0.1th to 0.9th quantile.}\label{fig:study_fig8}
\end{figure}

The changes in operating mode degrade the prediction accuracy of models during these days. On November 29 (the first day when the operating mode started to change), all three models believed the original operating mode would be maintained. Therefore, the forecasts followed the pattern in the previous operating mode (see Fig.~\ref{fig:study_fig8}{a}). The good news is that models adjusted their forecasts to adapt to the new operating mode from November 30 (the second day that the operating mode changed). After the operating mode changed to the old pattern before November 29, the forecasts of models also adapted to the change. The changes also introduce more uncertainty into forecasts. As shown in Fig.~\ref{fig:study_fig8}{b}, the 80\% prediction interval (from 0.1th quantile to 0.9th quantile) during the daytime of the five days from November 29 to December 3 was relatively higher than during the daytime of the days before the operating mode changed. Furthermore, the higher uncertainty for forecasts during the daytime continued after the operating mode changed to the old pattern (see December 4 and 5). 

Similar changes in the operating mode of the City Museum caused the prediction accuracy of models to deteriorate in November and December compared to the previous three months in the test set. As assessed by inspecting the boxplot (see Fig.~\ref{fig:study_fig9}) of CV-RMSE per 24 hours of the best five models, the median CV-RMSE of most models increased in November and December, and the distribution became broader in the two months.

\begin{figure}[!ht]
\includegraphics{figures/study/fig9.png}
\centering
\caption{The boxplot of the metric CV-RMSE per 24 hours of the best five models for predicted electricity consumption of the City Museum on the test set.}\label{fig:study_fig9}
\end{figure}

\subsubsection{Uncertainty Brought by Performing Shows in the City Theatre}
Activities held in a building might bring some uncertainty to electricity consumption. Fig.~\ref{fig:study_fig10} depicts the actual and predicted hourly electricity consumption of the City Theatre in four days of October 2019. Each of the first three days had a show performed, and each show lasted for three hours. The hourly electricity consumption was higher during the show, and these predictive models can make good predictions ( Fig.~\ref{fig:study_fig10}{a}). However, there is more uncertainty in forecasts when there are shows performed ( Fig.~\ref{fig:study_fig10}{b}). Interestingly, on October 7 (Monday), the electricity consumption was expected to drop after 18:00, according to the probabilistic forecast (P50). However, it remained high until 23:00. Such information can be further investigated to better understand building energy use.

\begin{figure}[!ht]
\includegraphics{figures/study/fig10.png}
\centering
\caption{The actual and predicted hourly electricity consumption of the City Theatre from October 4 (Friday) to October 7 (Monday), 2019. (\textbf{a}) Point forecasts of the best three models and (\textbf{b}) probabilistic forecast of the TFT model. During the first three days, one show was performed each day. No show was performed on the last day.}\label{fig:study_fig10}
\end{figure}

\subsubsection{Heating is More Predictable than Electricity}
Previous quantitative analysis indicates that heating load is more predictable than electricity consumption. On the one hand, higher predictability is attributed to strong influencing factors like dry-bulb temperature being involved in making predictions. On the other hand, the heating load is less affected by the change in operating mode. As shown in Fig.~\ref{fig:study_fig11}{a}, even on November 29 and 30, the two days when the operating mode changed, the best three models still made good predictions.
Similarly, the uncertainty in predictions was greater during the daytime than during the nighttime (see Fig.~\ref{fig:study_fig11}{b}). The authors speculated that higher uncertainty in the daytime is likely due to more heat exchange between the indoor and the outdoor environment brought by staff and visitors.

\begin{figure}[!ht]
\includegraphics{figures/study/fig11.png}
\centering
\caption{The actual and predicted hourly heating load of the City Museum from November 26 to November 30, 2019. (\textbf{a}) Point forecasts of the best three models and (\textbf{b}) probabilistic forecast of the TFT model. }\label{fig:study_fig11}
\end{figure}

\subsection{Applying a Digital Twin Model}

The predictive models developed in this study can be integrated into a digital twin model of the energy system of a building or a digital twin model of the entire building. A digital twin is a virtual model of a physical object~\cite{glaessgen_digital_2012}. The physical object, e.g., a building, is deployed with various sensors related to its critical functional areas. These sensors collect information about various aspects of physical object status, such as energy consumption and indoor climate. These data are then synchronized to the digital twin for further analysis to provide functions like real-time monitoring and diagnosis. Creating a digital twin of a building can combine information and communication technologies, such as Internet of Things, cloud computing, and ontology~\cite{ni_enabling_2022}. A digital twin model of a building contributes to several aspects of the operation and maintenance of the building, including defect detection and asset monitoring, analysis and diagnosis, as well as automatic control~\cite{jiang_digital_2021}.

By integrating predictive models developed in this study, the digital twin model can predict the future energy consumption of a building. A digital twin model can also simulate energy use in different operating modes and conditions. This can be used to discover areas where energy use can be reduced, optimize building operations, and improve overall sustainability and efficiency. Furthermore, the data generated by a digital twin can be utilized to continuously improve the prediction accuracy of the energy forecasting model. It creates a feedback loop where the digital twin helps increase the accuracy of the forecasting model, which in turn improves the effectiveness of the digital twin. This could ultimately result in cost savings, improved human comfort, and a more sustainable built environment.

\section{Conclusion}
\label{sec:study_conclusion}

This study set out to adapt and apply state-of-the-art deep learning architectures to address the problem of multi-horizon building energy forecasting. Eight methods, including seven deep learning architectures, were studied to develop models for point and probabilistic forecasts. A comprehensive case study was conducted on two public historic buildings in Norrk\"oping, Sweden, to evaluate the performance of these models and investigate factors that affect the predictability of energy consumption. 

The results show that incorporating future information that determines energy consumption is critical for making multi-horizon predictions. Moreover, changes in the operating mode of a building and activities held in a building bring more uncertainty in energy consumption and deteriorate the performance of point forecasts. For point forecast, the TFT model performed best on both types of energy consumption of the City Museum (CV-RMSE 29.7\% on electricity consumption and CV-RMSE 8.7\% on heating load). The LR model performed best on electricity consumption of the City Theatre (CV-RMSE 17.9\%), while the LSTM model performed best on heating load of the City Theatre (CV-RMSE 12.5\%). The TFT model dominated the probabilistic forecast. Meanwhile, recurrent models like LSTM and GRU can make competitive quantile forecasts.

For future work, more features, especially occupancy and building operational data, might be included to study their impact on prediction accuracy. Also, the predictive models developed in this study could be integrated into a digital twin model of a building to reduce energy use while keeping the expected functionalities of the building.

\section{Acknowledgements}
The Swedish Energy Agency is acknowledged for the financial support of this study. The authors thank Johan Bj\"orhn and his colleagues at Norrevo Fastigheter AB in Norrk\"oping for providing access to the City Museum and the City Theatre as well as offering historical energy consumption data for these two buildings. Anna Donarelli at Uppsala University helps collect information about shows performed in the City Theatre. The Swedish Meteorological and Hydrological Institute is acknowledged for providing application programming interfaces to access meteorological data.

\printbibliography[heading=subbibliography]
\end{refsection}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../demothesis"
%%% End: 


==> pdftopdfa <==
#! /usr/bin/env bash
filenames=${@%.pdf}
#### Use sRGB for now, proper color profile handling likely first in latex-3
#  -sColorConversionStrategy=UseDeviceIndependentColor 
for filename in ${filenames[@]}; do
  echo Converting ${filename}.pdf
  gs -dPDFA -dBATCH -dNOPAUSE              \
    -sColorConversionStrategy=RGB          \
    -sDEVICE=pdfwrite                      \
    -dPDFACompatibilityPolicy=3            \
    -sOutputFile=${filename}_pdfa_rgb.pdf  \
     ${filename}.pdf
  gs -dPDFA -dBATCH -dNOPAUSE              \
    -sColorConversionStrategy=CMYK         \
    -sDEVICE=pdfwrite                      \
    -dPDFACompatibilityPolicy=3            \
    -sOutputFile=${filename}_pdfa_cmyk.pdf \
     ${filename}.pdf
done


==> sammanfattning.tex <==
%%% sammanfattning.tex --- 
%% 
%% Filename: sammanfattning.tex
%% Description: 
%% Author: Ola Leifler
%% Maintainer: 
%% Created: Thu Oct 14 13:34:11 2010 (CEST)
%% Version: $Id$
%% Version: 
%% Last-Updated: Thu Apr 13 11:36:41 2017 (+0200)
%%           By: Ola Leifler
%%     Update #: 8
%% URL: 
%% Keywords: 
%% Compatibility: 
%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% 
%%% Commentary: 
%% 
%%  Populärvetenskaplig sammanfattning av arbetet på svenska
%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% 
%%% Change log:
%% 
%% 
%% RCS $Log$
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% 
%%% Code:

Smart underhåll av kulturhistoriska byggnader med digital teknologi och dataanalys underlättar bevarandet av det kulturhistoriska värdet såväl som anpassning för olika användning. Lokalt utplacerade uppkopplade sakernas internet enheter (Internet of Things, IoT) möjliggör realtidsövervakning av miljösensordata. Genom att analysera insamlade data så kan beslutsfattare identifiera och proaktivt hantera potentiella risker i byggnaden. Underhåll av kulturhistoriska byggnader är ett långsiktigt arbete där varje åtgärd kan få långtgående konsekvenser. Digitala verktyg kan därför bidra dels genom bättre historisk spårbarhet, dels genom bättre prediktion av vad som kommer att hända med byggnaden. En lyckad digital transformering kräver stabila och skalbara lagrings- och beräkningsresurser för att organisera och presentera byggnadsdata. Flexibla applikationer med väl integrerad dataanalys är viktigt för att teknologins fulla potential ska kunna nås.

Denna licentiatavhandling presenterar ett digitaliseringsramverk som adresserar dessa utmaningar genom att integrera IoT, molnberäkning, ontologisk modellering och maskininlärning. IoT-enheterna möjliggör realtidsövervakning av byggnadens status. Användningar en publika molnplattform erbjuder stabila och skalbara resurser för att lagra och analysera data. Ontologi ger ett klart och koncist sätt att organisera och representera byggnadsdata, vilket gör det enklare att förstå hur olika ingående delar påverkar byggnaden. Från detta kan fysikaliskt motsvarande digitala tvillingar skapas. Genom att applicera maskininlärning på dessa tvillingar så kan mönster identifieras som ger beslutsfattaren all nödvändig information för ett smart, väl optimerat underhåll av byggnaden.

Artikel I och II fokuserar på konceptformulering och validering av principen. Artikel I går igenom metoden som används för att skapa digitala tvillingar av historiska byggnader. Artikel II presenterar en referensimplementation av metoden. Den implementerade lösningen är ett komplett system för datainsamling, dataöverföring genom en edge-plattform och datalagring med Microsoft Azure Cloud. Artikel III presenterar fälttest med det egenutvecklade systemet i tre olika historiska byggnader, nämligen Stadsteatern, Stadsmuseet och Hörsalen i Norrköping, Sverige. Fälttestet verifierar stabiliteten hos systemet när det gäller långsiktig drift för datainsamling. Artikel IV introducerar ontologisk modellering till systemet för att tillhandahålla ett enhetligt format för att organisera och representera byggnadsdata. En fallstudie utfördes i Stadsteatern för att verifiera lösningens användbarhet, det studerades hur antalet besökare påverkar inomhusklimatet och potentiella risker identifierades. Artikel V och VI jämför prestanda hos moderna djupinlärningsmetoder med avseende på förmåga att prognostisera byggnaders energiförbrukning. Artikel V fokuserar på prestanda hos egenutvecklade prediktiva modeller vilka utvärderades i Stadsteatern och Stadsmuseet, som utgör två olika driftsfall. Artikel VI visar vad kombinationen av prediktiva modeller och digitala tvillingar kan göra för att förbättra byggnaders energiprestanda.

Sammanfattningsvis bidrar denna avhandling till bevarande av kulturhistoriskt viktiga byggnader med ett omfattande digitaliseringsramverk. Ett ramverk som integrerar olika digitala teknologier med en holistisk strategi för att möjliggöra smart underhåll av historiska byggnader.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% sammanfattning.tex ends here


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "demothesis"
%%% End: 

